Piecing Together Clues: A Benchmark for Evaluating the Detective Skills of Large Language Models

Detectives frequently engage in information detection and reasoning simultaneously when making decisions across various cases, especially when confronted with a vast amount of information. With the rapid development of large language models~(LLMs), evaluating how these models identify key information and reason to solve questions becomes increasingly relevant. We introduces the DetectBench, a reading comprehension dataset designed to assess a model's ability to jointly ability in key information detection and multi-hop reasoning when facing complex and implicit information. The DetectBench comprises 3,928 questions, each paired with a paragraph averaging 190 tokens in length. To enhance model's detective skills, we propose the Detective Thinking Framework. These methods encourage models to identify all possible clues within the context before reasoning. Our experiments reveal that existing models perform poorly in both information detection and multi-hop reasoning. However, the Detective Thinking Framework approach alleviates this issue.

==> figures/GPT4Verification.tex <==
\begin{figure*}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tikzpicture}
\begin{axis}[
    title={Correlation between Consistency and Length of Answers},
    xlabel={Answer Length},
    ylabel={Consistency},
    xmin=20, xmax=305,
    ymin=0, ymax=5.3,
    height=4cm,
    width=10cm,
    xtick={25,50,75,100,125,150,175,200,225,250,275,300},
    ytick={0,1,2,3,4,5},
    legend pos=south east,
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=blue,
    mark=square,
]
coordinates {
% (5,25)(4,50)(4,75)
(25,5)(50,5)(75,5)(100,5)(125,4)(150,4)(175,5)(200,5)(225,5)(250,4)(275,4)(300,4)
};
\legend{Consistency}

\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[
    title={Correlation between Consistency and Length of Answers},
    xlabel={Answer Length},
    ylabel={Consistency},
    xmin=20, xmax=305,
    ymin=0, ymax=5.3,
    height=4cm,
    width=10cm,
    xtick={25,50,75,100,125,150,175,200,225,250,275,300},
    ytick={0,1,2,3,4,5},
    legend pos=south east,
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=blue,
    mark=square,
]
coordinates {
% (5,25)(4,50)(4,75)
(25,5)(50,5)(75,5)(100,5)(125,4)(150,4)(175,5)(200,5)(225,5)(250,4)(275,4)(300,4)
};
\legend{Consistency}

\end{axis}
\end{tikzpicture}
}

\caption{The correlation between the consistency of GPT-4 scores and human scores to the length of ground truth.
The average consistency shown in the figure is 91.7\%.}
\label{fig:gpt4verification}
    \vspace{-3mm}
\end{figure*}

==> figures/SQPerformance.tex <==
\begin{figure*}[t]
    \centering
    % \resizebox{\textwidth}{!}{\includegraphics{figures/ContextLength.png}\includegraphics{figures/HintLength.png}\includegraphics{figures/AnswerLength.png}\includegraphics{figures/ReasoningLength.png}}
    \resizebox{\textwidth}{!}{\includegraphics{figures/SQPerform.png}}
    
    \caption{
    The correlation between GPT-4's performance on Self-Question Prompts and human performance with the length of the Question, Hint, Ground Truth, and Reasoning Length. 
    And the correlation between the time expenditure of human reasoning with the length of the Question, Hint, Ground Truth, and Reasoning Length.
    % The correlation between the GPT-4 performance of Self-Question Prompt and human Performance with the length of Question, Hint, Ground Truth, and Reasoning Length. 
    % And the correlation between the time expense of human spend in reasoning with with the length of Question, Hint, Ground Truth, and Reasoning Length.
    }
    \label{fig:SQPerformance}
    \vspace{-5mm}
\end{figure*}

==> latex/01.Introduction.02.tex <==
Reasoning ability is crucial for helping individuals make decisions, solve problems, and think critically based on the existing knowledge and situation~\cite{huang2022towards,qiao2022reasoning}.
In Cognitive Psychology, ``reasoning'' is composed of formal reasoning and informal reasoning~\cite{frith2008implicit,apperly2009humans}.
Formal reasoning is a systematic and logical process that follows a set of rules and principles, often used in mathematics and logic. 
While, informal reasoning is a less structured approach that relies on intuition, experience, and common sense to draw conclusions and solve problems, and is often used in everyday life~\cite{galotti1989approaches, bronkhorst2020logical}.
Notwithstanding the prevalence of formal reasoning in the field of machine learning research, the term ``reasoning'' mostly refer to informal reasoning in its common, everyday usage~\cite{cobbe2021training,huang2022towards}.

\begin{figure}[t]
    \centering
    \resizebox{0.8\columnwidth}{!}{
    \includegraphics{./figures/introduction.pdf}
    }
    \caption{A real response from GPT-4.
    Despite employing thorough prompting, GPT-4 continues to exhibit a deficiency in understanding real-life scenarios.}
    \label{fig:intro}
    \vspace{-5mm}
\end{figure}

The ability of Informal Reasoning is a fundamental human capability, permeating people's daily lives~\cite{blanchette2010influence,perkins2012everyday,bronkhorst2020logical}. 
For instance, on a hot summer day, when observing many people sitting in a room with closed windows and doors, one can easily deduce that the room is air-conditioned. 
The process of deduction is based on the common sense of the reasoner and the experience of once sitting in air-conditioned rooms.
This manifestation of inference abilities prevalent across diverse real-life scenarios showcases an array of cognitive skills, such as grasping common sense, abstracting problems, computing probabilities, discarding irrelevant information, and employing logical reasoning. 
Humans excel at doing informal reasoning, especially in life scenarios, often extracting conclusions subconsciously within a brief time span~\cite{woiceshyn2020intuiting}. 
As the capabilities of LLMs continue to scale these days, the crucial question arises: \textit{Can artificial neural networks also display super-powerful informal reasoning capabilities just like or go beyond humanity?}





Limited attention has been devoted to exploring this question within the field of Natural Language Processing~(NLP)~\cite{kaddour2023challenges,huang2022towards} after the fast development of large language models~(LLMs). 
Currently, the majority of AI reasoning endeavors concentrate on formulaic reasoning~\cite{hendrycks2021measuring, lewkowycz2022solving} or predicate reasoning~\cite{lu2022parsing}. 
Although these reasoning capacities aid the prevailing LLMs in tackling abstract problems~\cite{fu2023chain}, they fall short in fostering a deeper comprehension of human experiences.
To propel LLMs towards achieving Artificial General Intelligence~(AGI), it is imperative to not only cultivate their reasoning capabilities in disciplines such as mathematics and physics but as well as equip them with the ability to reason within real-world contexts.
Even the advanced GPT-4, which is considered to be one of the most powerful LLM, exhibits a lackluster performance in informal reasoning as illustrated in Fig.~\ref{fig:intro}.


Transitioning from mere recognition of the gap between LLMs and humans in informal reasoning ability to the investigation of human-like reasoning in neural models and narrowing this gap, we underscore the significance of developing a novel reasoning dataset targeting everyday life scenarios.
To this end, we introduce Detective Reasoning Puzzle Benchmark, which is an assembly of 1,200 questions gathered from accessible online resources and aiming at evaluating the model's informal reasoning ability in real life context.
Compared to recent popular domain knowledge reasoning datasets, the Detective Reasoning Puzzle Benchmark primarily comprises many detective-related questions, incorporating an abundance of information pertaining to character roles, human behaviors, mental activities, and environment description.
Solving these problems requires models to discover clues from details in the context, and reasoning based on the connection between clues and the questions.


In addition, we propose the Self-Question Prompt Framework to bridge the gap in LLMs' ability to carry out informal reasoning. 
To borrow the idea from the powerful informal reasoning ability of humans, we recruited 50 participants to tackle 20 questions each from the Detective Reasoning Puzzle Benchmark, leading to a detailed study of the reasoning processes of both humans and the model. 
Most participants said they find the clues mainly based on intuition without deeper thinking during the test, which is a typically informal reasoning process that sidesteps logical thinking, and instead uses experience and common sense to unearth critical elements in the context, promoting deep reflection, ultimately resulting in a reasoned outcome.
By mirroring human intuitive thinking, Self-Questioning is composed of four steps to improve the model's ability for informal reasoning. 
The goals of these steps respectively are to find key elements, deeply investigate the connections between these elements, encourage the relationship between each element and the problem, and finally, require the model to reasonably answer the problem.

Experimental results show that even the lowest score amongst participants~(46.6\%) significantly surpasses the best score from the LLMs questioned based on naive prompt~(16.0\%) within Detective Reasoning Puzzle Benchmark. 
Compared to the reasoning-enhanced prompts proposed by other researchers, our proposed self-question prompt generated the greatest performance improvement for GPT-4~(an increase of 17.4\%).
Although a self-question prompt is a better way to excite the model's potential in doing informal reasoning, there is still a huge gap between the SoTA LLMs performance~(33.4\%) with the average human participants~(74.2\%).




In conclusion, our study makes several key contributions: 
(1) To facilitate further detailed exploration into the informal reasoning abilities of large language models, we constructed Detective Reasoning Puzzle Benchmark, which is super challenging for LLMs but easy for humans, that includes 1,200 pieces of detective reasoning data. 
% Solving these reasoning problems requires the model to be able to disregard irrelevant information, utilize common knowledge, identify incongruities in the details of the problem, and thereby arrive at a proper reasoning outcome. 
(2) We designed a self-questioning prompt framework that can reliably induce the model to identify irrelevant information, draw the clue from the context, and perform reasoning based on the clues drawn from the details in the context. 
(3) We collected actual human responses to the Detective Reasoning Puzzle Benchmark and carried out numerous experiments using LLMs. 
Regarding these experimental outcomes, we conducted extensive analysis and discussion, which includes the gap between existing LLMs and humans in informal reasoning, the superiority of self-questioning prompts, and how LLMs can supplement informal reasoning abilities.



% Although formal reasoning is often occured in machine learning researches, the term ``reasoning'' refer to informal reasoning in most daily usage~\cite{cobbe2021training,huang2022towards}.

% The faculty of reasoning plays a pivotal role in equipping individuals with the capacity to make informed decisions, resolve predicaments, and exercise critical thinking, grounded in pre-existing knowledge and situational contexts~\cite{huang2022towards,qiao2022reasoning}. 
% Within the domain of Cognitive Psychology, ``reasoning'' encompasses two facets, namely formal and informal reasoning. Formal reasoning denotes a systemic, logical procedure adhering to a prescribed set of rules and principles, which is primarily employed within mathematics and logic. 
% Conversely, informal reasoning represents a less regimented approach that calls upon intuition, experience, and practical wisdom to derive conclusions and untangle situations. It is typically utilized in day-to-day life~\cite{galotti1989approaches, bronkhorst2020logical}. 
% Notwithstanding the prevalence of formal reasoning in the field of machine learning research, the term ``reasoning'' mostly refer to informal reasoning in its common, everyday usage~\cite{cobbe2021training,huang2022towards}.


% Transitioning from mere recognition of real-life scenarios to the investigation of human-like reasoning in neural models, we underscore the significance of developing a novel reasoning dataset targeting everyday life scenarios.
% To narrow this gap, we introduce Detective Reasoning Puzzle Benchmark, which is an assembly of 1,200 questions gathered from accessible online resources, aims at evaluating the model's informal reasoning ability in real life context.


% 进一步，我们提出使用Self-Question Prompt Framework来弥补LLM在Informal Reasoning能力上的缺失。
% 我们邀请了50位参与者每人回答20道Detective Reasoning Puzzle Benchmark里的题目，并对人类和模型的推理过程进行了详细的分析。
% 大多数受试者在测试时都依靠直觉进行了推理。
% 直觉推理是一种绕过理性思考，依靠经验和常识发现Context中的关键点，并进行深度思考，最终得到推理结果的方法。
% LLM没有直觉，所以我们尝试改进prompt，通过不断地Self-Question来还原人类依靠直觉进行思考的过程，从而提升LLM的informal reasoning能力。



% 我们模仿人类的直觉思考，设计了Self-Question的四个过程来增强模型的informal reasoning的能力，目标分别是发现关键要素、深究要素之间的关联、启发各个要素与问题之间的联系，最后要求模型合理地回答问题。

% we recreating the human thought process driven by intuition through continuous Self-Questioning, thereby enhancing the LLM's capacity for informal reasoning.



% The benchmark consists of an assembly of 1,200 questions compiled from accessible online resources.
% The question is mainly gathered from open source web, and are filtered and preprocessed manually before experiments and released.
% Except for the ``Context'', ``Question'' and ``Answer'', which can be obtained directly from online resource, we manually annotate the ``Hint'' for every question to facilitate model training or deep exploration for furture research. 

% We referred to guidelines built on psychological principles~\cite{minnameier2010abduction} and made use of web scraping to gather clear explanations and hint for each question and answer within the Benchmark.
% Since there are lot of internet slang, incorrect words present in the raw text, and varying quality levels of the initial questions, we proceeded with a manual review. 
% Ultimately, each question is transformed into a structured form as depicted in Fig.~\ref{fig:example}.

% In addition to this, we have further designed a prompt framework capable of thoroughly extracting various detailed information from the context to increase the performance of LLM on Detective Reasoning Puzzle Benchmark.
% As LLM generally assumes that prompts are correct and useful, the presence of distracting information greatly hampers its effectiveness~\cite{shi2023large}.
% Besides, we find that ChatGPT and GPT-4, which are LLMs contain huge amount of common-sense knowledge, have better performance in answering the detective reasoning puzzles when step-by-step asking them to draw the clue from the context, and do the reasoning based on the given context and the clues.
% In order to stably induce LLMs to ignore the irrelevant context, and to find the clues based on the given context, we propose the self-question prompt framework.
% As depicted in Fig.~\ref{fig:intro}, the self-question prompt framework comprises four stages: detail detection, detail connection, relevance inspiration, and output command.
% This approach allows models to uncover the implicit hints embedded within the context, discard irrelevant information, and reasoning based on beneficial information.


% To evaluate the gap between human and AI models in informal reasoning, we invite 50 participants to each answer 20 questions within our proposed Detective Reasoning Puzzles Benchmarks. 
% In addition, we examined the performance of four best models in Alpaca-Eval with different parameter magnitudes on the Detective Reasoning Puzzles Benchmarks. 
% Given that GPT-4 has been confirmed by most researchers to have strong evaluation capabilities, we employed GPT-4 to help with our assessments. 
% To ensure accuracy, we utilized manual sampling evaluations to cross-check the results derived from GPT-4. 



% \begin{enumerate}
% \item To facilitate further detailed exploration into the informal reasoning abilities of large language models, we constructed a detective reasoning benchmark that includes 1,200 pieces of detective reasoning data. 
% Solving these reasoning problems requires the model to be able to disregard irrelevant information, utilize common knowledge, identify incongruities in the details of the problem, and thereby arrive at a proper reasoning outcome. 
% \item We designed a self-questioning prompt framework that can reliably induce the model to identify irrelevant information, draw the clue from the context, and perform reasoning based on the clues drawn from the details in context. 
% \item We collected actual human responses to the Detective Reasoning Benchmark and carried out numerous experiments using LLMs. 
% Regarding these experimental outcomes, we conducted extensive analysis and discussion, which includes the gap between existing LLMs and human in informal reasoning, the superiority of self-questioning prompts, and how LLMs can supplement informal reasoning abilities.

% \end{enumerate}


==> latex/01.Introduction.03.tex <==
人类每天面对那么大量的信息，总能够过滤掉各种不重要的信息，利用重要的信息来帮助自己进行抉择。
xxxx
随着大语言模型变得越来越智能。
我们会疑问，大语言模型是否也具有从大量信息中寻找重要信息的能力。

考虑到以往的benchmark很多都是要求模型根据已有的信息来推断出答案。
但并没有很多工作研究模型是否能够从大量无关信息中找到和问题相关的关键信息。
大多数现有的模型和算法重点关注在已知信息的逻辑推理上，忽略了信息筛选的重要性。
因此，我们认为研究这个领域对于提高模型的实用性和普适性至关重要。

我们提出Detective Reasoning Benchmark，一个以选择题为主的Benchmark。
这个benchmark基于大量的开源侦探推理puzzle来进行设计，包含了大量的环境、情节、角色的描述，许多内容都跟问题有着若有若无的联系，只有能够深入理解这些内容背后的连接，才能够破解问题。


考虑到过程监督的重要性，我们为所有的题目标注了合理的推理过程。
我们将推理过程构造成graph的形式，即clue graph，来保证推理的逻辑性和系统性。
具体而言，clue graph从原文中和问题有关的信息出发，不断发现信息背后的新线索，以及线索之间所可能产生的连接，最终推导出答案。

根据我们提出的benchmark，我们设计了一个名为Self-Question Prompt的方法，这个方法能够用来增强LLM在过滤大量无关信息场景下的Zero-Shot Reasoning的performance。
这种方法要求模型根据问题慢慢精炼自己获得到的信息，最后得到最有用的结果。
在跟其他增强模型Performance的Prompt方法对比下，我们的方法能够明显增加模型的推理效果。
除此之外，我们发现将Self-Question Prompt和clue-graph一起用来微调模型，还能够增强在Detective Reasoning Benchmark上Self-Question的Zero-Shot performance

除此之外，我们发现将clue graph的部分内容以Context的形式注入LLM之后，几乎所有参数量级别的LLM效果都能有所提升。
这说明了clue graph本身质量的可靠性，同时也证明了题目具有复杂性，因此需要多步推理。
但值得惊讶的是，当把Clue Graph完整地注入LLM，即答案也注入模型，仍然有小部分模型无法答对所有题目。


总结而言，我们在这篇论文中做出的贡献如下：
1. 我们设计了一个Detective Reasoning Benchmark
2. 我们设计了Self-Question Prompt来增强Zero-shot Performance
3. 我们基于Detective Reasoning Benchmark中的clue graph和Self-Question Prompt，发现了一种可以增强模型xxx性能的微调方法
4. 我们做了大量的实验，发现现有模型难以发现关键信息，并且即便给定了关键信息，也难以做出深层次的推理。而在经过了合理地微调之后，模型可以有效地缓解这一情况


% The ability of Informal Reasoning is a fundamental human capability, permeating people's daily lives~\cite{blanchette2010influence,perkins2012everyday,bronkhorst2020logical}. 
% For instance, on a hot summer day, when observing many people sitting in a room with closed windows and doors, one can easily deduce that the room is air-conditioned. 
% The process of deduction is based on the common sense of the reasoner and the experience of once sitting in air-conditioned rooms.
% This manifestation of inference abilities prevalent across diverse real-life scenarios showcases an array of cognitive skills, such as grasping common sense, abstracting problems, computing probabilities, discarding irrelevant information, and employing logical reasoning. 
% Humans excel at doing informal reasoning, especially in life scenarios, often extracting conclusions subconsciously within a brief time span~\cite{woiceshyn2020intuiting}. 
% As the capabilities of LLMs continue to scale these days, the crucial question arises: \textit{Can artificial neural networks also display super-powerful informal reasoning capabilities just like or go beyond humanity?}

% Limited attention has been devoted to exploring this question within the field of Natural Language Processing~(NLP)~\cite{kaddour2023challenges,huang2022towards} after the fast development of large language models~(LLMs). 
% Currently, the majority of AI reasoning endeavors concentrate on formulaic reasoning~\cite{hendrycks2021measuring, lewkowycz2022solving} or predicate reasoning~\cite{lu2022parsing}. 
% Although these reasoning capacities aid the prevailing LLMs in tackling abstract problems~\cite{fu2023chain}, they fall short in fostering a deeper comprehension of human experiences.
% To propel LLMs towards achieving Artificial General Intelligence~(AGI), it is imperative to not only cultivate their reasoning capabilities in disciplines such as mathematics and physics but as well as equip them with the ability to reason within real-world contexts.
% Even the advanced GPT-4, which is considered to be one of the most powerful LLM, exhibits a lackluster performance in informal reasoning as illustrated in Fig.~\ref{fig:intro}.

% Transitioning from mere recognition of the gap between LLMs and humans in informal reasoning ability to the investigation of human-like reasoning in neural models and narrowing this gap, we underscore the significance of developing a novel reasoning dataset targeting everyday life scenarios.
% To this end, we introduce Detective Reasoning Puzzle Benchmark, which is an assembly of 1,200 questions gathered from accessible online resources and aiming at evaluating the model's informal reasoning ability in real life context.
% Compared to recent popular domain knowledge reasoning datasets, the Detective Reasoning Puzzle Benchmark primarily comprises many detective-related questions, incorporating an abundance of information pertaining to character roles, human behaviors, mental activities, and environment description.
% Solving these problems requires models to discover clues from details in the context, and reasoning based on the connection between clues and the questions.

% In addition, we propose the Self-Question Prompt Framework to bridge the gap in LLMs' ability to carry out informal reasoning. 
% To borrow the idea from the powerful informal reasoning ability of humans, we recruited 50 participants to tackle 20 questions each from the Detective Reasoning Puzzle Benchmark, leading to a detailed study of the reasoning processes of both humans and the model. 
% Most participants said they find the clues mainly based on intuition without deeper thinking during the test, which is a typically informal reasoning process that sidesteps logical thinking, and instead uses experience and common sense to unearth critical elements in the context, promoting deep reflection, ultimately resulting in a reasoned outcome.
% By mirroring human intuitive thinking, Self-Questioning is composed of four steps to improve the model's ability for informal reasoning. 
% The goals of these steps respectively are to find key elements, deeply investigate the connections between these elements, encourage the relationship between each element and the problem, and finally, require the model to reasonably answer the problem.

% Experimental results show that even the lowest score amongst participants~(46.6\%) significantly surpasses the best score from the LLMs questioned based on naive prompt~(16.0\%) within Detective Reasoning Puzzle Benchmark. 
% Compared to the reasoning-enhanced prompts proposed by other researchers, our proposed self-question prompt generated the greatest performance improvement for GPT-4~(an increase of 17.4\%).
% Although a self-question prompt is a better way to excite the model's potential in doing informal reasoning, there is still a huge gap between the SoTA LLMs performance~(33.4\%) with the average human participants~(74.2\%).

% In conclusion, our study makes several key contributions: 
% (1) To facilitate further detailed exploration into the informal reasoning abilities of large language models, we constructed Detective Reasoning Puzzle Benchmark, which is super challenging for LLMs but easy for humans, that includes 1,200 pieces of detective reasoning data. 
% (2) We designed a self-questioning prompt framework that can reliably induce the model to identify irrelevant information, draw the clue from the context, and perform reasoning based on the clues drawn from the details in the context. 
% (3) We collected actual human responses to the Detective Reasoning Puzzle Benchmark and carried out numerous experiments using LLMs. 
% Regarding these experimental outcomes, we conducted extensive analysis and discussion, which includes the gap between existing LLMs and humans in informal reasoning, the superiority of self-questioning prompts, and how LLMs can supplement informal reasoning abilities.



==> latex/01.Introduction.04.tex <==
在侦探工作中，侦探们经常面临海量的信息，但只有少数信息对解决案件至关重要。 
侦探往往会根据已有的信息进行非常深度的思考，从而发现真正有价值的信息，并用来解决问题。
随着大语言模型的输入长度越来越长，以及面对的任务越来越复杂，处理海量庞杂的信息，即Information Overload，是使用大语言模型一定会面对的挑战。
让大语言模型能像侦探一样从海量信息中提取出关键信息，进而发现解决问题的关键是一件非常必要的事情。

目前有许多Benchmark也涉及关键信息发现，如阅读理解(Reclor)、检索推理(HotPotQA)、事实检验(FEVER)。
这些Benchmark中的关键信息和问题之间都有着非常明显的关联，往往可以用关键字或者字符匹配便能定位。
而在面对真正的Information Overload场景时，关键信息并不是很容易获得，这是是需要基于对于环境和问题具有深度理解才能捕获的。
如图~\ref{fig:intro}所示，只有考虑到“温度差和湿度可能会使玻璃起雾”，才能反推到现关键信息是能够体现温度和湿度的描述。



为了量化模型对于像侦探一样从庞杂的信息中定位关键信息，并根据关键信息回答问题的能力，我们设计了Detective Reasoning Benchmark。
该基准借鉴了众多公开的侦探推理谜题，通过复杂的情景、情节和人物设定，构建了一个充满挑战的推理环境。
在这个环境中，许多信息与问题的关联非常深层，另外还有许多误导性的信息，只有深入分析这些信息背后的原理，以及信息之间的联系，才能发现真正重要的因素并解开谜题。

Detective Reasoning Benchmark本身包含了题目、问题、四个选项、标准答案和解释。
其中，考虑到过程监督的重要性，Detective Reasoning Benchmark为过程提供了监督标签，基准中的每个问题都提供了详细推理过程的解释。
为了确保推理过程的逻辑性和系统性，我们将这些推理过程构建成了一个名为clue graph的结构。
如图~\ref{fig:intro}中的推理过程所示，clue graph包含了从与题目中直接能找到的和问题有关的信息出发，逐步通过推理以及信息关联揭示新的线索，并最终指向答案。


针对Detective Reasoning Benchmark我们同时要求人类受试者和大语言模型进行了两块实验——要求模型输出关键信息、以及输出认为最合理的答案。
我们发现在这两块实验中，人类的表现都要远高于SoTA的LLM。
大多数的语言模型，即便是那些能够在其他Benchmark上定位到关键信息的模型，也难以在Detective Reasoning上找到关键信息。
而在将关键信息作为context输入模型后，模型的推理表现能有大幅度提升。
这一来说明了Detective Benchmark的合理性和Clue graph的有效性，二来也说明大多数模型无法定位关键信息。

为了增强模型在面对Information Overload场景下的推理能力。
我们提出了一种名为Self-Question Prompt和Self-Question Finetune的两种baseline。
Self-Question Prompt旨在提升现有大型语言模型在面对Information Overload场景下的Zero-Shot Reasoning能力。
该方法通过引导模型先全面思考所有可能的线索，然后随意地进行推理，最后总结和问题相关的内容并进行提炼，最终提升回答问题的Performance。
Self-Question Finetune通过合理地利用标注了推理过程的benchmark，或者通过答案合理地诱导出推理过程来构造满足Self-Question Prompt的数据，从而有效增强模型面对Information Overload场景时的发现关键信息，并进行多跳推理的能力。
当直接使用Self-Question Prompt时，与其他旨在提升模型性能的提示方法相比，能够提高模型在面对Information Overload场景下的关键信息发现以及问题解决的效果。
而当我们使用了Detective Reasoning Benchmark来进行Self-Question Prompt时，大模型不仅在Detective Reasoning Benchmark上有了显著的提升，还在其他的信息挖掘、多跳推理的benchmark上有了明显的效果提升。


总结本研究的贡献如下：
\begin{enumerate}
    \item 我们提出了“侦探式推理基准”，为评估模型的关键信息发现和推理能力提供了新的标准。
    \item 我们开发了“自问式提示”方法，显著提升了模型在零样本推理场景下的性能。
    \item 我们基于“侦探式推理基准”和“自问式提示”，探索了一种有效的模型微调方法，以增强模型的特定能力。
    \item 我们通过广泛的实验验证了现有模型在发现关键信息和进行深层次推理方面的局限性，并展示了经过精心设计的微调后，模型在这些方面的表现有了显著提升。
\end{enumerate}


\begin{figure}[t]
    \centering
    \resizebox{0.9\columnwidth}{!}{
    \includegraphics{./figures/introduction.pdf}
    }
    \caption{A real response from GPT-4.
    Despite employing thorough prompting, GPT-4 continues to exhibit a deficiency in understanding real-life scenarios.}
    \label{fig:intro}
    \vspace{-5mm}
\end{figure}

==> latex/01.Introduction.05.tex <==

% 在信息量爆炸的今天，人们在做决策时常常被过多的信息所淹没，这些信息跟所需要解决的问题之间存在着怎样的联系谁也不清楚，因此最好的决策需要全面地考虑海量的信息中的关键内容常常令人头痛，这种现象被称为Information Overload。
% 这些海量的信息都和需要做的决策有着似有若无的联系，而有经验的人，如面对刑侦案件时的侦探，能够对所有必要的信息进行深入思考，发现解决问题最关键的信息，然后深入挖掘这些关键信息并最终解决任务。
% 随着大语言模型的输入长度越来越大，面对的任务越来越复杂，我们也会好奇这些LLM在面对Information Overload场景下的表现会如何，以及能否对他们进行有效地增强。

% 大型语言模型凭借其出色的上下文理解和问题解决能力，成为人们处理复杂任务和繁杂信息的重要工具。
% 随着这些模型能力越来越强，人们越来越依赖大模型能够解决自己生活中所面对的Information Overload问题。

% Information Overload, 在信息量爆炸的今天，人们在做决策时常常被过多的数据和信息所淹没
% 因此，研究大型语言模型如何在Information Overload的情景下识别关键信息，并据此有效解决问题，具有重要的学术和应用价值。

在当今信息爆炸的时代背景下，决策过程经常因为Information Overload而受到影响，即决策者在面对与问题相关性不明的海量信息时感到困惑。
经验丰富的专业人士，比如侦探，在面对案件时会先深入分析所有的关键信息，识别出解决问题的核心线索，并进一步挖掘这些关键信息以达成任务目标。
随着大型语言模型（LLM）处理的输入长度和任务复杂度的不断增加，大模型作为Agent Core时常也会面对着Information Overload问题。
因此，探索这些模型在处理大量、复杂信息时的效能，对于提高它们的实用性和决策支持能力具有重要意义。

面对Information Overload场景解决问题的关键在于能否发现关键信息，以及能否根据关键信息进行深入推理。
众多现有的基准测试，如阅读理解（Reclor）、检索推理（HotPotQA）、事实核查（FEVER）等，都涉及到关键信息发现和多跳推理的结合。
但在这些测试中，一些Benchmark的关键信息与问题通常存在直接的联系，可通过关键词或字符匹配等方式进行定位。
然而，在现实世界的Information Overload场景中，要获取关键信息并不总是那么直截了当，这往往需要对问题背景中的所有信息都先进行深入的理解和推理，然后才能发现重要的线索。
如图~\ref{fig:intro}所示，只有在意识到温度和湿度变化可能导致玻璃起雾的情况下，我们才能推断出温度和湿度相关的信息对于能否看向玻璃外非常关键。

\begin{figure}[t]
    \centering
    \resizebox{\columnwidth}{!}{
    \includegraphics{./figures/introduction.pdf}
    }
    \caption{
    In the context of information overload, language models may produce outputs arbitrarily due to their inability to engage in deep contemplation.
    In contrast, individuals with experience, like detectives, deeply analyze and correlate all available information, thereby identifying pivotal clues that lead to the answer of the problem.    
    }
    \label{fig:intro}
    \vspace{-5mm}
\end{figure}

鉴于此，我们从侦探在面对复杂案件时展现出的深度推理和关键信息挖掘能力中获得灵感。
为了定量评估大型语言模型在识别和利用复杂信息中的关键信息以解答问题的能力，我们设计了Detective Reasoning Benchmark。
该基准模拟了侦探推理谜题中的复杂场景、情节和角色设置，构建了一个挑战性极高的推理环境。
在这一环境中，信息与问题之间的联系往往非常微妙，并且伴随着大量的干扰信息。
只有通过对信息背后的逻辑和相互关系进行深入分析，仿佛侦探一般，我们才能揭示出解决问题的关键要素。

Detective Reasoning Benchmark包括题目、问题、四个选项、正确答案和解释，强调了过程监督的重要性。每个问题都附有详细的推理过程解释，我们将这些推理过程构建成了名为clue graph的结构，这些线索图从题目中直接相关的信息出发，通过逐步推理和信息关联揭示新的线索，最终指向答案。

在对人类受试者和大型语言模型进行的实验中，我们评估了它们发现关键信息和提供最合理答案的能力。我们发现，在这两项任务中，人类的表现都远远超过了最先进的大型语言模型。大多数模型，即使是那些在其他基准测试中能够定位关键信息的模型，在“侦探推理”任务上也难以找到关键信息。然而，当将关键信息作为上下文输入模型后，模型的推理表现得到了显著的提升。这一方面证明了Detective Reasoning Benchmark的合理性和“线索图”的有效性，另一方面也表明了大多数模型在定位关键信息方面的不足。

为了增强模型在面对Information Overload场景下的推理能力，我们提出了两种基线方法：Self-Question Prompt 和 Self-Question Finetune。
Self-Question Prompt旨在提升现有大型语言模型在零样本推理场景下的能力，通过引导模型全面考虑所有可能的线索，然后进行推理，最后总结与问题相关的内容并进行提炼。
而Self-Question Finetune则通过利用标注了推理过程的基准测试，或通过答案合理引导出推理过程来构造数据，从而有效增强模型在Information Overload场景下发现关键信息和进行多跳推理的能力。
当直接使用Self-Question Prompt时，与其他旨在提升模型性能的Prompt Engineer相比，能够提高模型在Information Overload场景下发现关键信息和解决问题的效果。
而当我们使用Detective Reasoning Benchmark的数据进行Self-Question Finetune时，大型模型不仅在Detective Reasoning Benchmark上取得了显著提升，而且在其他需要信息挖掘和多跳推理的基准测试上也取得了明显的效果提升。

总之，本研究的主要贡献包括：
1. 提出了Detective Reasoning Benchmark，为评估模型的关键信息发现和推理能力提供了新的标准。
2. 开发了“自我提问提示”方法，显著提升了模型在零样本推理场景下的性能。
3. 开发了Self-Question Finetune方法，探索了一种有效的模型微调方法，以增强模型的特定能力。
4. 通过广泛的实验，验证了现有模型在发现关键信息和进行深层次推理方面的局限性，并展示了经过精心设计的微调后，模型在这

==> latex/01.Introduction.06.tex <==
\begin{figure}[t]
    \centering
    \resizebox{0.8\columnwidth}{!}{
    \includegraphics{./figures/introduction.pdf}
    }
    \caption{
    In the context of information overload, language models may produce outputs arbitrarily due to their inability to engage in deep contemplation.
    In contrast, individuals with experience, like detectives, deeply analyze and correlate all available information, thereby identifying pivotal clues that lead to the answer of the problem.    
    }
    \label{fig:intro}
    \vspace{-5mm}
\end{figure}

In today's era of information explosion, decision-making processes are often impacted by Information Overload, where decision-makers feel overwhelmed when faced with vast amounts of information whose relevance to the problem at hand is unclear.


% 推理能力很重要
% 推理能力应当被应用在对于环境的理解上。
% 随着LLM的进化，LLM越来越面对真实需求，而人类往往会将推理和信息挖掘能力联合培养
% LLM这方面的能力值得评估

% The ability to perform reasoning and inference over a real environment is an important aspect of intelligence.
% 人类对于环境的理解可以拆分为——不断通过推理发现现实世界中大量信息中的关键内容，然后又根据关键内容进行推理最终影响自己的决策。
% 而如今，随着LLM的能力越来越强，我们不免也提出这样的疑问：LLM能否应对真实

% 随着LLM的能力越来越强，我们会期待LLM能够

真实环境中充斥着海量的信息，人们往往从自己的需求出发，发现关键信息，并从关键信息进行推理并最终得到决策。
发现信息、进行推理，这是一个联合的动态过程，是人类面向自己的需求，处理生活中海量信息的方式。
随着LLM的能力越来越强，我们会好奇在面对海量庞杂信息时，LLM是否也能够发现关键信息，并针对关键信息做出合理的推理，从而有效地解决问题。

% Experienced professionals, such as detectives, delve deep into analyzing all key information when facing a case, identify the core clues to solve the problem, and further excavate these key pieces of information to achieve the task objectives. As the input length and task complexity handled by Large Language Models (LLMs) continue to increase, these models, serving as Agent Cores, frequently encounter the issue of Information Overload. Therefore, exploring the efficacy of these models in handling large and complex information is crucial for enhancing their practicality and decision-support capabilities.

% The key to solving problems in Information Overload scenarios lies in the ability to discover key information and to reason deeply based on that information. 

Many existing benchmarks, such as reading comprehension~\cite{yu2020reclor}, retrieval reasoning~\cite{yang2018hotpotqa}, and fact verification~\cite{thorne2018fever}, involve a combination of key information discovery and multi-hop reasoning.
However, in these tests, the key information often has a direct connection to the question, which can be located through keyword or character matching. In contrast, in real-world Information Overload scenarios, obtaining key information is not always straightforward; it often requires a deep understanding and reasoning of all the information in the problem background before important clues can be discovered. As illustrated, only when we realize that changes in temperature and humidity can cause glass to fog, can we infer that information related to temperature and humidity is crucial for seeing through the glass.

Inspired by the depth of reasoning and key information mining capabilities demonstrated by detectives when facing complex cases, we designed the Detective Reasoning Benchmark to quantitatively assess the abilities of large language models to identify and utilize key information within complex information to answer questions. This benchmark simulates complex scenarios, plots, and character settings found in detective reasoning puzzles, creating a highly challenging reasoning environment. In this environment, the connections between information and questions are often subtle and accompanied by a large amount of distracting information. Only by analyzing the logic and relationships behind the information in depth, akin to a detective, can we reveal the key elements to solve the problem.

The Detective Reasoning Benchmark includes questions, options, correct answers, and explanations, emphasizing the importance of process supervision. Each question is accompanied by a detailed reasoning process explanation, and we constructed these reasoning processes into structures called clue graphs. These clue graphs start from information directly related to the question, reveal new clues through step-by-step reasoning and information association, and ultimately point to the answer.

In experiments conducted on human subjects and large language models, we assessed their abilities to discover key information and provide the most reasonable answers. We found that humans significantly outperformed the most advanced large language models in both tasks. Most models, even those capable of locating key information in other benchmarks, struggled with the ``detective reasoning'' task. However, when key information was provided as context input to the models, their reasoning performance significantly improved. This demonstrates the validity of the Detective Reasoning Benchmark and the effectiveness of ``clue graphs'' while also highlighting the deficiencies of most models in locating key information.

To enhance models' reasoning abilities in Information Overload scenarios, we proposed two baseline methods: Self-Question Prompt and Self-Question Finetune. The Self-Question Prompt aims to enhance the zero-shot reasoning capabilities of existing large language models by guiding them to consider all possible clues comprehensively, reason, and then summarize and refine content related to the question. The Self-Question Finetune method, by utilizing benchmarks annotated with reasoning processes or constructing data through reasonable guidance from answers, effectively enhances models' abilities to discover key information and perform multi-hop reasoning in Information Overload scenarios. Using the Self-Question Prompt directly improved models' effectiveness in discovering key information and solving problems in Information Overload scenarios compared to other prompts aimed at enhancing model performance. Moreover, when using data from the Detective Reasoning Benchmark for Self-Question Finetune, large models not only achieved significant improvements on the Detective Reasoning Benchmark but also showed noticeable performance enhancements on other benchmarks requiring information mining and multi-hop reasoning.

In summary, the main contributions of this study include:
\begin{enumerate}
    \item The introduction of the Detective Reasoning Benchmark, providing a new standard for assessing models' key information discovery and reasoning abilities.
    \item The development of the ``Self-Question Prompt'' method, significantly enhancing models' performance in zero-shot reasoning scenarios.
    \item The development of the Self-Question Finetune method, exploring an effective model fine-tuning approach to boost specific capabilities of models.
    \item Through extensive experiments, the limitations of existing models in discovering key information and conducting deep reasoning were verified, and it was shown that these limitations could be mitigated after using the Self-Question Prompt/Finetune methods.
\end{enumerate}

==> latex/01.Introduction.07.tex <==
\begin{figure}[t]
    \centering
    \resizebox{0.8\columnwidth}{!}{
    \includegraphics{./figures/introduction.pdf}
    }
    \caption{
    When facing overloaded information LLMs may produce outputs arbitrarily due to their inability to engage in deep contemplation.
    In contrast, humans who are experienced, like detectives, analyze and correlate all available information, thereby identifying pivotal clues that lead to the answer of the problem.    
    }
    \label{fig:intro}
    \vspace{-5mm}
\end{figure}


The essence of detective skills in handling vast amounts of information across various cases lies in the simultaneous processes of locating information and reasoning from it. 
Experienced detectives typically begin by identifying the information they require, isolating the crucial details, deducing insights from these details, and subsequently making informed decisions.
With the development of LLMs~\cite{openaichatgpt,touvron2023llama}, it raise a question that \textit{Do LLMs possess akin detective capabilities for identifying key information and employing it for effective reasoning and problem-solving when facing with complicated information?}

When facing overloaded information in real-cases, obtaining key information is not always straightforward.
This typically requires that models not only comprehend the question's meaning fully but also understand multiple approaches to solve it, allowing them to identify the specific information they need to search for.
For example, as shown in Figure~\ref{fig:intro}, only when we realize that changes in temperature and humidity can make glass foggy, can we figure out that details about temperature and humidity are key to seeing through the glass.
There has many existing benchmarks evaluate the model's joint abilities in information detection and multi-hop reasoning, such as reading comprehension~\cite{yu2020reclor,kazi2021uquad1,lu2022contextual}, retrieval reasoning~\cite{yang2018hotpotqa,chen2023benchmarking}, and fact verification~\cite{thorne2018fever,Thorne19FEVER2,Aly21Feverous}.
However, in these tests, the important information often links directly to the question, which can be found through searching for specific keywords or characters.


Inspired by the combined clues mining and reasoning done by detectives when facing huge amount of implicit information, we designed the \textbf{DetectBench}.
This benchmark includes 3,928 questions, with each question pair with a paragraph that averages 190 tokens, to measure how well models in finding and reasoning from key information in complex texts to answer questions.
DetectBench mimics the intricate stories, situations, and character interactions found in detective puzzles, offering a challenging test of reasoning.
We transformed original detective puzzles into multiple-choice question\&answer benchmark consists of context, question, options, answer, and an explanation of the answer.
Each question comes with a thorough explanation of how to arrive at the answer, using what we call ``Clue Graphs'', as seen at the bottom of Figure~\ref{fig:intro}.
These graphs start with important information that exact matches to the text in context, then step by step, they connect new clues through reasoning and linking information, leading directly to the answer.

% DetectBench containing 3928 questions with an average paragraph length of 190 tokens, to quantitatively assess the abilities of LLMs to identify and utilize key information within complex information to answer questions.
% This benchmark simulates complex scenarios, plots, and character settings found in detective reasoning puzzles, creating a highly challenging reasoning environment.
% We rewrite the raw detective reasoning puzzles into seperated context, question, options, answer and explanation to answer.
% Each question is accompanied by a detailed reasoning process explanation, and we constructed these reasoning processes into structures called ``Clue Graphs'' as shown in the below of Fig.~\ref{fig:intro}.
% These clue graphs start from key information which can be exact matched to the question, reveal new clues through step-by-step reasoning and information association, and ultimately point to the answer.


% In this environment, the connections between information and questions are often subtle and accompanied by a large amount of distracting information.
% Only by analyzing the logic and relationships behind the information in depth, akin to a detective, can we reveal the key elements to solve the problem.



In experiments conducted on human participants and LLMs, we assessed their abilities to discover key information and provide the most reasonable answers.
We found that humans significantly outperformed the most advanced LLMs in both tasks.
Most models, even those capable of locating key information in other information retrieving benchmarks, struggled with the detective reasoning task.
However, when key information is provided to the models as contextual input, their reasoning performance improves significantly.
This demonstrates the effectiveness of the DetectBench and emphasizes the fact that finding needle in a hay stack is critical to problem solving.

To jointly enhance model's key information detection ablities and reasoning abilities, we proposed two baseline methods: Self-Question Prompt and Self-Question Finetune.
The Self-Question Prompt aims to enhance the zero-shot reasoning capabilities of existing LLMs by guiding them to consider all possible clues comprehensively, reason, and then summarize and refine content related to the question.
The Self-Question Finetune, by utilizing benchmarks annotated with reasoning processes or constructing data through reasonable guidance from answers, effectively enhances model's abilities to discover key information and perform multi-hop reasoning.

Using the Self-Question Prompt directly improved model's effectiveness in discovering key information and solving problems compared to other prompt engineers.
Moreover, when using data from the DetectBench for Self-Question Finetune, LLMs not only achieved significant improvements on the DetectBench but also showed noticeable performance enhancements on other benchmarks requiring information mining and reasoning.

In summary, the main contributions of this study include:
\begin{enumerate}
    \item The introduction of the DetectBench, providing a new standard for assessing model's key information detection and reasoning abilities.
    \item The development of the Self-Question Prompt and Self-Question Finetune method, significantly enhancing model's joint performance in information detection and reasoning abilities.
    \item Through extensive experiments, the limitations of existing models in discovering key information and conducting deep reasoning are verified, and it was shown that these limitations could be mitigated after using the Self-Question Prompt/Finetune methods.
\end{enumerate}

==> latex/01.Introduction.08.tex <==
\begin{figure}[t]
    \centering
    \resizebox{0.8\columnwidth}{!}{
    \includegraphics{./figures/introduction.pdf}
    }
    \caption{
    When facing overloaded information LLMs may produce outputs arbitrarily due to their inability to engage in deep contemplation.
    In contrast, humans who are experienced, like detectives, analyze and correlate all available information, thereby identifying pivotal clues that lead to the answer of the problem.    
    }
    \label{fig:intro}
    \vspace{-5mm}
\end{figure}


% The essence of detective skills in handling vast amounts of information across various cases lies in the simultaneous processes of locating information and reasoning from it. 
% Experienced detectives typically begin by identifying the information they require, isolating the crucial details, deducing insights from these details, and subsequently making informed decisions.
% With the development of LLMs~\cite{openaichatgpt,touvron2023llama}, it raise a question that \textit{Do LLMs possess akin detective capabilities for identifying key information and employing it for effective reasoning and problem-solving when facing with complicated information?}

When handling vast amounts of information across various cases, experienced detectives typically engage in a continuous process of discovering clues, conducting reasoning, updating clues and updating reasoning.
This ability to combine clue detection and reasoning is a critical aspect of detective skills.
\red{It is only when the key clues are found that effective reasoning can be carried out to solve the problem.}
As the LLM evolves, user often inject complex, massive amounts of reference to it when solving problems.
This raises a question: \textit{when faced with overloaded information, does the LLM also possess detective skills to recognize clues and use it to reason effectively and solve problems?}


Clues, often concealed within seemingly unrelated and dispersed information, is seldom straightforward in real-cases. 
This necessitates models capable of discerning the essences and reasoning from them.
For example, as shown in Figure~\ref{fig:intro}, only when we realize that changes in temperature and humidity can make glass foggy, can we figure out that details about temperature and humidity are key to seeing through the glass.
There has many existing tasks evaluate the model's joint abilities in clues detection and reasoning, such as reading comprehension~\cite{yu2020reclor,kazi2021uquad1,lu2022contextual}, retrieval reasoning~\cite{yang2018hotpotqa,chen2023benchmarking}, and fact verification~\cite{thorne2018fever,Thorne19FEVER2,Aly21Feverous}.
However, for the existing benchmarks in these tasks, important information is clustered together and often linked directly to questions that can be found by keywords.


% Inspired by the combined clues detection and reasoning done by detectives when facing huge amount of implicit information, we propose \textbf{DetectBench}.
% This benchmark includes 3,928 questions, with each question pair with a paragraph that averages 190 tokens.
% to measure how well models in finding and reasoning from clues in complex context to answer questions，DetectBench具有以下特点：
% 1.和解决问题相关的线索没有直接出现在context中。
% 2.需要对context中的multiple clues进行组合推理才能得到更加关键的clues。 
% 3.context中还存在着大量的误导信息和无关信息。
Drawing inspiration from the detective's process of detecting and reasoning from a vast array of implicit information, we propose a multiple-choice question answering benchmark called \textbf{DetectBench}.
This benchmark comprises 3,928 questions, each paired with a paragraph averaging 190 tokens.
The purpose of DetectBench is to evaluate the proficiency of models in identifying and reasoning from clues within a complex context to answer questions.
The characteristics of DetectBench include:
1. Clues related to problem-solving do not directly appear within the context.
2. It necessitates the combination of multiple clues within the context to derive more critical clues.
3. The context contains a significant amount of misleading and irrelevant information.


% 我们收集了开源平台的大量detective puzzles, and rewrite the original detective puzzles into DetectBench consists of context, question, options, answer, and an explanation of the answer.
% The context in DetectBench mimics the intricate stories, situations, and character interactions found in detective puzzles.
% Each context pair with a question, options and answer, together they offer a challenging test of clues detection and reasoning.
% Each question comes with a thorough explanation of how to arrive at the answer, using what we call ``Clue Graphs'', as seen at the bottom of Figure~\ref{fig:intro}.
% These graphs start with text that exact matches in context to the basic clues, then step by step connect clues into new clues, leading directly to the answer.


We collect a large number of detective puzzles from open-source platforms and rewrit them into DetectBench, which consists of context, question, options, answer, and an explanation of the answer.
The context in DetectBench mimics the intricate stories, situations, and character interactions found in detective puzzles.
Each context pair includes a question, options, and an answer, providing a challenging test of the model's ability to detect and reason with clues.
Each question is accompanied by an explanation of how to arrive at the answer, utilising ``Clue Graphs'' as shown at the bottom of Figure~\ref{fig:intro}.
These graphs begin with text that exactly matches the basic clues in context, and then gradually connect the clues into new ones, leading directly to the answer.

In experiments conducted on human participants and LLMs, we assessed their abilities to clue detection and accuracy in answer questions.
Our findings indicate that humans significantly outperformed the most advanced LLMs in both tasks, suggesting that most LLMs have poorer detective skills than the average person.
We also found that performance in clue detection correlates with performance in answering questions. 
This demonstrates the effectiveness of the annotation in DetectBench and emphasizes the importance of detecting clues before reasoning.

To enhance model's detective skills, we proposed a baseline method to jointly enhance model's clue detection ablities and reasoning abilities: Detective Thinking.
Since experienced detective are doing clues detection and reasoning combinedly，Detective Thinking enhance the detective skills of existing LLMs by guiding them to consider all possible clues comprehensively, reason, and then summarize content related to the question.
Using the Detective Thinking improved model's performance in both clues detection and reasoning, but the performance is still greatly leg behind human participants. 

% Moreover, when using data from the DetectBench for Detective Thinking Finetune, LLMs not only achieved significant improvements on the DetectBench but also showed noticeable performance enhancements on other benchmarks requiring information mining and reasoning.

% The Detective Thinking Prompt aims to enhance the zero-shot detective skills of existing LLMs by guiding them to consider all possible clues comprehensively, reason, and then summarize content related to the question.
% The Detective Thinking Finetune, by finetuning on the benchmarks annotated with reasoning processes or constructing data through reasonable guidance from answers, effectively enhances model's abilities in clue detection and reasoning.


In summary, the main contributions of this study include:
\begin{enumerate}
    \item The introduction of the DetectBench, providing a new standard for assessing model's key information detection and reasoning abilities.
    \item The development of the Detective Thinking Prompt and Detective Thinking Finetune method, significantly enhancing model's joint performance in information detection and reasoning abilities.
    \item Through extensive experiments, the limitations of existing models in discovering key information and conducting deep reasoning are verified, and it was shown that these limitations could be mitigated after using the Detective Thinking Prompt/Finetune methods.
\end{enumerate}

==> latex/02.RelatedWork.01.tex <==




\subsection{Informal Reasoning}
% 当人类进行直觉推理和经验推理时，他们的大脑会使用两种不同的思维方式：formal and informal reasoning~\cite{huang2022towards}。
% informal reasoning是一种快速、自动的思维方式，不需要经过深思熟虑，而是基于以往的经验和感觉。
% formal reasoning是一种更加缓慢、有意识的思维方式，需要深思熟虑和逻辑推理~\cite{evans2010intuition}。
% 这两个思维过程共同组成了双推理理论，研究学者普遍认为直觉通常是快速的、提供信心感、可以反映大量的信息处理，并且在基于相关经验学习时最有可能提供准确的判断~\cite{,kannengiesser2019design,doherty2020believing,grayot2020dual,sloman2021cognitive}。
% 与推理不同，直觉是低效的，并且不会竞争中央工作记忆资源。它提供默认响应，可以通过高效、反思性的推理进行干预。然而，在关于推理和决策制定的心理学文献中，直觉也被指责为一系列认知偏差的原因~\cite{ellis2018so,khatri2000role}。

When humans engage in intuitive reasoning and experiential reasoning, their brains use two different modes of thinking: formal and informal reasoning~\cite{huang2022towards}.
Informal reasoning is a fast, automatic mode of thinking that does not require deep thought but is based on past experience and feelings. 
Formal reasoning is a slower, more conscious mode of thinking that requires deep thought and logical reasoning~\cite{evans2010intuition}.
These two modes of thinking together make up the dual-reasoning theory, and researchers generally believe that informal reasoning is usually fast, provides a sense of confidence, reflects a large amount of information processing, and is most likely to provide accurate judgments when based on relevant experience learning~\cite{kannengiesser2019design,doherty2020believing,grayot2020dual,sloman2021cognitive}.
Unlike formal reasoning, informal reasoning is inefficient and does not compete for central working memory resources.
It provides default responses that can be intervened by efficient, reflective reasoning. However, in the psychological literature on reasoning and decision-making, intuition has also been blamed for a series of cognitive biases~\cite{ellis2018so,khatri2000role}.


Although informal reasoning is often used by humans in their daily lives, it has received little attention in the machine learning community in recent years~\cite{huang2022towards}.
Traditional common sense reasoning benchmarks, such as HellaSwag~\cite{zellers2019hellaswag} and WinoGrande~\cite{sakaguchi2021winogrande}, have been designed in a way that does not reflect human usage habits.
They directly construct question-answer pairs about common sense knowledge for evaluation, greatly reducing the difficulty to the baby-level~\cite{hendrycks2021measuring}.
Besides, the greatest need for humans to rely on informal reasoning is to quickly extract important information from a large amount of information in real-life scenarios~\cite{huang2022towards}.
The most nearly proposed informal reasoning dataset is True Detective~\cite{del2023true}, which is also a detective-related dataset without open source until now and consists of only 191 questions without manual annotation.
Our Detective Reasoning Puzzle Benchmark contains 1,200 manual annotated detective reasoning-related puzzles, which involve a large number of life-like scenarios in free-text form.
As shown in Figure~\ref{fig:relatedwork}, Detective Reasoning Puzzle is more challenging for language models than previous well-known benchmarks.
Solving these puzzles truly tests the model’s human-like informal reasoning ability.
The introduction of Detective Reasoning Puzzle has bridged the gap between existing informal reasoning benchmarks and the need for humans to apply this ability.


\subsection{Prompt Engineering}
The ability of generative language models is largely influenced by the prompt words~\cite{liu2023pre}. 
After the introduction of LLMs, scholars have continuously improved the paradigm of prompt words to enhance the model’s ability in various tasks~\cite{mialon2023augmented}.
These improvements mainly focus on enhancing the language model’s ability in formal reasoning and can be roughly divided into two types: Chain-of-Thought and Ensemble.
People generally use Chain-of-Thought (CoT) to evoke the inherent step-by-step reasoning ability of large language models (LLMs), enabling them to formulate intermediate reasoning chains that are essential for solving problems~\cite{brown2020language}.
Ensemble mainly allows the model to generate multiple answers and select the most likely answer based on the answers~\cite{fu2022complexity,wang2022self}.
Researches results show that many current CoT and model ensemble schemes have significantly improved the formal reasoning ability of language models~\cite{wei2022chain,zhang2022automatic,wang2023plan}.

Considering that there has been no challenging informal reasoning benchmark proposed in the past, this has restricted scholars from improving the informal reasoning ability of models.
Self-Question mainly draws the ideas from CoT.
Compared with simply modifying existing CoT schemes to enhance the model’s informal reasoning ability, Self-Question restores the intermediate process of human intuitive reasoning, which is more in line with the application scenarios of informal reasoning and can obtain better answers.

% 生成式语言模型的能力很大程度上受到提示词的影响~\cite{liu2023pre}。
% 在大模型提出后，不断有学者改进提示词的范式，以提高模型在各方面任务的能力~\cite{mialon2023augmented}。
% 这类改进主要聚焦于提升语言模型在正式推理上的能力，大致可以分为Chain-of-Thought和Ensemble两种类型。
% 人们普遍利用Chain-of-Thought（CoT）来唤起大型语言模型（LLM）内在的逐步推理能力，使其能够制定对解决问题至关重要的中间推理链~\cite{brown2020language}。
% 而Ensemble主要是让模型生成多个回答，并根据回答选择最可能的答案~\cite{fu2022complexity,wang2022self}。
% 研究结果表明，目前的诸多CoT和模型ensemble的方案都对于增强语言模型的formal reasoning能力有显著提高~\cite{wei2022chain,zhang2022automatic,wang2023plan}。

% 考虑到以往并没有有挑战性的informal reasoning benchmark的提出，因此制约了学者提出新的改进模型的informal reasoning ability的方案。
% Self-Question主要借鉴了CoT的思路，相较于将已有的CoT方案进行简单修改来增强模型的informal reasoning ability，Self-Question还原了人类进行直觉推理的中间流程，更符合informal reasoning的应用场景，从而可以得到更好的回答。



% 已有的CoT方案都可以做些简单的修改用来增强模型的Informal reasoning能力，

% 但这些方法都没有抓住人类能够进行informal reasoning的核心。
% 其中Plan-and-Solve CoT提出了整理

% Recent literature has reported the prevalent utilization of Compositional Tasks (CoT) to evoke the stepwise reasoning skills inherent within Large Language Models (LLMs) (Wei et al., 2022b).
% Practical application of CoT methodologies provokes the LLM's intrinsic capacity to formulate intermediate reasoning chains pivotal to problem resolution.
% Empirical findings underline the efficacious employment of LLM's in CoT reasoning within two fundamental operational paradigms, namely Zero-Shot-CoT (Kojima et al., 2022) and Few-Shot-CoT (Wei et al., 2022b; Zhang et al., 2022).

% In the context of Zero-Shot-CoT paradigm, Kojima et al. (2022) fostered an impromptu thought process within the LLMs by appending a prompt such as "Let's think step by step" subsequent to the test question, thereby instigating CoT reasoning. The Few-Shot-CoT paradigm operates by integrating several sequential reasoning demonstrations as inferential prerequisites. Each demonstration encompasses a query and a corresponding reasoning trajectory that culminates in the final verdict. The establishment of these demonstrations is commonly reliant on either meticulous manual construction or automated generation, thereby giving rise to the respective Manual-CoT (Wei et al., 2022b) and Auto-CoT (Zhang et al., 2022) methodologies.

% Owing to the provision of potent demonstrations, the Few-Shot-CoT paradigm typically outperforms the Zero-Shot-CoT paradigm and has consequently garnered significant scholarly attention. Consequently, the majority of the recent investigative endeavors have been primarily geared towards enhancing the Few-Shot-CoT paradigm. These diverse studies can primarily be classified into two core investigational strands: (i) refining the demonstrations; (ii) augmenting the reasoning chains. Table 1 represents a comparative analysis of typical CoT methodologies.

% Although informal reasoning is used by human in their every life, it is not well studied after the published of MMLU~\cite{hendrycks2021measuring}.
% MMLU propose that the existing common sense reasoning dataset, which is a simple and direct form of informal reasoning, are too easy that even the baby can achieve high score.
% After the MMLU, although there are much more powerful language models, like ChatGPT, Claude or Bard, have been proposed, the benchmark of testing models' informal reasoning ability is greatly lagged behind.
% Besides, the traditional informal reasoning benchmark only focus on the very simple and direct common sense question



% 尽管informal reasoning在人类日常生活中经常被使用，但是近几年的机器学术界却很少关注informal reasoning。
% 传统的common sense reasoning benchmark以一种不符合人类使用习惯的方法被设计出来，如HellaSwag~\cite{zellers2019hellaswag}、WinoGrande~\cite{sakaguchi2021winogrande}等，他们直接将常识知识构成问答对用于评估，从而大大地降低了模型回答的难度。
% 我们认为这没有体现出人类依赖于informal reasoning最大的需求，即在真实的生活场景中面对大量信息能够根据直觉和经验快速抽取出重要信息的能力。
% 我们构建的Detective Reasoning Puzzle Benchmark包含了大量的侦探推理相关的puzzle，这一类puzzle涉及了大量的生活化场景，解决这类的题目真正地考验了模型的类人informal reasoning ability.
% Detective Reasoning Puzzle的提出了弥补了已有informal reasoning benchmark和人类应用这个能力的需求之间的差距。
% 并且如图~\ref{fig:relatedwork}所示，Detective Reasoning Puzzle相较于以往最有名的benchmark而言，对于语言模型更具有挑战性。

% 尽管人类在日常生活中使用非正式推理，但在MMLU~\cite{hendrycks2021measuring}发表后，它并未得到充分研究。MMLU提出，现有的常识推理数据集，即一种简单直接的非正式推理形式，过于简单，甚至婴儿都能取得高分。在MMLU之后，尽管出现了更强大的语言模型，如ChatGPT、Claude或Bard，但测试模型非正式推理能力的基准大大落后。此外，传统的非正式推理基准仅关注非常简单直接的常识问题。



% Informal reasoning is a ability that 

% The well-established complexity of reasoning problems presents considerable challenges for Natural Language Processing (NLP) models. These problems encompass diverse domains such as mathematical reasoning, typified by conceptual understanding of mathematics, computational skills and multi-step reasoning (Cobbe et al., 2021; Patel et al., 2021; Ling et al., 2017; Koncel-Kedziorski et al., 2016), commonsense reasoning, which necessitates judgment based on commonsense knowledge (Talmor et al., 2019; Geva et al., 2021), and logical reasoning that obligates the symbolic manipulation through implementing formal logical norms (Wei et al., 2022b).

% Prior to the emergence of Large Language Models (LLMs), Talmor et al. (2019) induced training of the NLP model employing explanations produced via the fine-tuned Generative Pretrained Transformer (GPT) model. Subsequent research evidenced enhanced performance by the trained model in relation to commonsense Question-Answering (QA), problems. Hendrycks et al. (2021) endeavored to refine pre-trained language models utilizing labeled rationale, but the resulting fine-tuned models were deficient in generating high-quality reasoning steps.

% Recent research by Wei et al. (2022a) indicates that Large Language Models (LLMs) exhibit a robust reasoning capacity, on being scaled up to tens of billions of parameters, as exemplified in GPT-3 (Brown et al., 2020) and PaLM (Chowdhery et al., 2022). Although significant performance in diverse NLP tasks has been observed with these LLMs utilising a few demonstration exemplars, their execution remains subpar in problems necessitating multi-step reasoning. This shortcoming may be ascribed to the insufficient quantity of exemplars provisioned, which undermines the full potential of the LLMs' capabilities.




==> latex/02.RelatedWork.02.tex <==



\subsection{Information Retrieval}
现在有许多工作都会涉及Information Retrieval，从传统的专门的Information Extraction任务，再到现在以解决其他任务为导向的Information Detection。
这些需要被找到的信息可能存在于大量的文本之中，这样的Information Retrieval的难点在于如何从大量的文本中找到关键信息。
如HotPotQA需要从段落中找到和问题相关的信息来辅助回答、FEVER需要定位evidence来support or regute a claim、RECLOR需要对原文进行划线来判断哪些内容可以用于回答query。

Detective Reasoning Benchmark中的Key Information Detection有别于这些，它既存在于大量的文本之中，但同时又需要对query或context能有深度地理解，才能有效地发现关键信息。


\subsection{Commonsense Reasoning}

常识推理已经在多个研究中被研究过。目前主要分为：单跳推理、多跳推理、uncommon but possible reasoning。
单跳推理的数据集，如HellaSwag和WinoGrande都涉及故事续写类型的常识推理，这些数据集的难点一般会在选项设置上，以及可能会针对某个模型进行对抗性选项设置。
多跳推理benchmark，如StrategyQA，数据集中一般会标注推理过程，但这些数据集的问题非常简短，重点在于模型根据给定的问题能否进行多跳推理。
Uncommon but possible reasoning，如α-NLG、d-NLI、UnCommonsense Reasoning，这些数据集很多都从已有的数据集出发，选择一个概率最低的选项作为正确答案，并为这个选项补全解释。


Detective Reasoning Benchmark属于uncommon but possible multi-hop reasoning，因为Detective Reasoning Benchmark的重点之一是在于从哪些线索开始进行推理，重点之二在于如何进行多跳推理。
Detective Reasoning Benchmark的推理往往从一些看似不起眼的点开始，然后慢慢深挖，才能发现一条非常完整的推理到正确答案的路径

\input{tables/tab_dataset_comparsion}

% \subsection{Reasoning Enhanced Prompt Engineer}
% 主要要写和d-NLI、αNLG、UnCommonsense Reasoning、StrategyQA、HellaSwag、WinoGrande的不同
% 主要要写和CoT、ToT、GoT、ReAct、Reflexion的不同
% xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, xxxxx, 

% αNLG (Bhagavatula et al., 2020) is the most closely related task to UNCOMMONSENSE: both require generating explanations to bridge contexts and outcomes (except αNLG focuses on common, everyday scenarios). d-NLI (Rudinger et al., 2020) consider a related task of generating an explanation explanation that weakens an outcome. Additional works cover methods for generating explanations, e.g., Du et al. (2022), Zhou et al. (2021), Wang et al. (2019), Zhang et al. (2020a), inter alia. Reasoning about uncommon but possible scenarios has been studied in other settings. Arnaout et al. (2022) propose a method for identifying informative negations about everyday concepts in large-scale commonsense knowledge bases. Tang et al. (2023) present a decoding method for producing less plausible explanations for everyday events. Collins et al. (2022) create a small-scale benchmark containing about 800 curated uncommon statements, along with explanations making sense of these statements. UNCOMMONSENSE differs in structure and focus from these prior works. Finally, TODAY (Feng et al., 2023) proposes a temporal reasoning task to study the order of two events. Atypical order of two events could be uncommon, and justifying the order is uncommonsense reasoning. Because UNCOMMONSENSE is not built from reversing the order of temporal events, it encompasses a different set of uncommon situations, including social reasoning, cultural reasoning, and physical reasoning. With each situation, UNCOMMONSENSE also contains more than one explanation, collected from both crowd workers and GPT-4. We summarize the differences between UNCOMMONSENSE and existing datasets in Figure 8.

==> latex/02.RelatedWork.03.tex <==

\input{tables/tab_dataset_comparsion}
\subsection{Information Retrieval}

% Information Retrieval is a critical component of many tasks, ranging from traditional Information Extraction tasks to Information Detection aimed at solving other specific tasks~\cite{zhu2023large,yang2022survey}. 

The purpose of Information Retrieval is to solve related task by identifying key information from vast amounts of reference, most challenge one can be lie into implicit key information identification~\cite{zhu2023large,yang2022survey}.
虽然传统的Information Retrieval Benchmark都将Information Extraction任务单独拎出来评估模型~\cite{martinez2020information}.
但最近 Many works has build benchmark for 端到端评估任务是否能被解决。
HotPotQA~\cite{yang2018hotpotqa} involves finding question-related information within paragraphs to assist in answering, FEVER~\cite{} requires locating evidence to support or refute a claim, and RECLOR~\cite{yu2020reclor} involves highlighting text to determine which content can answer a query.
However, 这些Benchmark的关键信息和问题之间的连接太过明显，这些Benchmark都可以通过字符串匹配定位到关键信息，而针对关键信息进行一两跳的推理就可以得到正确答案。

Key Information Detection within the Detective Reasoning Benchmark differs from these tasks in that it not only requires sifting through extensive text but also necessitates a deep understanding of the query or context to effectively uncover key information.

\subsection{Commonsense Reasoning}

Commonsense reasoning has been explored in multiple research studies, primarily categorized into single-hop reasoning, multi-hop reasoning, and uncommon but possible reasoning. 
Single-hop reasoning datasets, such as HellaSwag~\cite{zellers2019hellaswag} and WinoGrande~\cite{sakaguchi2021winogrande}, involve story continuation types of commonsense reasoning, where the challenge often lies in the setup of options and possibly in adversarial option settings targeted at specific models. 
Multi-hop reasoning benchmarks, like StrategyQA~\cite{geva2021did}, typically annotate the reasoning process, with the focus on whether models can perform multi-hop reasoning based on a given question. Uncommon but possible reasoning, as seen in datasets like α-NLG~\cite{bhagavatula2019aNLG}, d-NLI~\cite{rudinger2020bNLG}, and UnCommonsense Reasoning~\cite{zhao2023uncommonsense, arnaout2022uncommonsense}, often start from existing datasets, selecting the least probable option as the correct answer and providing an explanation for this choice.

The Detective Reasoning Benchmark falls into the category of uncommon but possible multi-hop reasoning. One of its key focuses is identifying the starting points for reasoning, with a second focus on how to conduct multi-hop reasoning. Reasoning in the Detective Reasoning Benchmark often starts from seemingly insignificant details, which, upon deeper exploration, reveal a comprehensive path to the correct answer.


==> latex/03.BenchmarkConstruction.01.tex <==


% In this section, we describe the construction details of our LSR-Benchmark.
% The dataset consists of 2,162 questions, and the construction process is composed of two main steps: data collection and data rewriting. 

\subsection{Data Collection} 

We construct Detective Reasoning Puzzle Benchmark based on openly available content online.
The goal is to collect free-text reasoning datasets that contain information about real-life scenarios.
So we collect detective reasoning puzzles which mainly encompass a wide range of real-life scenarios, characterized by their extensive involvement of commonsense, encyclopedic, and idiom knowledge.
Besides logically combining and reasoning between clues, these questions require models to possess a robust perception of real-life scenarios and a certain understanding of human behavior and psychology.
In this manner, models can effectively eliminate irrelevant information from questions and identify appropriate clues to solve problems.



\begin{figure}[t]
    \centering
    \resizebox{0.8\columnwidth}{!}{
    \includegraphics{figures/Example.pdf}
    }
    \caption{The example of the question in Detective Reasoning Puzzle Benchmark}
    \label{fig:example}
    \vspace{-5mm}
\end{figure}

\subsection{Data Preprocessing}

\subsubsection{Question Rewrite}

\subsubsection{Options Setting}

\subsubsection{Clue Graph Building}
To ensure the compatibility of the Detective Reasoning Puzzle Benchmark with diverse baselines, each question is represented in a JSON format, which comprises four elements: ``context'', ``question'', ``hint'', and ``analysis'' as shown in Fig.~\ref{fig:example}.

We elected to exclude questions incapable of being resolved solely through textual information, which demands visual or audio information to answer the question.
Besides, we also exclude questions that comprised of many numerous mathematical formulas. 
The reason behind this is the fact that these types of questions evaluated the formal reasoning capacity of the models, which does not align with the objective of the Detective Reasoning Puzzle Benchmark.
The examples of exactly what kind of questions are excluded are listed in Appendix.

% The original puzzle questions were often intermingled with the description of the story, we separate each puzzle's description into the ``context'' of the story and the ``question'' in order to provide a clearer presentation for each puzzle.
% Taking into consideration the significant improvement with the help of process supervision, we employed GPT-4 to generate the reasoning process for each question when given answer and the question. 
% The generated reasoning process underwent manual correction and was represented by ``hint'' field.
% Lastly, as the answer is often described into story style, which may incur confusion when doing verification, so we shorten the raw answer by deleting the story-telling content in it, and use ``answer'' field to denote it.

Online puzzles often intertwine the questions with the narrative's description.
We separate each puzzle's description into the ``context'' of the story and the ``question'' in order to provide a clearer presentation for each puzzle.
Acknowledging the marked improvement achieved through process supervision, we leveraged GPT-4 to generate a reasoning process for each question, given an answer and the question itself.
This generated reasoning process underwent manual check for correction and was denoted by a ``hint'' field, the detail about our human annotators and manual check are described in Appendix.
Notably, answers often adopt a narrative style, potentially leading to confusion during validation.
We hence shortened the unprocessed answer by eliminating its narrative elements, and the refined answers are indicated in the ``answer'' field.



In this way, we acquire 1,200 detective reasoning puzzle questions.
We randomly choose 33.4\%, 33.3\%, and 33.2\% of the puzzles to respectively form the training, validation, and test set.
The test set was handed to human participants, with an average of 2 human responses per puzzle without hint being recorded, serving as a means of assigning a level of difficulty to each test puzzle.
The detailed statistic information is listed in Tab~\ref{tab:statistic}.
% Given that the majority of language learning models (LLMs) allow a maximum input length of 2048, we have maintained that the sum of context length, question length and hint length for every question in the test set should not surpass this limit.

\begin{table}[t]
\centering
\begin{tabular}{ll}
\hline
Statistic & Number \\ \hline
Total questions & 1,200 \\
\hline
Training questions & 401 \\
Validation questions & 400 \\
Test questions & 399 \\
\ \ $*$ \textit{Simple Test question} & 223\\
\ \ $*$ \textit{Medium Test question} & 94\\
\ \ $*$ \textit{Hard Test question} & 82\\
\hline
Context Length (Average/Max) & 104.9 / 1379 \\
\ \ $*$ \textit{Test} & \ \ 97.6 / 387\\
Question Length (Average/Max) & \ \ 17.6 / 39 \\
\ \ $*$ \textit{Test} & \ \ 12.4 / 18\\
Hint Length (Average/Max) & \ \ 71.3 / 176 \\
\ \ $*$ \textit{Test} & \ \ 47.9 / 101\\
Analysis Length (Average/Max) & \ \ 84.2 / 960 \\
\ \ $*$ \textit{Test} & \ \ 66.3 / 176\\
\hline 
\end{tabular}
\caption{Key statistics for Detective Reasoning Puzzle Benchmark.
} 
\label{tab:statistic}
    \vspace{-5mm}
\end{table}

==> latex/03.BenchmarkConstruction.02.tex <==
\subsection{Data Collection} 

We construct Detective Reasoning Puzzle Benchmark based on openly available content online.
The goal is to collect free-text reasoning datasets that contain information about real-life scenarios.
So we collect detective reasoning puzzles which mainly encompass a wide range of real-life scenarios, characterized by their extensive involvement of commonsense, encyclopedic, and idiom knowledge.
Besides logically combining and reasoning between clues, these questions require models to possess a robust perception of real-life scenarios and a certain understanding of human behavior and psychology.
In this manner, models can effectively eliminate irrelevant information from questions and identify appropriate clues to solve problems.



\begin{figure}[t]
    \centering
    \resizebox{0.8\columnwidth}{!}{
    \includegraphics{figures/Example.pdf}
    }
    \caption{The example of the question in Detective Reasoning Puzzle Benchmark}
    \label{fig:example}
    \vspace{-5mm}
\end{figure}

\subsection{Data Preprocessing}

\subsubsection{Question Rewrite}

\subsubsection{Options Setting}

\subsubsection{Clue Graph Building}
To ensure the compatibility of the Detective Reasoning Puzzle Benchmark with diverse baselines, each question is represented in a JSON format, which comprises four elements: ``context'', ``question'', ``hint'', and ``analysis'' as shown in Fig.~\ref{fig:example}.

We elected to exclude questions incapable of being resolved solely through textual information, which demands visual or audio information to answer the question.
Besides, we also exclude questions that comprised of many numerous mathematical formulas. 
The reason behind this is the fact that these types of questions evaluated the formal reasoning capacity of the models, which does not align with the objective of the Detective Reasoning Puzzle Benchmark.
The examples of exactly what kind of questions are excluded are listed in Appendix.


Online puzzles often intertwine the questions with the narrative's description.
We separate each puzzle's description into the ``context'' of the story and the ``question'' in order to provide a clearer presentation for each puzzle.
Acknowledging the marked improvement achieved through process supervision, we leveraged GPT-4 to generate a reasoning process for each question, given an answer and the question itself.
This generated reasoning process underwent manual check for correction and was denoted by a ``hint'' field, the detail about our human annotators and manual check are described in Appendix.
Notably, answers often adopt a narrative style, potentially leading to confusion during validation.
We hence shortened the unprocessed answer by eliminating its narrative elements, and the refined answers are indicated in the ``answer'' field.



In this way, we acquire 1,200 detective reasoning puzzle questions.
We randomly choose 33.4\%, 33.3\%, and 33.2\% of the puzzles to respectively form the training, validation, and test set.
The test set was handed to human participants, with an average of 2 human responses per puzzle without hint being recorded, serving as a means of assigning a level of difficulty to each test puzzle.
The detailed statistic information is listed in Tab~\ref{tab:statistic}.

\begin{table}[t]
\centering
\begin{tabular}{ll}
\hline
Statistic & Number \\ \hline
Total questions & 1,200 \\
\hline
Training questions & 401 \\
Validation questions & 400 \\
Test questions & 399 \\
\ \ $*$ \textit{Simple Test question} & 223\\
\ \ $*$ \textit{Medium Test question} & 94\\
\ \ $*$ \textit{Hard Test question} & 82\\
\hline
Context Length (Average/Max) & 104.9 / 1379 \\
\ \ $*$ \textit{Test} & \ \ 97.6 / 387\\
Question Length (Average/Max) & \ \ 17.6 / 39 \\
\ \ $*$ \textit{Test} & \ \ 12.4 / 18\\
Hint Length (Average/Max) & \ \ 71.3 / 176 \\
\ \ $*$ \textit{Test} & \ \ 47.9 / 101\\
Analysis Length (Average/Max) & \ \ 84.2 / 960 \\
\ \ $*$ \textit{Test} & \ \ 66.3 / 176\\
\hline 
\end{tabular}
\caption{Key statistics for Detective Reasoning Puzzle Benchmark.
} 
\label{tab:statistic}
    \vspace{-5mm}
\end{table}

==> latex/03.BenchmarkConstruction.03.tex <==
\begin{figure*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \includegraphics{figures/Example_2.pdf}
    }
    \caption{The example of the question in Detective Reasoning Puzzle Benchmark}
    \label{fig:example}
    \vspace{-5mm}
\end{figure*}

\subsection{Data Collection} 

我们在网上公开内容的基础上构建了侦探推理谜题基准。
我们的目标是收集包含真实场景信息的自由文本推理数据集。
因此，我们收集的侦探推理谜题主要包括各种现实生活场景，其特点是广泛涉及常识、百科知识和成语知识。
这些问题除了需要对线索进行逻辑组合和推理外，还要求模型对现实场景有较强的感知能力，对人类的行为和心理有一定的了解。
这样，模型就能有效地排除问题中的无关信息，找出解决问题的适当线索。


\subsection{Data Preprocessing}
我们将Detective Reasoning Benchmark中的每个问题都处理成JSON格式表示。
如图~\ref{fig:example}所示，每道题主要包括五个元素：``Context''、 ``Question''、 ``Options''、 ``Answer''、 ``Clue Graph''。
具体而言，我们将原数据处理分为题目过滤、题目重写、人工校验三个步骤进行。其中，前两个过程主要是使用gpt-4-turbo-1106-preview进行，具体的prompt我们放在Appendix中。

\textbf{题目过滤}
为了使Detective Reasoning Benchmark能够聚焦``Daily Information Overload‘’, ``关键信息发现'', ``多跳推理''这三个点，我们对所有获得的题目进行了过滤。
对于侦探推理而言，答案和推理过程可能并非唯一，但我们仍然希望在我们benchmark中的题目包含尽可能少的不同推理方案，从而保证标注答案和推理的合理性与唯一性。
同时，我们希望Detective Reasoning Benchmark是面向通用领域的，所以不希望题目内包含太多符号推理或者需要领域知识的内容。

因此，我们将满足下面三个条件的问题全部从Detective Reasoning Benchmark中过滤。
1. 无法仅通过文本信息解决的问题，如需要视觉或听觉信息来回答。
2. 思维太过反逻辑、或者答案非常不合理
3. 需要大量数学公式、领域知识进行推理的问题。

\textbf{题目改写}
原题目可能会将问题和题干合在一起，而有些题目会直接告诉你答案，并问你推理过过程。
我们将题目进行改写，将问题的描述和问题的提问分开用``Context''和``Question''进行表示。
其次，我们根据原始的题目，将问题进行改写并将答案部分藏去，来构建选择题，并将选项用字段``Options''进行表示、答案用``Answer''进行表示。
最后，根据原始题目和答案，我们要求gpt-4-turbo-1106-preview来生成clue-graph，并要求模型从题目中原始的信息出发，不断对信息进行深入推理、总结、关联从而推理出新的线索，最终推理出答案。

\textbf{人工校验}
最后，我们使用了人工来校验所有经过gpt-4-turbo-1106-preview标注过的题目。
我们总共招募了5名标注者和作者一同进行标注任务，标注主要分为两种方式：
作者对所有题目进行粗筛，主要包含删除答案、选项构建不合理的，或者需要较大修改的题目。
对于被招募的标注者而言，他们需要对选项、答案进行略微的修改，使选项和答案构建的更加合理、自然。
我们将具体的标注要求和示例放在了Appendix中。


通过上述方式，我们获得了1200道侦探推理谜题。
我们随机选择其中的33.4\%、33.3\%和33.2\%分别组成训练集、验证集和测试集。
测试集由人类参与者参与，平均每道谜题记录2个无提示的人类回答，以此来为每道测试谜题分配难度等级。
详细的统计信息请见表~ref{tab:statistic}。



\input{tables/tab_dataset_statistic}

==> latex/03.BenchmarkConstruction.04.tex <==
Detective Reasoning Benchmark的重点是在于验证模型``面对Information Overload场景下的关键信息发现和多跳推理能力''，因此整个Benchmark的重点在于：
1. 问题需要有足够长、庞杂、且看似无关的信息描述
2. 解题过程需要包含从原始信息出发的多跳推理过程。
3. 需要能够客观、准确地对模型表现进行有效的评估。

网络公开的侦探推理谜题一般会将解题的关键信息藏于题目描述之中，并且发现这些关键信息需要能对所有可用的信息进行一定的深度推理才能发现。
而构建一套可用的LLM Evaluation Benchmark，我们首先需要对题目进行严格的质量审查和道德审查。
另外，我们还需要将解题的多跳推理过程标注出来，以方便进行过程监督。
同时，我们参考目前许多工作都在使用的选择问答的评估形式，希望将Detective Reasonging Benchmark构建成选择题的形式来增加评估的客观性、可量化性，以及降低评估的开销。

在Detective Reasoning Benchmark中，每个题目均以JSON格式组织，包含五个主要元素：
``Context''、``Question''、``Options''、``Answer''及``Clue Graph''。
数据处理分为题目过滤、题目改写及人工校验三个阶段，前两阶段主要借助gpt-4-turbo-1106-preview模型完成，具体的prompt细节见附录。

\textbf{题目过滤}
为确保侦探推理基准聚焦于``信息过载''、``关键信息发现''和``多跳推理''，我们对题目进行了筛选。
考虑到侦探推理题的答案和推理路径可能多样，我们仍力求每个题目的推理方案尽可能单一，以保证答案和推理过程的合理性与唯一性。
同时，为保证基准的通用性，我们排除了过分依赖符号逻辑或专业领域知识的题目。
具体而言，我们排除了以下三类题目：1. 需要视觉或听觉信息辅助的题目；2. 过于反逻辑或答案不合理或太过多样的题目；3. 需要大量符号推理或领域知识的题目。

\textbf{题目改写}
原始题目可能混合了问题描述和问题本身，有些甚至直接给出答案，我们需要对题目进行改写。
我们用``Context''和``Question''区分问题的描述与提问。
我们将原始的自然文本式的题目改写成了选择题的形式，选项与答案分别用``Options''和``Answer''字段表示。
此外，我们从题目原始信息中发现初始线索，并不断对线索进行深入推理、归纳和关联，推导出新线索，最终找到答案，并将整个推理过程用字段``Clue Graph''进行存储。

\textbf{人工校验}
所有通过gpt-4-turbo-1106-preview处理的题目均经过人工校验。我们共招募了5名标注者与作者共同参与校验工作，主要包括初步筛选（剔除答案、选项不合理或需大幅修改的题目）和细节调整（微调选项和答案，使其更合理、自然）。标注的具体要求和示例详见附录。

经过上述流程，我们共收集了1200道侦探推理题。
随机选取其中33.4\%、33.3\%和33.2\%分别作为训练集、验证集和测试集。
测试集的难度等级由人类参与者评定，每道题平均记录两个未经提示的人类答案。详细统计信息见统计表。

==> latex/03.BenchmarkConstruction.05.tex <==
\begin{figure*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \includegraphics{figures/Example_2.pdf}
    }
    \caption{The example of the question in Detective Reasoning Benchmark}
    \label{fig:example}
    \vspace{-5mm}
\end{figure*}


\begin{figure*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \includegraphics{figures/Framework_2.pdf}
    }
    \caption{
    Within the Self-Question Prompt paradigm, the process is bifurcated into distinct phases: Detail Detection and Detail Connection, followed by Answer Inspiration and Weighted Reasoning. 
    These stages collectively encourage the LM to autonomously mine and integrate maximal contextual clues, subsequently leveraging these insights to engage in reasoning and synthesis relative to the posed inquiry.
    The Self-Question Finetune strategy is predominantly aimed at collecting data for fine-tuning.
    The first three phases permits free generation via open-source models, culminating in the aggregation of these outputs into a cohesive answer during the final stage.
    Employing a benchmark annotated with explicit reasoning pathways, like our Detective Reasoning Benchmark, facilitates the direct transformation of these reasoning sequences into fine-tuning datasets.
    % The illustration of Self-Question Prompt and Finetune framework.
    % In Self-Question Prompt, Detail Detection and Detail Connection phases prompt LM to extract maximum clues from the context freely, and Answer Inspiration and Weighted Reasoning phase prompt LM to reasoning and summarize the clues based on the question.
    % In Self-Question Finetune， 主要的目标是收集微调数据, 前三个过程可以使用开源模型进行随意输出，而将随意输出的内容在最后一个过程总结到答案。
    % 如果使用一个标注了推理过程的benchmark，比如Detective Reasoning Benchmark，则可以直接将推理过程改写为微调数据。
    }
    \label{fig:framework}
    \vspace{-5mm}
\end{figure*}

\input{tables/tab_human}
侦探推理基准（Detective Reasoning Benchmark）旨在评估模型在信息过载情景下的关键信息识别与多步推理能力。因此，该基准的核心要素包括：
1. 题目描述应包含长篇、复杂且表面看似不相关的信息。
2. 解答过程需涉及基于原始信息的多步推理。
3. 应能够客观、精确地评估模型的性能。

公开的侦探推理题目通常将解题关键信息隐藏于题目描述中，需要通过深度推理对所有信息进行分析以发现这些信息。
为了构建一个有效的LLM评估基准，我们首先对题目进行了严格的质量和道德审查。
此外，我们还标注了解题的多步推理过程，以便于过程监督。
我们对关键信息在原文中进行了句子级别的标注，同样，为了关键信息不覆盖原文过多的内容，我们在不影响对原文又进行了句子级的扩展。
最后，参考当前许多研究采用的选择问答评估方式，我们期望将侦探推理基准以选择题形式构建，以增强评估的客观性、可量化性，并降低评估成本。

在侦探推理基准中，每个题目以JSON格式组织，包括``Context''、 ``Question''、 ``Options''、 ``Answer''和``Clue Graph''五个主要元素。
数据处理包括题目筛选、题目改写和人工校验三个阶段，前两阶段主要借助gpt-4-turbo-1106-preview模型完成。

\textbf{题目筛选：}
为保证基准聚焦于信息过载''、关键信息发现''和``多步推理''，我们筛选了题目。鉴于侦探推理题可能有多种答案和推理路径，我们尽量确保每个题目的推理方案尽可能简明，以确保答案和推理过程的合理性和唯一性。同时，为确保基准的广泛适用性，我们排除了过度依赖符号逻辑或专业知识的题目。
具体来说，我们排除了四类题目：
1. 需要视觉或听觉信息辅助的题目；
2. 反逻辑或答案不合理或过于多样的题目；
3. 需要大量符号逻辑或领域知识的题目；
4. 关键信息太过明显的题目。

\textbf{题目改写：}
原始题目可能将问题描述和问题本身混为一谈，有时甚至直接透露答案，有些题目并没有包含太多的无关内容。
因此，我们需要对题目进行改写，使用Context''和Question''区分问题的背景与提问。
将原始的自然文本题目改为选择题形式，用Options''和Answer''字段表示选项和答案。
此外，我们从原始信息中提取初始线索，并通过深入推理、归纳和关联来发现新线索，最终找到答案，并用``Clue Graph''字段记录整个推理过程。
同时，在不改变原文的推理方式的基础上，对所有题目进行合理地加长，来保证``Clue Graph''中的``Key Information''只覆盖了至多30\%的原文内容。
最后，我们将所有题目翻译为了英语。

\textbf{人工校验:}
所有经gpt-4-turbo-1106-preview模型处理的题目均需经过人工校验。
我们招募了5名标注者与作者共同进行校验，主要包括初步筛选（淘汰答案或选项不合理或需大幅修改的题目）和细节调整（微调选项和答案，使其更合理、自然）。标注的具体要求和示例详见附录。

\input{tables/tab_benchmark_case}

==> latex/03.BenchmarkConstruction.06.tex <==
\begin{figure*}[t]
    \centering
    \resizebox{0.8\textwidth}{!}{
    \includegraphics{figures/Example_2.pdf}
    }
    \caption{The example of the question in Detective Reasoning Benchmark}
    \label{fig:example}
    \vspace{-5mm}
\end{figure*}


\begin{figure*}[t]
    \centering
    \resizebox{0.8\textwidth}{!}{
    \includegraphics{figures/Framework_2.pdf}
    }
    \caption{
    Within the Self-Question Prompt paradigm, the process is bifurcated into distinct phases: Detail Detection and Detail Connection, followed by Answer Inspiration and Weighted Reasoning. 
    These stages collectively encourage the LM to autonomously mine and integrate maximal contextual clues, subsequently leveraging these insights to engage in reasoning and synthesis relative to the posed inquiry.
    The Self-Question Finetune strategy is predominantly aimed at collecting data for fine-tuning.
    The first three phases permits free generation via open-source models, culminating in the aggregation of these outputs into a cohesive answer during the final stage.
    Employing a benchmark annotated with explicit reasoning pathways, like our Detective Reasoning Benchmark, facilitates the direct transformation of these reasoning sequences into fine-tuning datasets.
    }
    \label{fig:framework}
    \vspace{-5mm}
\end{figure*}

\input{tables/tab_human}
\input{tables/tab_benchmark_case}
The Detective Reasoning Benchmark aims to evaluate models' abilities to identify key information and perform multi-step reasoning in scenarios characterized by information overload. Therefore, the core elements of this benchmark include:

1. Question descriptions should contain lengthy, complex, and seemingly unrelated information.
2. The solution process must involve multi-step reasoning based on the original information.
3. The model's performance should be assessed objectively and accurately.

Publicly available detective reasoning questions typically hide the key information within the question descriptions, necessitating deep reasoning to analyze all information and uncover these details.
To construct an effective LLM evaluation benchmark, we first conducted a rigorous quality and ethical review of the questions.
Furthermore, we annotated the multi-step reasoning process of solving the questions to facilitate process supervision.
We performed sentence-level annotations of key information in the original text, and to prevent excessive coverage of the original content by key information, we expanded the sentences without affecting the original text.
Lastly, in line with the multiple-choice question-and-answer evaluation method adopted by many current studies, we aim to construct the Detective Reasoning Benchmark in a multiple-choice format to enhance the objectivity, quantifiability, and reduce the cost of evaluation.

In the Detective Reasoning Benchmark, each question is organized in JSON format, comprising five main elements: "Context," "Question," "Options," "Answer," and "Clue Graph."
Data processing includes question selection, question rewriting, and manual verification stages, with the first two stages primarily assisted by the GPT-4-turbo-1106-preview model.

\textbf{Question Selection:}
To ensure the benchmark focuses on "information overload," "key information discovery," and "multi-step reasoning," we screened questions. Given the potential for multiple answers and reasoning paths in detective reasoning questions, we endeavored to ensure each question's reasoning scheme was as clear and straightforward as possible to ensure the reasonableness and uniqueness of the answers and reasoning processes. Simultaneously, to ensure the benchmark's broad applicability, we excluded questions overly dependent on symbolic logic or specialized knowledge.
Specifically, we excluded four types of questions:

1. Questions requiring visual or auditory information for support;
2. Questions that are anti-logical, have unreasonable answers, or are overly diverse;
3. Questions requiring extensive symbolic logic or domain knowledge;
4. Questions with overly obvious key information.
\textbf{Question Rewriting:}
The original questions might conflate the problem description with the question itself, sometimes even revealing the answer directly, and some questions do not contain much irrelevant content.
Therefore, we needed to rewrite the questions, using "Context" and "Question" to distinguish between the background of the problem and the inquiry.
We converted the original natural text questions into multiple-choice format, with "Options" and "Answer" fields representing the choices and the correct answer.
Additionally, we extracted initial clues from the original information and discovered new clues through in-depth reasoning, induction, and association to find the answer, which was documented in the "Clue Graph" field.
Simultaneously, without altering the original reasoning approach, we reasonably extended all questions to ensure the "Key Information" in the "Clue Graph" covered at most 30% of the original content.
Lastly, we translated all questions into English.

\textbf{Manual Verification:}
All questions processed by the GPT-4-turbo-1106-preview model were subject to manual verification.
We recruited five annotators to work with the authors on verification, which included initial screening (eliminating questions whose answers or options were unreasonable or required significant modification) and detail adjustment (fine-tuning options and answers to make them more reasonable and natural). Specific requirements and examples for annotation are detailed in the appendix.







==> latex/03.BenchmarkConstruction.07.tex <==

\begin{figure*}[t]
    \centering
    \resizebox{0.85\textwidth}{!}{
    \includegraphics{figures/Example_2.pdf}
    }
    \caption{The example of the question in DetectBench}
    \label{fig:example}
    \vspace{-5mm}
\end{figure*}


\begin{figure*}[t]
    \centering
    \resizebox{0.85\textwidth}{!}{
    \includegraphics{figures/Framework_2.pdf}
    }
    \caption{
    Within the Self-Question Prompt paradigm, the process is bifurcated into distinct phases: Detail Detection and Detail Connection, followed by Answer Inspiration and Weighted Reasoning. 
    The Self-Question Finetune strategy is predominantly aimed at collecting data for fine-tuning.
    The first three phases permits free generation via open-source models, culminating in the aggregation of these outputs into a cohesive answer during the final stage.
    }
    \label{fig:framework}
    \vspace{-5mm}
\end{figure*}

\input{tables/tab_human}
\subsection{Benchmark Construction}
The DetectBench aims to evaluate model's joint abilities in information detection and multi-step commonsense reasoning.
Therefore, benchmark should provide the following elements:
(1). Question that lack ethical integrity or encompass topics of a sensitive nature.
(2). Question descriptions should contain lengthy, complex, and seemingly unrelated information.
(3). The solution to the question should involve multi-step reasoning based on the original information.
(4). The model's response to the question should be assessed objectively and accurately.


Each question is organized in JSON format, comprising five main elements: ``Context'', ``Question'', ``Options'', ``Answer'' and ``Clue Graph'' as shown in Fig.~\ref{fig:example}.
Data processing includes question selection, question rewriting, and manual verification stages, with the first two stages primarily assisted by the GPT-4-turbo-1106-preview model.

\textbf{Question Selection:}
To ensure the benchmark focuses on ``key information discovery'' and ``multi-step commonsense reasoning'', we screened questions.
Given the potential for multiple answers and reasoning paths in detective reasoning questions, we endeavored to ensure each question's reasoning scheme was as clear and straightforward as possible to ensure the reasonableness and uniqueness of the answers and reasoning processes.
Simultaneously, we excluded questions overly dependent on symbolic logic or specialized knowledge because such questions cannot be solved simply by retrieving related infomation.
Specifically, we excluded five types of questions:
1. Questions that are not ethical or have sensitive matters.
2. Questions requiring visual or auditory information for support;
3. Questions that are anti-logical, have unreasonable answers, or are overly diverse;
4. Questions requiring extensive symbolic logic or domain knowledge;
5. Questions with overly obvious key information.

\textbf{Question Rewriting:}
The original questions might conflate the problem description with the question itself, sometimes even revealing the answer directly, and some questions do not contain much irrelevant content.
Therefore, we needed to rewrite the questions, using \underline{``Context''} and \underline{``Question''} to distinguish between the background of the problem and the inquiry.
We converted the original natural text questions into multiple-choice format, with \underline{``Options''} and \underline{``Answer''} fields representing the choices and the correct answer.
Addationally, we construct \underline{``Clue Graph''} to explicitly represent the reasoning process. 
We annotated important content within the original text as \underline{``Key Information from Context''}. 
Based on these key information, we delineated the \underline{``Multi-Hop Reasoning From Key Information''} encompasses the reasoning process from a single piece of information as well as joint reasoning based on multiple pieces of information. 

\textbf{Manual Verification:}
All questions processed by the GPT-4-turbo-1106-preview model are subject to manual verification.
We recruited five annotators to work with the authors on verification, which included initial screening (eliminating questions whose answers or options were unreasonable or required significant modification) and detail adjustment (fine-tuning options and answers to make them more reasonable and natural). Specific requirements and examples for annotation are detailed in the Appendix~\ref{appendix_annotators}.


\subsection{Human Performance}

To explore the nuances of human performance on the DetectBench and to compile benchmark results, we engaged 50 human participants to address questions within the dev set. The examination spanned a total of three hours, with participants afforded the option to leave upon early completion. This cohort consisted of undergraduate and graduate students from universities across China, each remunerated at rates exceeding the local minimum hourly wage. Additionally, participants were awarded bonuses for each correctly answered question. For the purpose of facilitating human participation, the benchmark was translated into Chinese, and responses were provided in the same language.

We utilized an established online question-and-answer platform. Each participant was tasked with responding to 15 questions, employing a subset of 250 questions from the dev set of the DetectBench. This approach ensured that each question received responses from three distinct participants. The performance of humans on the DetectBench is documented in Tab.~\ref{tab:human_performance}.

% ~(https://www.wjx.cn/)








==> latex/04.OurMethod.01.tex <==

\begin{figure*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \includegraphics{figures/Framework.pdf}
    }
    \caption{
    The illustration of Self-Question Prompt framework. 
    During the Detail Detection and Detail Connection phase, the model is prompted to extract maximum clues from the primary context. 
    In the Answer Inspiration phase, the model is tasked with discerning the correlation between these clues and the initial question. 
    Throughout the Output Command stage, the model is required to generate an ideal response that draws upon both the context and the cognitive processes aforementioned.
    }
    \label{fig:framework}
    \vspace{-5mm}
\end{figure*}
% \input{tables/tab_questions}

As shown in Figure~\ref{fig:framework}, Self-Question consists of four stages, namely Detail Detection, Detail Connection, Answer Inspiration, and Output Command. 
These four components guide the model in its thinking process, sequentially stimulating a deeper understanding of the text as well as allowing the model to identify key and distractor information. 
Finally, using all previous thought processes, it generates correct answers for the questions.
The detailed prompts we provide in each stage are listed in Appendix in Tab.~\ref{tab:prompts}.


% \textbf{Detail Detection:} During this phase, it is incumbent upon the Language Learning Model (LLM) to engage in an intense exploration to comprehend the presented textual information, and subsequently extract concealed details within the text, including the identification and interpretation of facts, concepts, and events. The primary focus of this stage is to direct the model to generate exhaustive details and facts grounded in the presented context, with particular emphasis on details that are not overtly discernible in the raw context. This process significantly bolsters the model's comprehension of real-life contexts and supplies the fundamental information base for the model's ensuing reasoning process.

% \textbf{Detail Connection:} This phase entails the analysis and comprehension of the previously identified details, and strives to establish potential connections amongst them. The objective of this stage is to facilitate the model's understanding of the composition of textual information, further directing the models to create additional details based on the given ones. This practice enables the extraction of more profound details as the supporting evidence for more advanced reasoning.

% \textbf{Answer Inspiration:} In this phase, the model is necessitated to scrutinize the interrelations between these details and the inquiry. The aim of this stage is to unveil hints within the existing data which could be instrumental in formulating a response to the inquiry. This operation not only amplifies the model's prediction capabilities, but also leads the model to an accurate determination of the ultimate response, substantially mitigating the likelihood of speculative searching.

% \textbf{Weighted Reasoning:} During this phase, the model is encouraged to prioritize the information extrapolated from the previous three stages, subsequently considering the information encapsulated in the original document, and provide a response after a comprehensive reasoning. The goal of this stage is to ensure that the model effectively leverages the reasoning content for its final response, thus enhancing the reliability of the response. This not only augments the model's discernment, but also improves the precision and credibility of the model-generated response.


\textbf{Detail Detection:} 
% At this stage, LLM is prompted to delve deeply into understanding the given text information and output more details hide behind the text, which includes identification and handling of facts, concepts, and events. 
The objective of this stage is to ask model to generate as much detail and facts based on the given context as possible, especially for the details that are not explicit in the raw context.
This would notably enhance the model's understanding of the real-life context and provide the essential information foundation for the subsequent reasoning process of the model.

\textbf{Detail Connection:}
% The work at this stage involves parsing and understanding the identified details and attempting to find possible connections among them.
The aim of this stage is to enable the model to understand how the textual information is assembled together, further asking models to generate more details based on the given details.
By doing so, deeper details are mined out as evidence for deeper reasoning.

\textbf{Answer Inspiration:}
% In this phase, the model is required to analyze the connections between these details and the question.
The objective of this stage is to find clues from the existing information that can aid in answering the question.
This operation, on the one hand, can enhance the model's predictive power, and on the other hand, it can help the model to precisely pinpoint the final answer, greatly reducing the possibility of random search.

\textbf{Weighted Reasoning:}
At this stage, the model is prompted to prioritize the information deduced from the previous three stages, then take the information in the original article into consideration, and output the answer after comprehensive reasoning.
The objective of this stage is to ensure that, when producing the answer, the model can effectively utilize the reasoning content for the final response, thereby improving the reliability of the answer.
This not only escalates the model's judgment but also enhances the accuracy and credibility of the model-generated answer.


% \textbf{细节检测:} 
% 在这个阶段，LLM被要求对给定的文本信息进行深入理解和解读，包括对事实、概念和事件等的识别和处理。
% 这个阶段的目标是确保模型能准确理解文本，对文本的全局和局部信息有一个清晰的认识。
% 这样做可以明显地提升模型的理解能力和信息处理能力，为模型后续的推理过程提供必要的信息基础。

% \textbf{细节关联:} 
% 此阶段的工作是解析和理解识别到的这些细节，并尝试在这些细节之间找到可能存在的关联。
% 这个阶段的目标是让模型能明白文本的信息是如何组装在一起的，进一步推动模型掌握到文本的内在逻辑。
% 通过这样做，模型的关联分析能力可以被有效提升，使得模型能更好地理解和处理复杂的推理问题。

% \textbf{回答启发:} 
% 在这个阶段中，模型被要求分析这些细节与问题之间的联系，尝试用已经掌握的信息来预测可能的答案。
% 这个阶段的目标是从现有的信息中找出对解答问题有帮助的线索。
% 这样的操作一方面能提升模型的预测能力，另一方面也能帮助模型更精准地锁定最终的答案，大大降低了随机搜索的可能性。

% \textbf{集成输出:}
% 在这个阶段，模型在生成答案时需要着重考虑自己通过前三个阶段推理得到的信息，然后再考虑使用原始文章中的信息，进行综合考量后输出答案。
% 此阶段的目标是确保模型在输出答案时，能够有效地使用推理内容进行最后的回答，从而提高答案的可靠度。
% 这样做不仅能提升模型的判断力，还能提高模型生成答案的准确性和信度。









% \textbf{细节检测:} 
% 细节检测阶段的目标在于对于给定的文本信息进行深入理解和解读。
% 具体而言，我们要求LLM首先对指定的文本进行阅读和处理，其核心对事实、事件、概念、观点等进行辨别和分类。
% 此任务对LLM涌现广泛知识和技能的需求以确保对全文的全面理解和解读，其也极为关键，对于后续的思考步骤做了必要的铺垫。

% \textbf{细节关联:} 
% 在模型挖掘出了大量细节之后，我们要求LLM根据已有的细节进行深入的分析以及关联。
% 此过程的目标在于找出并揭示潜在的、并非直观的、有可能的联系以及因果关系。
% 此步骤增加了寻找答案的复杂性，但同时也拓宽了发现准确答案的可能性。

% \textbf{回答启发:} 
% 在明确文本细节以及其相互关系后，我们要求模型分析这些细节与问题之间的联系。
% 此步骤的目标在于诱导LLM从海量信息中寻找关键内容。
% 这个过程将全文信息以及问题紧密地联系起来，找到问题答案与文本细节之间的桥梁，为最后的答题步骤做好充分的准备。

% \textbf{集成输出:}
% 依托于前三个步骤，我们会要求LLM整合之前所有的线索，并根据整合内容输出问题可能的结果。
% 这一步的目标在于让模型理解前面所有信息的权重是不同的。
% 这个过程将输入的prompt



% 按照要求重写下列内容：
% 1. 将所有的GPT-4词汇都变为LLM
% 2. 取消所有的举例说明。
% 3. 这段文本是源于一篇论文，下面的四个过程是对于提示词的改进方法。所以重写之后的文本要能够体现通过改进提示词能够使模型能够做到细节发现、细节关联、回答启发以及集成输出。


% 我为了提升大模型解决侦探推理益智题的能力，设计了一种提示词框架。
% 这个提示词框架包含四个主要的阶段，分别是“细节检测”、“细节关联”、“回答启发”、“加权输出”。
% “细节检测”阶段的工作时对于给定的文本信息进行深入理解和解读。
% “细节关联”阶段的工作是根据已有的细节进行深入的分析以及关联。
% “回答启发”阶段的工作是分析这些细节与问题之间的联系。
% “加权输出”阶段的工作是要求模型着重考虑自己推理得到的内容，然后再结合原始文章并进行输出。
% 请你帮我把这四个阶段的工作描述进行扩写。要求每个阶段的描述分别包含三个内容，分别为：这个阶段做了什么，这么做的目标是什么，这么做能给大模型带来什么提升。




% ```
% \textbf{Detail Detection:}
% 这一步准确地说是理解和解读文本信息。
% 最初，GPT-4 会阅读并处理所提供的文本，主要是对事实、事件、概念、观点等进行识别和分类。
% 这项任务非常艰巨，因为它要求 GPT-4 具备足够的知识和技能来理解和解读整个文本。
% 然而，这也是必不可少的，因为透彻准确的理解和解码为后续的思考奠定了基础。
% 例如，一篇文章可能包含多个主题，每个主题都与不同的事实和观点有关。
% GPT-4 积极识别这些不同的元素并挖掘细节，为下一步提供重要信息。

% \textbf{Detail Connection:}
% 一旦汇总了所有细节，GPT-4 就会利用其固有的算法和框架进行更深入的探索和分析。
% 这一过程通常被称为 "模式识别 "或 "深度连接挖掘"，它试图找到并揭示潜在的、非显而易见的、潜在的关系或因果关系。
% 例如，它可以揭示文章中某一主题的立场如何影响或决定其他主题的态度或观点。
% 这一步骤增加了寻找问题答案的复杂性，但也为发现准确答案提供了更多可能性。

% \textbf{Answer Inspiration:}
% 在明确文本细节及其相互联系之后，下一步就是分析这些细节与具体问题之间的关系。
% 这有助于 GPT-4 更准确地回答问题，避免盲目地从海量信息中寻找答案的尴尬局面。
% 这一步要求 GPT-4 运用分析结果解决具体问题，将全文信息与问题紧密联系起来，找到问题答案与文本细节之间的桥梁，为最后的答题步骤准备充足的信息支持。

% \textbf{Output Command:}
% 在前三个步骤的基础上，GPT-4 采取最后一步，根据既定的综合思维过程，利用收集到的信息和之前的深刻分析回答问题。
% 这个答案需要深思熟虑，应该是之前抽象思维过程的具体应用和实例化，验证各种基本逻辑。
% 这一步骤体现了 GPT-4 的推理作答能力，力求尽可能提高推理的准确性和深度。```

% \textbf{Detail Detection:}
% This step accurately involves understanding and deciphering the textual information. 
% Initially, GPT-4 reads and processes the provided text, mainly identifying and categorizing facts, events, concepts, opinions, and so forth. 
% This task is arduous as it requires GPT-4 to possess sufficient knowledge and skills to comprehend and decode the whole text.
% Nonetheless, it is essential, since thorough and precise comprehension and decoding lay the foundation for subsequent contemplation.
% For instance, an article might contain multiple themes, each associated with different facts and opinions.
% GPT-4 actively identifies these different elements and mines the details, providing essential information for the next step.

% \textbf{Detail Connection:}
% Once all the details are compiled, GPT-4 uses its inherent algorithm and framework for a more profound exploration and analysis.
% Often referred to as "pattern recognition" or "deep connection mining", this process attempts to locate and reveal latent, non-obvious, potential relationships or causality.
% For instance, it might unveil how the standpoint of one theme in an article influences or determines the attitude or opinion of other themes.
% This step adds a layer of complexity to finding the answer to a question but also offers more possibilities for discovering the accurate answer.

% \textbf{Answer Inspiration:}
% Upon clearly establishing the text details and their interconnections, the next step involves analyzing the relationship between these details and the specific question.
% This aids GPT-4 in answering the question more accurately, avoiding the awkward situation of blindly searching for the answer from a vast amount of information.
% This step demands GPT-4 applies the analysis results to solve the specific question, tightly linking the whole text information with the problem, finding the bridge between the question's answer and the text details, and preparing ample information support for the final question-answering step.

% \textbf{Output Command:}
% Based on the previous three steps, GPT-4 takes the final step, answering the question according to the established comprehensive thinking process, utilizing the gathered information and previous profound analysis.
% This answer needs thorough contemplation and should be a specific application and instantiation of the previous abstract thinking process, validating various underlying logics.
% This step manifests GPT-4’s reasoning response ability, striving to enhance the accuracy and depth of reasoning as much as possible.



==> latex/04.OurMethod.02.tex <==

\begin{figure*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \includegraphics{figures/Framework.pdf}
    }
    \caption{
    The illustration of Self-Question Prompt framework. 
    During the Detail Detection and Detail Connection phase, the model is prompted to extract maximum clues from the primary context. 
    In the Answer Inspiration phase, the model is tasked with discerning the correlation between these clues and the initial question. 
    Throughout the Output Command stage, the model is required to generate an ideal response that draws upon both the context and the cognitive processes aforementioned.
    }
    \label{fig:framework}
    \vspace{-5mm}
\end{figure*}


\subsection{Self-Question Prompt}
如图所示，自问自答模型包括四个阶段：Detail Detection、Detail Connection、Answer Inspiration和Weighted Reasoning。
这四个部分依次引导模型先推理，然后发现关键信息，最后结合关键信息挖掘正确的答案。
各阶段的具体提示列在Appendix中。

\textbf{Detail Detection: }
该阶段的目的是促使模型基于给定内容生成尽可能多的细节和事实，特别是原始上下文中未明确给出的细节。
这将显著增强模型对现实情境的理解，并为模型后续推理过程提供必要的信息基础。

\textbf{Detail Connection:}
该阶段旨在使模型理解文本信息如何组合在一起，并进一步要求模型基于给定细节生成更多细节。

\textbf{Answer Inspiration:}
该阶段的目标是从现有信息中找到有助于回答问题的关键信息，并根据关键信息进行推理。

\textbf{Weighted Reasoning:}
考虑到Self-Question Prompt可以在一次问答也可以分别在多轮对话中使用，而在一次问答时，LLM将会根据前面context里的所有内容选择最终的答案。
而LLM的推理很受context所有内容的影响，所以在经过了前面所有的推理之后，最终答案的选择应该更加重视推理过程中LLM自己总结的内容。
加上Weighted Reasoning这一个阶段，将有助于增强模型在一次问答的总结答案时更加重视之前LLM自己生成的推理结果，而不是全面考虑所有的context信息。

\subsection{Self-Question Finetune}
基于上面给出的prompt方法，我们进一步提出能够增强模型面对Information Overload场景下的一种微调方法。
The idea of Self-Question Finetune is simple: 就是将推理过程和答案按照每个prompt阶段进行诱导和组合。

对于像Detective Reasoning Benchmark这种标注了推理过程的Benchmark，可以简单地将推理过程中对应的组件输出，并要求模型根据结构化的过程生成自然文本，然后将自然文本进行组合。
而对于一般只有标准答案的Benchmark，可以让模型自动根据答案和问题补全中间的推理过程，然后将推理过程收集为finetune数据。






% 在此阶段，模型将根据前三个阶段推导出的信息进行优先级排序，考虑原始文章中的信息，并在综合推理后输出答案。该阶段的目标是确保在产出答案时，模型能有效利用推理内容进行最终响应，从而提高答案的可靠性。这不仅提升了模型的判断力，还增强了模型生成答案的准确性和可信度。



% 如图~ref{fig:framework}所示，"自我提问 "包括四个阶段，即细节检测、细节连接、答案启发和输出指令。
% 这四个部分引导模型的思考过程，依次激发对文本的深入理解，并允许模型识别关键信息和干扰信息。
% 最后，利用之前所有的思维过程，它将为问题生成正确答案。
% 我们在每个阶段提供的详细提示列于附录中的 Tab.~ref{tab:prompts}。

% \textbf{Detail Detection:} 
% 这一阶段的目的是要求模型根据给定上下文生成尽可能多的细节和事实，尤其是原始上下文中没有明确指出的细节。
% 这将显著增强模型对现实语境的理解，并为模型的后续推理过程提供重要的信息基础。

% \文本连接：} textbf{Detail Connection:}
% 这一阶段的目的是让模型理解文本信息是如何组合在一起的，进一步要求模型根据给定的细节生成更多细节。
% 通过这样做，可以挖掘出更深层次的细节，作为更深层次推理的证据。

% \文本bf{答案启发：} 本阶段的目标是找到文本信息的来源。
% 这一阶段的目标是从现有信息中找到有助于回答问题的线索。
% 这一操作一方面可以增强模型的预测能力，另一方面可以帮助模型精确定位最终答案，大大降低随机搜索的可能性。

% \textbf{Weighted Reasoning:}
% 在这一阶段，会提示模型对前三个阶段推导出的信息进行优先排序，然后将原文中的信息考虑在内，经过综合推理后输出答案。
% 这一阶段的目的是确保模型在生成答案时，能有效利用推理内容进行最终回答，从而提高答案的可靠性。
% 这不仅能提升模型的判断力，还能增强模型生成答案的准确性和可信度。




==> latex/04.OurMethod.03.tex <==


\subsection{Self-Question Prompt}

自问自答模型的构建涵盖四个主要阶段：细节检测、细节关联、答案启发和加权推理。这一过程旨在通过逐步深入的逻辑推理，使模型能够识别关键信息并据此提炼出准确的答案。各阶段的详细操作指南见附录。

\textbf{细节检测：} 该阶段旨在激发模型挖掘给定内容的细节与事实，特别是那些在原始文本中未被直接阐述的信息。这一过程不仅增强了模型对情境的理解，而且为后续的推理过程奠定了坚实的信息基础。

\textbf{细节关联：} 此阶段着重于训练模型理解文本中信息的内在联系，并基于已识别的细节生成新的相关信息，从而进一步完善信息网络。

\textbf{答案启发：} 该阶段的目标是识别对解决问题至关重要的关键信息，并围绕这些关键信息展开推理，以触发可能的答案。

\textbf{加权推理：} 考虑到自问自答模型既可用于单轮问答，也可用于多轮对话，本阶段旨在强化模型对自身生成的推理结果的依赖，相较于整体上下文，更加重视这些推理结果在最终答案的确定中的作用。这一机制有助于模型在提炼最终答案时，更加准确地聚焦于关键的推理内容。

\subsection{Self-Question Finetune}

在上述自问自答模型的基础上，我们提出了一种针对信息过载场景下的微调策略。简言之，此策略通过按照各个阶段的提示对推理过程和答案进行诱导和整合，从而增强模型的处理能力。

对于已明确标注推理过程的基准测试（如Detective Reasoning Benchmark），可以直接提取各个阶段的推理输出，并引导模型基于这些结构化的推理内容生成自然语言文本，进而将这些文本整合。对于仅有标准答案的基准测试，模型可自动根据问题和答案补全推理过程，并将这些推理内容作为微调数据进行整理。这种方法有效地桥接了问题、推理过程与答案之间的逻辑链条，为模型提供了更为丰富且结构化的学习材料。

==> latex/04.OurMethod.04.tex <==
\subsection{Construction of the Self-Questioning Model}

The construction of the self-questioning model encompasses four primary stages: Detail Detection, Detail Association, Answer Elicitation, and Weighted Reasoning. This process is designed to enable the model to identify key information and thereby extract precise answers through progressively deeper logical reasoning. A detailed operational guide for each stage is provided in the appendix.

\textbf{Detail Detection:} This phase aims to stimulate the model to unearth details and facts within the given content, especially those not explicitly stated in the original text. This process not only enhances the model's understanding of the context but also lays a solid informational foundation for the subsequent reasoning process.

\textbf{Detail Association:} This stage focuses on training the model to understand the intrinsic connections between pieces of information in the text and to generate new related information based on identified details, thereby further refining the information network.

\textbf{Answer Elicitation:} The objective of this phase is to identify key information crucial for solving the question and to initiate reasoning around this information to trigger possible answers.

\textbf{Weighted Reasoning:} Considering that the self-questioning model can be applied to both single-round and multi-round dialogues, this stage aims to reinforce the model's reliance on its generated reasoning outcomes, valuing these outcomes more in the determination of the final answer compared to the overall context. This mechanism aids the model in more accurately focusing on essential reasoning content when refining the final answer.

\subsection{Self-Question Finetune}

Building upon the aforementioned self-questioning model, we propose a finetuning strategy for scenarios characterized by information overload. In essence, this strategy enhances the model's processing capabilities by guiding and integrating the reasoning process and answers according to prompts from each stage.

For benchmarks explicitly annotated with reasoning processes (such as the Detective Reasoning Benchmark), the model can directly extract reasoning outputs from each stage and guide the generation of natural language texts based on these structured reasoning contents, thereafter integrating these texts. For benchmarks with only standard answers, the model can automatically complete the reasoning process based on the questions and answers and organize these reasoning contents as finetuning data. This method effectively bridges the logical chain between questions, reasoning processes, and answers, providing the model with richer and more structured learning materials.

==> latex/04.OurMethod.05.tex <==
\subsection{Construction of the Self-Questioning Model}

The construction of the self-questioning model encompasses four primary stages: Detail Detection, Detail Association, Answer Elicitation, and Weighted Reasoning.
This process is designed to enable the model to identify key information and thereby extract precise answers through progressively deeper logical reasoning as shown the above of Fig.~\ref{fig:framework}.
Detailed prompts for each stage is provided in the Appendix~\ref{appendix_prompt}.

\textbf{Detail Detection} aims to stimulate the model to unearth details and facts within the given content, especially those not explicitly stated in the original text. 
\textbf{Detail Association} ask the model to understand the intrinsic connections between pieces of information in the text and to generate new related information based on identified details.
\textbf{Answer Elicitation} is to identify key information crucial for solving the question and to initiate reasoning around this information to trigger possible answers.
\textbf{Weighted Reasoning} to reinforce the model's reliance on its generated reasoning outcomes, value these outcomes more in the determination of the final answer compared to the overall context.

\subsection{Self-Question Finetune}



Building upon the aforementioned self-questioning model, we propose a finetuning strategy for jointly enhancing the ability of information detection and commonsense reasoning as shown the below of Fig.~\ref{fig:framework}.
For benchmarks explicitly annotated with reasoning processes (such as the DetectBench), one can directly concat reasoning outputs for each stage as the finetune data. 
For benchmarks with only standard answers, the model can automatically complete the reasoning process based on the questions and answers and organize these reasoning contents as finetuning data.
The advantage of this method lies in using the freely output of a LLM as finetune data in the first three stage, which significantly reducing the complexity of constructing datasets that include inferential processes.
% This method effectively bridges the logical chain between questions, reasoning processes, and answers, providing the model with richer and more structured learning materials.

==> latex/042.Human.tex <==

% 为了详细分析人类是如何进行informal reasoning的，以及为了收集人类进行informal reasoning的基准结果。
% We invited 50 human participants to solve questions within the test set of Detective Reasoning Puzzles.
% 我们利用了在线问答系统构建了问答题目，每个参与者在在线系统上进行问答的同时，方便我们追踪每道题目回答的时间。
% These 50 individuals were divided into two groups:


To delve into the specifics of how humans do informal reasoning and to gather benchmark results, we incorporated 50 human participants to tackle questions within the test set of Detective Reasoning Puzzles.
The total duration of the test was three hours, and the participants were permitted to depart upon early completion.
The 50 participants comprised undergraduate and graduate students from universities in China, each of whom was compensated with wages surpassing the local minimum hourly rate.
The benchmark is translated into Chinese language for human tests, and the answers provided by participants are also in Chinese.
Leveraging the existing online question-and-answer system~\footnote{https://www.wjx.cn/}, we assembled the questions so that each participant was able to respond online, allowing us to conveniently track the time each question was answered. 


In order to provide human baseline results, as well as to validate the effect of Hint on human performance, we divided 50 subjects into two groups:
The first group is primary for posing baseline results, which consists of 40 participants who were provided with the ``Context'' and ``Question'' from the test puzzles.
In this group, we assigned each participant 20 questions, and each test question was answered by at least two people.
We ensure the randomness of question allocation, whilst maintaining an approximately equal length for all questions answered by an individual.
The second group was used to validate the effect of Hint on human outcomes, which consisted of 10 participants, who, in comparison to the first group, received additional ``Hints'' in their puzzles. 
We utilized only 100 questions from the test set in this group to ensure that each question used for testing was answered by at least two people.

It is important to note that we understand the importance of ensuring an equal number of participants in both test groups to yield more representative results.
However, our approach was constrained by the wages we could offer, as well as the necessity to ensure that each test question was answered by at least two people in the first group.
Consequently, this necessitated the adoption of a seemingly biased grouping strategy.


% 值得一提的是，我们知道应该尽量保证两组实验的人数相等，以提供更具有参考性的结果。
% 但我们受限于我们所能提供的工资，以及需要保证每道测试题都被第一组的至少2个人及以上回答，所以才采用了如此有偏的分组策略。




==> latex/05.Experiments.01.tex <==
% We primarily conducted experiments on the currently acknowledged powerful closed-source model, GPT-3.5-turbo~\cite{chatgpt}, and the highly capable llama model~\cite{touvron2023llama}. In Section~\ref{setup}, our experimental setup is introduced. The results of all models are presented in Table~\ref{tab:experiments}, with a detailed analysis provided in Section~\ref{experiments}. Furthermore, a comprehensive case study of each model and human participants is available in Section~\ref{case} in the Appendix.


\input{tables/tab_experiments}
\subsection{Experiment Setup}
\label{setup}

\textbf{Models:}
Referring to the Alpaca-Eval leaderboard on July 27, 2023, we select four best-performing models in four different parameter scales:
GPT-4~\cite{openai2023gpt4}, GPT3.5-turbo~\cite{openaichatgpt}, Vicuna-33b-v1.3~\cite{zheng2023judging}, WizardLM-13B-V1.2~\cite{xu2023wizardlm}, and Vicuna-7b-v1.3~\cite{zheng2023judging}.
In these, we used the official openai API for GPT-4 and GPT-3.5-turbo between July 10th and 29th, 2023, with their parameter counts being 1800B and 175B respectively.
Vicuna-33b-v1.3, WizardLM-13B-V1.2, and Vicuna-7b-v1.3 are models with parameters of 33B, 13B, and 7B respectively.
% They were the best-performing models in their respective parameter scales on Alpaca-Eval as of July 27, 2023.
In table~\ref{tab:experiments}, we use \texttt{GPT-4} to denote GPT-4 model, \texttt{GPT-3.5} to denote GPT-3.5-turbo, \texttt{Vicuna-33B} to represent Vicuna-33b-v1.3, \texttt{WizardLM} to represent WizardLM-13B-v1.2, and \texttt{Vicuna-7B} to represent Vicuna-7b-v1.3.


\textbf{Baselines:}
We picked out some methods of constructing prompts that can be used to enhance the model's informal reasoning capabilities for comparison.
\texttt{Naive} is simply input the ``Context'' and ``Question'' to the LLMs, and ask for answer.
\texttt{Self-CoT}~\cite{kojima2022large} is a simple prompt trick that adds ``let's think step by step'' to the prompt to ask LLMs step by step output the reasoning process.
\texttt{Auto-CoT}~\cite{zhang2022automatic} automatically construct demonstration in CoT format.
So it is worth noting that Auto-CoT is not suitable in the 0-shot setting, so we only test the performance in the 5-shot setting.
\texttt{Cheat-Naive} use ``Hint'' as one of the input.
Since ``Hint'' will not incur other information, only tell LLMs where is key information, so we regard Cheat-Naive as the upper bound of the existing Language Models.
\texttt{Self-Consistency}~\cite{wang2022self} propose to use voting supersedes the simple, naive greedy decoding used in earlier CoT prompting to output the mostly generated result by the model.
In the experiment, we generate ten different outputs using LLMs, and we ask model to generate the final result based on all the outputs.
\texttt{Complexity-CoT}~\cite{fu2022complexity} uses the longest reasoning steps among all the outputs produced for a question to generate the final output.
\texttt{Plan-and-Solve CoT~(PS-CoT)}~\cite{wang2023plan} functions by first deconstructing the question before seeking its solution. 
\texttt{Self-Question} is a method that we propose, in which, we require the model to first delve deeply into the information already available in the original text, ponder the link between this information and the problem, and finally ask the model to integrate its existing thoughts to formulate a response.

\textbf{Demonstration:}
Furthermore, we investigate the influence of in-context learning on the performance of the model.
To accomplish this, we carried out tests on each of the examination questions using demonstrations sampled from the training set.
For each test sample, we randomly selected 5 training samples to form a demonstration.
In this way, different models using various prompt settings would utilize the same 5-shot sample-based demonstration for the same question.
For Naive and Cheat-Naive approaches, we directly concatenate the sampled questions with the ``Answer'' or ``Hint'' to form demonstrations.
For Auto-CoT, we ask LLMs to generate the reasoning process of few-shot samples in the format of CoT and concate the CoT to the samples as a demonstration.
For examples about how we construct demonstrations are listed in Appendix

% For methods such as CoT, PS-CoT, Complexity-CoT, and Self-Question, we utilized the hints of each problem as part of the reasoning process, combining the problem description, hints, and analysis to form a single demonstration. Taking into account the maximum input length, we sampled three questions as a demonstration for each question.


\input{figures/SQPerformance}


\subsection{Overall Performance}
\label{experiments}
The detailed results are shown in Tab.~\ref{tab:experiments}, and here we give our analysis of the experiment results as follows:



\subsubsection{Humans Achieve Much Better Performance than Models} 
We list six different types of human performance in Table~\ref{tab:experiments}. 
The informal reasoning ability of humans far exceeds those of the best LLMs. 
Even the worst human performance (47.3\%) significantly surpasses the performance of GPT-4 on the Detective Reasoning Benchmark.
This demonstrates the unattainable level of proficiency humans exhibit in informal reasoning, possibly due to the vast amount of experience and common sense they possess, which aids in understanding various common scenarios and tools in the questions.

\subsubsection{Proper Reasoning Hint Benefits Humans, but More for Language Models} 
When using hints to assist reasoning, both the model and human performance improve significantly (Result of \textit{Hint-Naive}).
Interestingly, we observe that the improvement of GPT-4 after hint injection (+49.3\%) surpasses the improvement of the worst human performance (+37.7\%).
Considering many studies have found that GPT-4 retains a large amount of factual knowledge, we can infer that the powerful informal reasoning ability of humans comes from the ability to directly retrieve experienced elements and phenomena from the subconscious based on the observed scenario.
Since LM lacks extensive experience, we need to delve into principles to understand problems.
Therefore, when we provide hints to LM, it can know which principles to use to get the correct answer, greatly improving the model's performance.

\subsubsection{Demonstration Will Harm the Reasoning Performance of Language Models}
We observed that under the Naive and CoT settings, the results of the 5-shot became worse than the 0-shot.
Even after injecting hints, it cannot reverse this conclusion that demonstration will lead to a decline in LM's reasoning performance.
This experimental conclusion is consistent with many previous findings that \textit{in-context learning hardly improves the performance of LLMs in reasoning tasks}~\cite{gu2023xiezhi, huang2023c}.
This may be because the model has difficulty obtaining the necessary information for reasoning from the context.
The longer the context, the more distractions there are, leading to worse performance~\cite{behnamghader2022can}.

\subsubsection{Self-Question greatly improve the informal reasoning ability of SoTA LLMs}
For models with fewer parameters, the effect of utilizing ``Self-Question'' is not as optimal as ``PS-CoT''.
However, when models possess a greater volume of parameters and more potent capabilities, the enhancement resulting from using ``Self-Question'' is substantial.
This suggests that, with a suitable prompt design, powerful LLM can compensate, to a certain degree, for the lack of life experience and an inability to carry out intuitive reasoning.
At present, ``Self-Question'' is regarded as the best prompt for enhancing a model's capacity for informal reasoning. Nonetheless, it's worth noting, even for GPT-4, the score achieved after deploying ``Self-Question''~(35.8\%) still hasn't surpassed the lowest human score~(47.3\%).

% The results shown in the table suggest that although for models with small parameter sizes, the effect of using Self-Question is not as good as PS-CoT.
% However, for models with stronger parameters and abilities, the improvement brought by Self-Question is significant.
% This reveals that Language Learning Models~(LLMs), after a reasonable prompt design, can compensate for shortcomings such as lack of experience and inability to reason intuitively to a certain extent.
% Currently, the Self-Question Prompt can be considered as the best prompt for enhancing a model's informal reasoning capability.
% However, it's noteworthy that even GPT-4, after using Self-Question, its score~(35.8\%) still does not surpass the worst score of humans~(47.3\%).

% 从表中的结果来看，虽然对于小参数量的模型而言，使用了Self-Question的效果还不如PS-CoT的。
% 但对于参数量和能力都更强的模型而言，Self-Question带来的提升是可观的。
% 这可以说明，LLM经过合理的prompt设计之后，是可以一定程度上弥补经验缺失、无法进行直觉推理等缺点的。
% Self-Question Prompt目前可以被认为是增强模型informal reasoning能力最好的prompt。
% 但值得注意的是，即便是GPT-4，在使用了Self-Question之后的成绩~(35.8\%)依然没有超过人类的最差成绩~(47.3\%)

\subsection{Difference Between Human and GPT-4}

\textbf{Difference in Performance:} 
We decompose the factors that may affect the performance of humans and GPT-4, and draw the following conclusions based on the content shown in Figure~\ref{fig:SQPerformance}:
Firstly, the length of the question does not affect the accuracy of humans, but it significantly slows down the response speed of human respondents.
From this, it can be inferred that humans spend a lot of time not on reasoning, but on reading the question. Secondly, the length of the question severely affects the performance of GPT-4 under the Naive setting.
This may be because the longer the question, the more distracting information it contains, and language models (LM) are extremely poor at handling such distractions.
Lastly, Self-Question can stably and significantly improve the performance of answering long questions, but it may have some negative impact on short questions.

\textbf{Difference in Verification:} 
We manually annotated 60 results generated by GPT-4 and compared them with the results annotated by GPT-4. 
As shown in Figure~\ref{fig:gpt4verification}, the overall consistency is 91.7\%. 
Among them, the consistency between the model and humans is better when the length of the standard answer is shorter.
However, when the length of the standard answer is longer, there may be some discrepancies between the model and humans.
This is mainly because informal reasoning itself is a probabilistic inference. When the standard answer is too long, GPT-4 may consider that it is not necessary to answer so precisely in some places to be considered correct, while human annotators will score strictly according to the standard answer.



\subsection{Ablation Study}
The results from our ablation study are presented in Table~\ref{tab:ablation}.
We denote the ``Weighted Reasoning'' stage with WR, the ``Answer Inspiration'' stage with AI, and the ``Detail Connection'' stage with DC.
It is observed that each component of Self-Question plays a role in improving the informal reasoning ability of LMs.
The contribution of Detail Detection evidences that language models do not inherently utilize common-sense knowledge.
The enhancement brought about by Detail Connection underscores that language models generally do not engage in profound thinking.
The improvement yielded by Answer Inspiration suggests that while language models cannot directly eliminate irrelevant information, they do possess the capability to do so. 
The advancement provided by Weighted Output elucidates that language models typically treat all input prompts impartially.
The improvements brought about by the four components of the Self-Question method serve to highlight the shortcomings of the existing LLMs in conducting informal reasoning.


% The contribution of the Output Command stage appears to be relatively limited, yet it still functions in Hard Cases.
% Conversely, the other three stages significantly enhance performance in Hard Cases.
% 使用Detail Detection能带来提升, 说明了语言模型不会应用常识知识，只有当人们要求他应用时，他才会使用。
% 使用Detail Connection能带来提升说明了语言模型一般不会进行深度思考。
% 使用Answer Inspiration能带来提升说明语言模型无法直接排除干扰信息，但是却具备排除干扰信息的能力。
% 而使用Weighted Output能带来提升说明了语言模型一般会平等地对待所输入的prompt。

% From the results, it can be gleaned that retaining only the Detail Detection stage could slightly impair the model's performance in Easy Cases.
% This could be attributed to the absence of excessive scene descriptions in Easy Cases.
% These cases demand more from the model's scene-completion capability, with hardly any details to be discovered in the text.
% Consequently, requiring the model to discover details amidst such scarcity could further diminish its performance.


\input{figures/GPT4Verification}
\input{tables/tab_ablation}

\subsection{Case Study}
The case study is conducted as detailed in Appendix. 
Two cases are listed in Table~\ref{tab:case1} and Table~\ref{tab:case2}, and the analysis towards the cases is as follow: 
Since there is not much difference between self-CoT and naive reasoning, which results in similar outcomes.
After injecting the Hint, the model can accurately answer the questions due to the Hint's ability to eliminate distractions and highlight suspicious points.
PS-CoT, by extracting key variables from the context, can avoid the influence of distracting content, thus achieving good results. 
However, Self-Question, with its superior ability to perform deep reasoning and associations, can achieve better results in the example requiring deep reasoning.


==> latex/05.Experiments.02.tex <==
\input{tables/tab_experiments}
\subsection{Experiment Setup}
\label{setup}

\textbf{Models:}
Referring to the Alpaca-Eval leaderboard on July 27, 2023, we select four best-performing models in four different parameter scales:
GPT-4~\cite{openai2023gpt4}, GPT3.5-turbo~\cite{openaichatgpt}, Vicuna-33b-v1.3~\cite{zheng2023judging}, WizardLM-13B-V1.2~\cite{xu2023wizardlm}, and Vicuna-7b-v1.3~\cite{zheng2023judging}.
In these, we used the official openai API for GPT-4 and GPT-3.5-turbo between July 10th and 29th, 2023, with their parameter counts being 1800B and 175B respectively.
Vicuna-33b-v1.3, WizardLM-13B-V1.2, and Vicuna-7b-v1.3 are models with parameters of 33B, 13B, and 7B respectively.
% They were the best-performing models in their respective parameter scales on Alpaca-Eval as of July 27, 2023.
In table~\ref{tab:experiments}, we use \texttt{GPT-4} to denote GPT-4 model, \texttt{GPT-3.5} to denote GPT-3.5-turbo, \texttt{Vicuna-33B} to represent Vicuna-33b-v1.3, \texttt{WizardLM} to represent WizardLM-13B-v1.2, and \texttt{Vicuna-7B} to represent Vicuna-7b-v1.3.


\textbf{Baselines:}
We picked out some methods of constructing prompts that can be used to enhance the model's informal reasoning capabilities for comparison.
\texttt{Naive} is simply input the ``Context'' and ``Question'' to the LLMs, and ask for answer.
\texttt{Self-CoT}~\cite{kojima2022large} is a simple prompt trick that adds ``let's think step by step'' to the prompt to ask LLMs step by step output the reasoning process.
\texttt{Auto-CoT}~\cite{zhang2022automatic} automatically construct demonstration in CoT format.
So it is worth noting that Auto-CoT is not suitable in the 0-shot setting, so we only test the performance in the 5-shot setting.
\texttt{Cheat-Naive} use ``Hint'' as one of the input.
Since ``Hint'' will not incur other information, only tell LLMs where is key information, so we regard Cheat-Naive as the upper bound of the existing Language Models.
\texttt{Self-Consistency}~\cite{wang2022self} propose to use voting supersedes the simple, naive greedy decoding used in earlier CoT prompting to output the mostly generated result by the model.
In the experiment, we generate ten different outputs using LLMs, and we ask model to generate the final result based on all the outputs.
\texttt{Complexity-CoT}~\cite{fu2022complexity} uses the longest reasoning steps among all the outputs produced for a question to generate the final output.
\texttt{Plan-and-Solve CoT~(PS-CoT)}~\cite{wang2023plan} functions by first deconstructing the question before seeking its solution. 
\texttt{Self-Question} is a method that we propose, in which, we require the model to first delve deeply into the information already available in the original text, ponder the link between this information and the problem, and finally ask the model to integrate its existing thoughts to formulate a response.

\textbf{Demonstration:}
Furthermore, we investigate the influence of in-context learning on the performance of the model.
To accomplish this, we carried out tests on each of the examination questions using demonstrations sampled from the training set.
For each test sample, we randomly selected 5 training samples to form a demonstration.
In this way, different models using various prompt settings would utilize the same 5-shot sample-based demonstration for the same question.
For Naive and Cheat-Naive approaches, we directly concatenate the sampled questions with the ``Answer'' or ``Hint'' to form demonstrations.
For Auto-CoT, we ask LLMs to generate the reasoning process of few-shot samples in the format of CoT and concate the CoT to the samples as a demonstration.
For examples about how we construct demonstrations are listed in Appendix

\input{figures/SQPerformance}


\subsection{Performance of Directly Finding Answers}

\subsection{Performance in Detecting Key Information}

\subsection{Performance in Finding Answers with Key Information Injection}

\input{figures/GPT4Verification}
\input{tables/tab_ablation}

\subsection{Case Study}
The case study is conducted as detailed in Appendix. 
Two cases are listed in Table~\ref{tab:case1} and Table~\ref{tab:case2}, and the analysis towards the cases is as follow: 
Since there is not much difference between self-CoT and naive reasoning, which results in similar outcomes.
After injecting the Hint, the model can accurately answer the questions due to the Hint's ability to eliminate distractions and highlight suspicious points.
PS-CoT, by extracting key variables from the context, can avoid the influence of distracting content, thus achieving good results. 
However, Self-Question, with its superior ability to perform deep reasoning and associations, can achieve better results in the example requiring deep reasoning.


==> latex/05.Experiments.03.tex <==
\input{tables/tab_prompt_experiments}
\input{tables/tab_finetune_experiments}
\input{figures/fig_perason}

\subsection{Models:}
考虑到Detective Reasoning Benchmark包含了中英双语的内容，我们挑选了如今在中文和英文上最有代表性的几个模型。
为了能够得到目前最强模型的能力，以及保证实验结果具有一定的可复现性，我们同时选用了API-based Model和Open Source-based Model来进行实验。(括号里表示的是我们在实验中使用的这些模型的简称。)
英语为主的模型有GPT4-turbo~（GPT4）~\cite{openai2023gpt4}, GPT3.5-turbo~(GPT35)~\cite{openaichatgpt}, Llama2-7b-Base~(llama2-base), llama2-7b-Chat~(llama2-chat)。
中文为主的模型有GLM4~~(GLM4)~\cite{zheng2023judging}, ChatGLM3-6b-Base~(chatglm3-base), ChatGLM3-6B-Chat~(chatglm3-chat)~\cite{xu2023wizardlm}
其中，我们在2024年1月10日至29日期间使用了GPT4-turbo, GPT-3.5-turbo, GLM-4的官方API。

\subsection{Prompt-Based Enhanced Performance}
\subsubsection{Experiments Setup}
\textbf{Baselines}
我们挑选了一些Prompt Engineer方法作为对比。
\texttt{Naive}是简单地向 LLMs 输入``Context'', ``Question'' 和 ``Options''，并要求回答。
\texttt{Naive \w Key Information}使用 ``Clue Graph''中的 ``Key Information''作为输入之一。
目标是观察告诉``Key Information''对于大模型在面对Information Overload场景下的Multi-hop推理能力的影响。
\texttt{Naive \w Answer}直接讲``Answer''告诉大模型，来判断大模型在已知答案后，能否推断出``Key Information''是哪些。
\texttt{Self-CoT}~\cite{kojima2022large}是一个简单的提示技巧，它在提示语中添加了 "让我们一步一步地思考"，要求LLM一步一步地输出推理过程。
\texttt{Auto-CoT}~\cite{zhang2022automatic}会自动构建CoT格式的演示。
值得注意的是，Auto-CoT 并不适合在 0 次拍摄的情况下使用，因此我们只测试了在 5 次拍摄的情况下的性能。
\texttt{Self-Consistency}~\cite{wang2022self}建议使用投票取代早期CoT提示中使用的简单、天真的贪婪解码，以输出模型生成的大部分结果。
在实验中，我们使用 LLM 生成了十种不同的输出，并要求模型根据所有输出生成最终结果。
\texttt{Complexity-CoT}~\cite{fu2022complexity}使用一个问题的所有输出中最长的推理步骤来生成最终输出。
\texttt{Plan-and-Solve CoT~(PS-CoT)}~cite{wang2023plan} 的功能是先解构问题，然后再寻求问题的解决方案。
\texttt{Self-Question~(SQ)}是我们提出的一种方法，在这种方法中，我们要求模型首先深入研究原文中已有的信息，思考这些信息与问题之间的联系，最后要求模型整合已有的想法，形成一个回应。在实验中，我们主要采用的是单轮对话的形式，在采用多轮对话时，会额外注明。

有些有名的能够用于增强模型逻辑推理的方法，如ToT、GoT，存在自验证的过程，并不满足Detective Reasoning Benchmark的题目设置，所以我们没有作为baseline进行比较。
另外还有些需要将模型的错误回复反复注入的方法，如Reflexion，因为总共就4选1，反复注入将极大程度提高模型蒙对题目的概率，因此我们也没有考虑与其进行比较。

\textbf{Demonstration:}
此外，我们还研究了Demonstration对模型性能的影响。
为此，我们使用从训练集中抽取的演示对每道试题进行了测试。
对于每个测试样本，我们随机抽取3个训练样本组成一个演示。
对于 Naive Prompt方法，我们直接将答案接在训练数据后面，然后再提问前连续输入3个示例。
对于 Auto-CoT，我们要求 LLM 在给定``Context'', ``Question''和 ``Answer''的前提下，生成推理过程，并将推理过程融入与样本连接起来作为演示。
有关我们如何构建演示的示例见附录。

\subsubsection{Analysis}
\textbf{Not All Prompt Engineer Improve Models' Performance:} 
从表~\ref{tab:prompt_experiments}的结果来看，各个闭源的大模型，如GPT4、GPT3.5和GLM4的表现要比目前主流的开源的大模型如Chatglm3、llama2表现要好。
在我们的实验中，GPT4和GLM4在使用Prompt Engineer后，其准确率分别都有所提升，与之相对的是，一些经典的工作，如Self-CoT在GPT3.5、Chatglm3、llama2上都有所下降，下降幅度在1\%-4\%之间
这可能是因为当模型本身具备了较高水平的认知能力之后，再在信息检索和推理的任务上利用prompt对其思想过程合理诱导，可以促使模型进行更合理地思考，从而得到更好的结果。
而如果模型本身不具备推理能力，模型在回答问题时可能会从字符相似度等其他角度取巧去进行回答，而这时候通过prompt来强行要求模型进行推理，反而损伤了模型的性能。

\textbf{Most Models do poor in Key Information Detection:} 
我们发现，几乎所有的模型在发现Key Information时表现都非常差。
即便是GPT4-Turbo在Key Information检测任务上的平均准确率仅为40\%。
虽然回答正确题目不一定要能够正确地找到Key Information，但如图~\ref{fig:perason}所示，模型在找到Key Information和正确回答问题之间依然有着正比关系。
而当我们将Key Information直接注入给模型时，以GPT4为例，模型找对Key Information的RougeL分数能上升21\%，同时模型的回答准确率能够上升8.3\%，这说明找对Key Information对于解题非常关键。
而当我们直接将答案告诉模型后，大多数模型依然无法正确地找到Key Information。

\textbf{Demonstration Often Make Model perform poorer:}
曾经很流行使用Demonstration来使模型理解输出的格式，从而能更好地从模型的回复中解析出答案。
但如今，当模型越来越具备遵从复杂指令的要求之后，Demonstration已经无法进一步提升模型的表现。
实验显示许多prompt method在加入了3-shot demonstration之后都会出现效果下降，从闭源的能力较强的模型再到开源模型无一例外，Demonstration展现出了非常不稳定的性能。

\textbf{Self-Question Prompt Improve Both Key Information Detection Ability And Commonsense Reasoning Ability} 
与其他所有的Prompt Engineer对比，Self-Question表现非常亮眼。在我们的实验中，使用Self-Question Prompt的模型在关键信息检测和常识推理能力上都有显著的提升。
在表现最好的模型上使用Self-Question Prompt，其在关键信息检测任务上的准确率提升了1.1\%，在模型最终表现的准确率上提升了5\%。
除此之外，Self-Question Prompt在绝大多数的模型上都证明了自己要比其他prompt method要好，这表明Self-Question Prompt能够有效地提升模型理解Context、发现Context中的重要信息，并进行深度推理的能力。


\input{figures/fig_analysis}
\subsection{Finetune-Based Enhanced Performance}
\subsubsection{Experiments Setup}
\textbf{Baselines}
在这章中，考虑到我们需要微调模型，以及保证实验的可复现性，所以我们使用了四个知名的开源模型进行了进一步的实验。
实验主要是验证直接使用Self-Question Prompt~（SQ Prompt）、在多轮对话中使用Self-Question Prompt~(SQ Prompt w/ MR Chat)、利用Detective Reasoning Benchmark的数据进行Self-Question Finetune~(SQ FT w/ Detective)、以及使用Detective Reasoning Benchmark中的Context、Question、Answer让模型自己生成Self-Question Finetune数据~(SQ FT w/ Generated)。
每种方法具体的prompt我们将会放在Appendix中。


值得一提的是，我们实验主要是验证Self-Question Finetune能否增强模型在发现Key Information和Commonsense Reasoning的能力。
因此我们只使用了训练集中的400个样本在AdamW优化器下训练了2个epoch来验证效果。
具体我们训练模型的细节，我们放在Appendix中。

\subsubsection{Analysis}

\textbf{将单轮对话拆成多轮对话将会有害于Chat模型的表现，但有助于Base模型的表现} 
在我们的实验中，我们发现将单轮对话拆分成多轮对话对模型的表现产生了负面影响。
具体来说，当我们将单轮对话拆分成多轮对话后，Chat模型的准确率平均下降了1.3\%，而base模型的准确率平均上升了3.0\%。
这可能是因为Base模型对于所有的context信息都非常敏感，将Self-Question拆成多轮对话之后可以有助于帮助模型过滤无意义的信息。
而Chat模型具有一定的发型Key Information的能力，因此将Self-Question拆成多轮对话之后，会因为丢失了一定的信息而降低了表现。

\textbf{直接使用Detective Reasoning Benchmark的数据进行Self-Question Finetune可以全方位提升模型的Key Infomation Detection能力和Commonsense Reasoning能力}
我们发现，直接使用Detective Reasoning Benchmark的数据进行Self-Question Finetune可以显著提升模型的Key Infomation Detection能力和Commonsense Reasoning能力。
在我们的实验中，使用Detective Reasoning Benchmark的数据进行Self-Question Finetune后，模型在关键信息检测任务上的准确率平均提升了15.2\%，在模型的最终表现上准确率平局提升了10.5\%。
这表明Detective Reasoning Benchmark的数据集非常适合用于同时提升模型的信息检索和常识推理能力。

% \textbf{针对于chat模型的微调将会带来更好的效果} 我们的实验结果也显示，针对chat模型的微调可以带来更好的效果。在我们的实验中，针对chat模型进行微调后，模型的准确率平均提升了15\%，并且在关键信息检测和常识推理任务上的表现也有显著提升。这可能是因为chat模型在处理对话任务时，需要理解和生成更加自然和流畅的对话，而微调可以帮助模型更好地适应这种任务需求。



\subsection{Detailed Analysis}
\subsubsection{影响模型表现的因素} 
如图~\ref{fig:gpt4_performance}从四个维度分别展示了目前效果最好的模型GPT4-Turbo在Detective Reasoning Benchmark上的表现受什么影响。
我们发现，随着Context Length反应了潜在关键信息的数量、发现关键信息的复杂度等从400字增长到800字，模型的表现下降得比较明显，平均准确率从65\%左右下降到了35\%左右。
而Options Length一定程度上反应了推理的复杂度，当选项总长度过短或者过长时，模型都表现得不是很好。

前两者是根据题目本身直接能判断的题目难度，而我们进一步又使用了我们的标注来分析模型的表现。
随着标注的Key Information的数量从5个增多到10多个个，模型表现下降非常明显。
同样，推理深度从9层增加到26层，模型的准确率也从60\%下降到了25\%左右，即随机猜测的准确率。
这些结果表明，我们的标注结果和模型的表现之间具有较高的一致性。
Key Information的数量和推理深度确实能够反应题目的复杂程度。

\subsubsection{在不同问题上的表现结果} 图~\ref{fig:performance_category}
展示了五个模型在九个问题上的不同表现。
可以看到，所有模型都几乎非常擅长回答Why、Where之类的问题，经过微调后的llama-2平均都准确率达到了90\%。
而模型在回答Who、which、以及一些其他类型的问题的时候表现却非常差，平均准确率只有50\%。
这可能是因为Why、Where之类的题目涉及到对于客观手法、环境的理解，而Who、Which这类问题需要模型具有更强的实体识别和关系理解能力，而目前的模型在这方面的能力还有待提高。


% \subsubsection{Case Study}
% The case study is conducted as detailed in Appendix. 
% Two cases are listed in Table~\ref{tab:case1} and Table~\ref{tab:case2}, and the analysis towards the cases is as follow: 
% Since there is not much difference between self-CoT and naive reasoning, which results in similar outcomes.
% After injecting the Hint, the model can accurately answer the questions due to the Hint's ability to eliminate distractions and highlight suspicious points.
% PS-CoT, by extracting key variables from the context, can avoid the influence of distracting content, thus achieving good results. 
% However, Self-Question, with its superior ability to perform deep reasoning and associations, can achieve better results in the example requiring deep reasoning.

% \input{tables/tab_case1}

==> latex/05.Experiments.04.tex <==
\input{tables/tab_prompt_experiments}
\input{tables/tab_finetune_experiments}
\input{figures/fig_perason}

\subsection{Overall Setup}
\textbf{Models:}
为了能够得到目前最强模型的能力，以及保证实验结果具有一定的可复现性，我们同时选用了几个知名的API-based Model和Open Source-based Model来进行实验~(括号里表示的是我们在实验中使用的这些模型的简称。)：
GPT4-turbo~（GPT4）~\cite{openai2023gpt4}, GPT3.5-turbo~(GPT35)~\cite{openaichatgpt}, Llama2-7b-Base~(llama2-base), llama2-7b-Chat~(llama2-chat)。GLM4~~(GLM4)~\cite{zheng2023judging}, ChatGLM3-6b-Base~(chatglm3-base), ChatGLM3-6B-Chat~(chatglm3-chat)~\cite{xu2023wizardlm}。
其中，我们在2024年1月10日至29日期间使用了GPT4-turbo, GPT-3.5-turbo, GLM-4的官方API。

\textbf{Metrics:}
Detective Reasoning Benchmark本身包含了四选一的选择题，我们用Accuracy来标注模型从Options中选择正确答案的概率~(Acc.)。
另外，我们期望评估模型对于关键信息发现的能力~（KeyInfo.），而在标注的数据中，``Key Information from Context''是来源于``Context''的关键信息，所以基于Detective Reasoning Benchmark的关键信息发现也可以视作机器阅读理解任务使用Accuracy来进行评估。
但实验中，我们发现大多数模型并没有直接生成``Context''中固定一段内容的能力，所以我们最终采用RougeL进行评估。



\subsection{Prompt-Based Enhanced Performance}
\subsubsection{Experiments Setup}
\textbf{Baselines}
我们挑选了一些Prompt Engineer方法作为对比。
\texttt{Naive}是简单地向 LLMs 输入``Context'', ``Question'' 和 ``Options''，并要求回答。
\texttt{Self-CoT}~\cite{kojima2022large}是一个简单的提示技巧，它在提示语中添加了 "让我们一步一步地思考"，要求LLM一步一步地输出推理过程。
\texttt{Auto-CoT}~\cite{zhang2022automatic}会自动构建CoT格式的演示。
值得注意的是，Auto-CoT 并不适合在 0 次拍摄的情况下使用，因此我们只测试了在 5 次拍摄的情况下的性能。
\texttt{Self-Consistency}~\cite{wang2022self}建议使用投票取代早期CoT提示中使用的简单、天真的贪婪解码，以输出模型生成的大部分结果。在实验中，我们使用 LLM 生成了五种不同的输出，并要求模型根据所有输出生成最终结果。
\texttt{Complexity-CoT}~\cite{fu2022complexity}使用一个问题的所有输出中最长的推理步骤来生成最终输出。
\texttt{Plan-and-Solve CoT~(PS-CoT)}~cite{wang2023plan} 的功能是先解构问题，然后再寻求问题的解决方案。
\texttt{Self-Question~(SQ)}是我们提出的一种方法，在这种方法中，我们要求模型首先深入研究原文中已有的信息，思考这些信息与问题之间的联系，最后要求模型整合已有的想法，形成一个回应。在实验中，我们主要采用的是单轮对话的形式，在采用多轮对话时，会额外注明。
\texttt{Naive \w Key Information}使用 ``Clue Graph''中的 ``Key Information''作为输入之一。
目标是观察告诉``Key Information''对于大模型在面对Information Overload场景下的Multi-hop推理能力的影响。
\texttt{Naive \w Answer}直接讲``Answer''告诉大模型，来判断大模型在已知答案后，能否推断出``Key Information''是哪些。

有些有名的能够用于增强模型逻辑推理的方法，如Tree of Thought~\cite{yao2023tot}、Graph of Thought~\cite{besta2023got}，存在自验证的过程，并不满足Detective Reasoning Benchmark的题目设置，所以我们没有作为baseline进行比较。
另外还有些需要将模型的错误回复反复注入的方法，如Reflexion~\cite{shinn2023reflexion}，因为总共就4选1，反复注入将极大程度提高模型蒙对题目的概率，因此我们也没有考虑与其进行比较。

\textbf{Demonstration:}
此外，我们还研究了Demonstration对模型性能的影响。
为此，我们使用从训练集中抽取的演示对每道试题进行了测试。
对于每个测试样本，我们随机抽取3个训练样本组成一个演示。
对于 Naive Prompt方法，我们直接将答案接在训练数据后面，然后再提问前连续输入3个示例。
对于 Auto-CoT，我们要求 LLM 在给定``Context'', ``Question''和 ``Answer''的前提下，生成推理过程，并将推理过程融入与样本连接起来作为演示。

\subsubsection{Analysis}
\textbf{Not All Prompt Engineer Improve Models' Performance:} 
从表~\ref{tab:prompt_experiments}的结果来看，各个闭源的大模型，如GPT4、GPT3.5和GLM4的表现要比目前主流的开源的大模型如Chatglm3、llama2表现要好。
在我们的实验中，GPT4和GLM4在使用Prompt Engineer后，其准确率分别都有所提升，与之相对的是，一些经典的工作，如Self-CoT在GPT3.5、Chatglm3、llama2上都有所下降，下降幅度在1\%-4\%之间
这可能是因为当模型本身具备了较高水平的认知能力之后，再在信息检索和推理的任务上利用prompt对其思想过程合理诱导，可以促使模型进行更合理地思考，从而得到更好的结果。
而如果模型本身不具备推理能力，模型在回答问题时可能会从字符相似度等其他角度取巧去进行回答，而这时候通过prompt来强行要求模型进行推理，反而损伤了模型的性能。

\textbf{Most Models do poor in Key Information Detection:} 
我们发现，几乎所有的模型在发现Key Information时表现都非常差。
即便是GPT4-Turbo在Key Information检测任务上的平均准确率仅为40\%。
虽然回答正确题目不一定要能够正确地找到Key Information，但如图~\ref{fig:perason}所示，模型在找到Key Information和正确回答问题之间依然有着正比关系。
而当我们将Key Information直接注入给模型时，以GPT4为例，模型找对Key Information的RougeL分数能上升21\%，同时模型的回答准确率能够上升8.3\%，这说明找对Key Information对于解题非常关键。
而当我们直接将答案告诉模型后，大多数模型依然无法正确地找到Key Information。

\textbf{Demonstration Often Make Model perform poorer:}
曾经很流行使用Demonstration来使模型理解输出的格式，从而能更好地从模型的回复中解析出答案。
但如今，当模型越来越具备遵从复杂指令的要求之后，Demonstration已经无法进一步提升模型的表现。
实验显示许多prompt method在加入了3-shot demonstration之后都会出现效果下降，从闭源的能力较强的模型再到开源模型无一例外，Demonstration展现出了非常不稳定的性能。

\textbf{Self-Question Prompt Improve Both Key Information Detection Ability And Commonsense Reasoning Ability} 
与其他所有的Prompt Engineer对比，Self-Question表现非常亮眼。在我们的实验中，使用Self-Question Prompt的模型在关键信息检测和常识推理能力上都有显著的提升。
在表现最好的模型上使用Self-Question Prompt，其在关键信息检测任务上的准确率提升了1.1\%，在模型最终表现的准确率上提升了5\%。
除此之外，Self-Question Prompt在绝大多数的模型上都证明了自己要比其他prompt method要好，这表明Self-Question Prompt能够有效地提升模型理解Context、发现Context中的重要信息，并进行深度推理的能力。


\input{figures/fig_analysis}
\subsection{Finetune-Based Enhanced Performance}
\subsubsection{Experiments Setup}
\textbf{Baselines}
在这章中，考虑到我们需要微调模型，以及保证实验的可复现性，所以我们使用了四个知名的开源模型进行了进一步的实验。
实验主要是验证直接使用Self-Question Prompt~（SQ Prompt）、在多轮对话中使用Self-Question Prompt~(SQ Prompt w/ MR Chat)、利用Detective Reasoning Benchmark的数据进行Self-Question Finetune~(SQ FT w/ Detective)、以及使用Detective Reasoning Benchmark中的Context、Question、Answer让模型自己生成Self-Question Finetune数据~(SQ FT w/ Generated)。
每种方法具体的prompt我们将会放在Appendix中。


值得一提的是，我们实验主要是验证Self-Question Finetune能否增强模型在发现Key Information和Commonsense Reasoning的能力。
因此我们只使用了训练集中的400个样本在AdamW优化器下训练了2个epoch来验证效果。
具体我们训练模型的细节，我们放在Appendix中。

\subsubsection{Analysis}

\textbf{将单轮对话拆成多轮对话将会有害于Chat模型的表现，但有助于Base模型的表现} 
在我们的实验中，我们发现将单轮对话拆分成多轮对话对模型的表现产生了负面影响。
具体来说，当我们将单轮对话拆分成多轮对话后，Chat模型的准确率平均下降了1.3\%，而base模型的准确率平均上升了3.0\%。
这可能是因为Base模型对于所有的context信息都非常敏感，将Self-Question拆成多轮对话之后可以有助于帮助模型过滤无意义的信息。
而Chat模型具有一定的发型Key Information的能力，因此将Self-Question拆成多轮对话之后，会因为丢失了一定的信息而降低了表现。

\textbf{直接使用Detective Reasoning Benchmark的数据进行Self-Question Finetune可以全方位提升模型的Key Infomation Detection能力和Commonsense Reasoning能力}
我们发现，直接使用Detective Reasoning Benchmark的数据进行Self-Question Finetune可以显著提升模型的Key Infomation Detection能力和Commonsense Reasoning能力。
在我们的实验中，使用Detective Reasoning Benchmark的数据进行Self-Question Finetune后，模型在关键信息检测任务上的准确率平均提升了15.2\%，在模型的最终表现上准确率平局提升了10.5\%。
这表明Detective Reasoning Benchmark的数据集非常适合用于同时提升模型的信息检索和常识推理能力。


\subsection{Detailed Analysis}
\subsubsection{影响模型表现的因素} 
如图~\ref{fig:gpt4_performance}从四个维度分别展示了目前效果最好的模型GPT4-Turbo在Detective Reasoning Benchmark上的表现受什么影响。
我们发现，随着Context Length反应了潜在关键信息的数量、发现关键信息的复杂度等从400字增长到800字，模型的表现下降得比较明显，平均准确率从65\%左右下降到了35\%左右。
而Options Length一定程度上反应了推理的复杂度，当选项总长度过短或者过长时，模型都表现得不是很好。

前两者是根据题目本身直接能判断的题目难度，而我们进一步又使用了我们的标注来分析模型的表现。
随着标注的Key Information的数量从5个增多到10多个个，模型表现下降非常明显。
同样，推理深度从9层增加到26层，模型的准确率也从60\%下降到了25\%左右，即随机猜测的准确率。
这些结果表明，我们的标注结果和模型的表现之间具有较高的一致性。
Key Information的数量和推理深度确实能够反应题目的复杂程度。

\subsubsection{在不同问题上的表现结果} 图~\ref{fig:performance_category}
展示了五个模型在九个问题上的不同表现。
可以看到，所有模型都几乎非常擅长回答Why、Where之类的问题，经过微调后的llama-2平均都准确率达到了90\%。
而模型在回答Who、which、以及一些其他类型的问题的时候表现却非常差，平均准确率只有50\%。
这可能是因为Why、Where之类的题目涉及到对于客观手法、环境的理解，而Who、Which这类问题需要模型具有更强的实体识别和关系理解能力，而目前的模型在这方面的能力还有待提高。



==> latex/05.Experiments.05.tex <==
\input{tables/tab_prompt_experiments}
\input{tables/tab_finetune_experiments}
\input{figures/fig_perason}

\subsection{Experimental Framework}

\textbf{Models:} 
In pursuit of harnessing the capabilities of the most advanced models available, and to ensure a degree of replicability in our experimental outcomes, we employed a selection of renowned models from both API-based and Open Source categories for our experimentation. These models, referred to by their abbreviations in parentheses, include: GPT4-turbo (GPT4)\cite{openai2023gpt4}, GPT3.5-turbo (GPT35)\cite{openaichatgpt}, Llama2-7b-Base (llama2-base), Llama2-7b-Chat (llama2-chat), GLM4 (GLM4)\cite{zheng2023judging}, ChatGLM3-6b-Base (chatglm3-base), and ChatGLM3-6B-Chat (chatglm3-chat)\cite{xu2023wizardlm}. Notably, the official APIs of GPT4-turbo, GPT-3.5-turbo, and GLM-4 were utilized for experimentation during the period from January 10 to January 29, 2024.

\textbf{Metrics:} 
The Detective Reasoning Benchmark, which comprises multiple-choice questions with four options, utilizes Accuracy as a metric to denote the probability of a model selecting the correct answer from the given options (Acc.). Additionally, we aimed to assess the models' proficiency in identifying key information (KeyInfo.), where "Key Information from Context" pertains to the crucial information derived from the "Context." Thus, the task of identifying key information based on the Detective Reasoning Benchmark can also be considered a machine reading comprehension task, evaluated using Accuracy. However, during our experiments, it was observed that most models lacked the capability to generate a fixed segment of content directly from the "Context." Consequently, we opted to use RougeL for evaluation in these instances.



\subsection{Enhancement of Performance through Prompt Engineering}
\subsubsection{Experimental Configuration}
\textbf{Baselines:}
For comparative analysis, various prompt engineering methods were selected. 
\begin{itemize}
    \item \texttt{Naive} method involves simply inputting the "Context," "Question," and "Options" to large language models (LLMs) and requesting an answer.
    \item \texttt{Self-CoT} approach~\cite{kojima2022large} employs a simple prompting trick that incorporates "Let's think step by step" into the prompt, asking the LLM to sequentially articulate the reasoning process.
    \item \texttt{Auto-CoT}\cite{zhang2022automatic} automatically constructs a Chain of Thought (CoT) format demonstration. Notably, Auto-CoT is not designed for zero-shot scenarios, thus, its performance was only evaluated in a five-shot setting.
    \item 
\end{itemize}
The \texttt{Naive} method involves simply inputting the "Context," "Question," and "Options" to large language models (LLMs) and requesting an answer. The \texttt{Self-CoT} approach~\cite{kojima2022large} employs a simple prompting trick that incorporates "Let's think step by step" into the prompt, asking the LLM to sequentially articulate the reasoning process. \texttt{Auto-CoT}\cite{zhang2022automatic} automatically constructs a Chain of Thought (CoT) format demonstration. Notably, Auto-CoT is not designed for zero-shot scenarios, thus, its performance was only evaluated in a five-shot setting. The \texttt{Self-Consistency} method\cite{wang2022self} suggests replacing the simple, naive greedy decoding used in early CoT prompts with a voting mechanism to determine the majority outcome from model-generated outputs. In our experiments, five different outputs were generated using an LLM, and the model was tasked with synthesizing a final response based on all outputs. \texttt{Complexity-CoT}\cite{fu2022complexity} generates the final output using the longest reasoning steps among all outputs for a question. \texttt{Plan-and-Solve CoT (PS-CoT)}\cite{wang2023plan} functions by deconstructing the problem before seeking solutions. \texttt{Self-Question (SQ)} is a method we propose, wherein the model is first asked to delve into the information present within the original text, ponder the connections between this information and the question, and ultimately synthesize the existing ideas to form a response. In our experiments, a single-round dialogue format was primarily used, with multi-round dialogues explicitly indicated when applied. \texttt{Naive \w Key Information} incorporates "Key Information" from the "Clue Graph" as one of the inputs, aiming to observe the impact of providing "Key Information" on the multi-hop reasoning abilities of large models in scenarios of information overload. \texttt{Naive \w Answer} involves directly informing the large model of the "Answer" to assess its capability to deduce "Key Information" upon knowing the answer.

Several renowned methods capable of enhancing model logic reasoning, such as Tree of Thought~\cite{yao2023tot} and Graph of Thought~\cite{besta2023got}, involve a self-verification process and do not conform to the question setup of the Detective Reasoning Benchmark, hence were not compared as baselines. Additionally, methods requiring repeated injection of a model's erroneous replies, such as Reflexion~\cite{shinn2023reflexion}, were also not considered for comparison due to their potential to significantly increase the probability of the model guessing the correct answer in a four-choice scenario.

\textbf{Demonstration:}
Furthermore, the impact of demonstrations on model performance was investigated. For this purpose, demonstrations extracted from the training set were tested on each question. For each test sample, three training samples were randomly selected to form a demonstration. For the Naive Prompt method, answers were directly appended after the training data, with three examples inputted consecutively before posing the question. For Auto-CoT, the LLM was instructed to generate a reasoning process given the "Context," "Question," and "Answer," and this reasoning process was integrated with the samples to serve as a demonstration.

\subsubsection{Analysis}
\textbf{Not All Prompt Engineering Methods Improve Model Performance:}
Results from Table~\ref{tab:prompt_experiments} indicate that closed-source large models such as GPT4, GPT3.5, and GLM4 outperform current mainstream open-source models like ChatGLM3 and Llama2. In our experiments, both GPT4 and GLM4 exhibited accuracy improvements when subjected to prompt engineering. Conversely, some classical works, such as Self-CoT, demonstrated a decline of 1\%-4\% in performance on GPT3.5, ChatGLM3, and Llama2. This decline suggests that when a model already possesses a high level of cognitive capability, further guiding its thought process through prompts in information retrieval and reasoning tasks can foster more rational thinking, thereby yielding better outcomes. If a model inherently lacks reasoning capabilities, it might resort to heuristics such as character similarity to answer questions, and forcibly prompting it to reason could actually impair its performance.

\textbf{Most Models Perform Poorly in Key Information Detection:}
It was observed that nearly all models exhibited poor performance in detecting Key Information, with GPT4-Turbo achieving an average accuracy of only 40\% in Key Information detection tasks. While correctly answering questions does not necessarily require correctly identifying Key Information, as illustrated in Figure~\ref{fig:perason}, there exists a proportional relationship between a model's ability to identify Key Information and correctly answer questions. When Key Information was directly fed to the models, for instance, GPT4, the RougeL score for correctly identifying Key Information increased by 21\%, and the accuracy of the model's answers rose by 8.3\%, highlighting the critical importance of correctly identifying Key Information for solving problems. However, even when the answers were directly provided to the models, most were still unable to correctly identify Key Information.

\textbf{Demonstrations Often Result in Poorer Model Performance:}
Demonstrations were once popular for helping models understand output formats, thereby facilitating easier parsing of answers from model responses. However, as models have become increasingly capable of following complex instructions, demonstrations no longer contribute to further performance enhancements. Experiments revealed that many prompt methods experienced a decline in effectiveness upon incorporating three-shot demonstrations, with both closed and open-source models exhibiting consistently unstable performance.

\textbf{The Self-Question Prompt Method Enhances Both Key Information Detection and Commonsense Reasoning Capabilities:}
Compared to all other prompt engineering methods, the Self-Question approach demonstrated exceptional performance. In our experiments, models utilizing the Self-Question prompt showed significant improvements in both key information detection and commonsense reasoning capabilities. Employing the Self-Question prompt on the best-performing models resulted in a 1.1\% increase in accuracy for key information detection tasks and a 5\% increase in overall model performance accuracy. Moreover, the Self-Question prompt proved superior to other prompt methods across the majority of models, indicating its effectiveness in enhancing models' abilities to understand context, identify critical information within it, and engage in in-depth reasoning.


\input{figures/fig_analysis}
\subsection{Enhanced Performance via Fine-Tuning}
\subsubsection{Experimental Setup}
\textbf{Baselines:}
In this chapter, considering the necessity to fine-tune models and to ensure the reproducibility of our experiments, we utilized four renowned open-source models for further experimentation. Our experiments primarily aimed to verify the effectiveness of directly using the Self-Question Prompt (SQ Prompt), employing the Self-Question Prompt in multi-round dialogues (SQ Prompt w/ MR Chat), utilizing the Detective Reasoning Benchmark data for Self-Question Fine-tuning (SQ FT w/ Detective), and generating Self-Question Fine-tune data using the Context, Question, and Answer from the Detective Reasoning Benchmark (SQ FT w/ Generated). Specific prompts used for each method will be detailed in the Appendix.

It is worth mentioning that our experiments primarily focused on verifying whether Self-Question Fine-tuning could enhance models' abilities in detecting Key Information and performing Commonsense Reasoning. Therefore, we used only 400 samples from the training set and trained for 2 epochs under the AdamW optimizer to validate the effects. Details of our training methodology are provided in the Appendix.

\subsubsection{Analysis}

\textbf{Splitting Single-Round Dialogues into Multi-Round Dialogues is Detrimental to Chat Models but Beneficial to Base Models:}
Our experiments revealed that splitting single-round dialogues into multi-round dialogues negatively impacted the performance of chat models, with an average accuracy decrease of 1.3\%, while base models saw an average accuracy increase of 3.0\%. This outcome may be attributed to base models being particularly sensitive to all contextual information, where splitting Self-Questions into multi-round dialogues could help filter out irrelevant information. Conversely, chat models, which possess a certain ability to identify Key Information, experienced performance degradation due to the loss of some information when the Self-Question was divided into multiple rounds.

\textbf{Directly Using Detective Reasoning Benchmark Data for Self-Question Fine-tuning Significantly Enhances Key Information Detection and Commonsense Reasoning Abilities:}
We discovered that directly using Detective Reasoning Benchmark data for Self-Question Fine-tuning significantly improved models' abilities in Key Information Detection and Commonsense Reasoning. After fine-tuning with Detective Reasoning Benchmark data, models showed an average accuracy improvement of 15.2\% in key information detection tasks and a 10.5\% average increase in overall model performance accuracy. This indicates that the Detective Reasoning Benchmark dataset is highly suitable for enhancing models' information retrieval and commonsense reasoning abilities.

\subsection{Detailed Analysis}
\subsubsection{Factors Influencing Model Performance}
As depicted in Figure~\ref{fig:gpt4_performance}, we analyzed the impact on the current best-performing model, GPT4-Turbo, on the Detective Reasoning Benchmark from four dimensions. We observed a significant performance decline as the Context Length, which reflects the quantity of potential Key Information and the complexity of its identification, increased from 400 to 800 words, with the average accuracy dropping from around 65\% to about 35\%. The Options Length, which somewhat indicates the complexity of reasoning, also showed that models performed poorly when the total length of options was either too short or too long.

The first two factors directly indicate the difficulty of questions based on the content itself, while we further analyzed model performance using our annotations. As the number of annotated Key Information increased from 5 to over 10, a significant decrease in model performance was evident. Similarly, as the reasoning depth increased from 9 to 26 layers, accuracy dropped from 60\% to around 25\%, which is close to the accuracy of random guessing. These results demonstrate a high consistency between our annotated results and model performance. The quantity of Key Information and the depth of reasoning indeed reflect the complexity of the questions.

\subsubsection{Performance Across Different Question Types}
Figure~\ref{fig:performance_category} illustrates the varying performance of five models across nine question types. It is evident that all models excel at answering questions like "Why" and "Where," with the fine-tuned Llama-2 model achieving an average accuracy of 90\%. However, models performed poorly when answering "Who," "Which," and other types of questions, with an average accuracy of only 50\%. This discrepancy may be due to the fact that questions like "Why" and "Where" involve understanding objective methods and environments, whereas questions like "Who" and "Which" require the models to possess stronger entity recognition and relational understanding capabilities, areas where current models still need improvement.



==> latex/05.Experiments.06.tex <==
\input{tables/tab_prompt_experiments}
\input{tables/tab_finetune_experiments}
\input{figures/fig_perason}

\subsection{Experimental Framework}

\textbf{Models:} 
In pursuit of harnessing the capabilities of the most advanced models available, and to ensure a degree of replicability in our experimental outcomes, we employed a selection of renowned models from both API-based and Open Source categories for our experimentation. These models, referred to by their abbreviations in parentheses, include: GPT4-turbo (GPT4)\cite{openai2023gpt4}, GPT3.5-turbo (GPT35)\cite{openaichatgpt}, Llama2-7b-Base (llama2-base), Llama2-7b-Chat (llama2-chat), GLM4 (GLM4)\cite{zheng2023judging}, ChatGLM3-6b-Base (chatglm3-base), and ChatGLM3-6B-Chat (chatglm3-chat)\cite{xu2023wizardlm}. Notably, the official APIs of GPT4-turbo, GPT-3.5-turbo, and GLM-4 were utilized for experimentation during the period from January 10 to January 29, 2024.

\textbf{Metrics:} 
The Detective Reasoning Benchmark, which comprises multiple-choice questions with four options, utilizes Accuracy as a metric to denote the probability of a model selecting the correct answer from the given options (Acc.). Additionally, we aimed to assess the models' proficiency in identifying key information (KeyInfo.), where "Key Information from Context" pertains to the crucial information derived from the "Context." Thus, the task of identifying key information based on the Detective Reasoning Benchmark can also be considered a machine reading comprehension task, evaluated using Accuracy. However, during our experiments, it was observed that most models lacked the capability to generate a fixed segment of content directly from the "Context." Consequently, we opted to use RougeL for evaluation in these instances.



\subsection{Enhancement of Performance through Prompt Engineering}
\subsubsection{Experimental Configuration}
\textbf{Baselines:}
For comparative analysis, various prompt engineering methods were selected. 
\texttt{\textbf{Naive}} method involves simply inputting the "Context," "Question," and "Options" to large language models (LLMs) and requesting an answer.
\texttt{\textbf{Self-CoT}}~\cite{kojima2022large} employs a simple  Chain of Thought (CoT) prompt that incorporates ``Let's think step by step'', asking the LLM to sequentially articulate the reasoning process.
\texttt{\textbf{Auto-CoT}}~\cite{zhang2022automatic} automatically constructs CoT format demonstration. Notably, Auto-CoT is not designed for zero-shot scenarios, thus, its performance was only evaluated in a three-shot setting.
\texttt{\textbf{Self-Consistency}}~\cite{wang2022self} suggests to summarize as many output as possible of the same model. In our experiments, five different outputs were generated using an LM, and the model was tasked with synthesizing a final response based on all outputs.
\texttt{\textbf{Complexity-CoT}}~\cite{fu2022complexity} generates the final output using the longest reasoning steps among all outputs for a question.
\texttt{\textbf{Plan-and-Solve CoT (PS-CoT)}}~\cite{wang2023plan} functions by deconstructing the problem before seeking solutions.
\texttt{\textbf{Self-Question Prompt}} is a method proposed in this paper.
\texttt{\textbf{Naive /w Key Info}} incorporates ``Key Information'' as one of the inputs. 
\texttt{\textbf{Naive /w Answer}} involves directly informing models of the ``Answer''.

Several renowned methods capable of enhancing model logic reasoning, such as Tree of Thought~\cite{yao2023tot} and Graph of Thought~\cite{besta2023got}, involve a self-verification process and do not conform to the question setup of the Detective Reasoning Benchmark, hence were not compared as baselines.
Additionally, methods requiring repeated injection of a model's erroneous replies, such as Reflexion~\cite{shinn2023reflexion}, were also not considered for comparison due to their potential to significantly increase the probability of the model guessing the correct answer in a four-choice scenario.

\textbf{Demonstration:}
Demonstration is a method employed within prompts for few-shot learning. It involves combining several questions that contain the correct answers in the same format as the test data and incorporating them into the prompt. This technique enhances the model's understanding of the output format and allows the model to acquire relevant knowledge by introducing a small number of samples. 
For the Naive Prompt method, answers were directly appended after the training data, with three examples inputted consecutively before posing the question. For Auto-CoT, the LLM was instructed to generate a reasoning process given the "Context," "Question," and "Answer," and this reasoning process was integrated with the samples to serve as a demonstration.
For specific examples and prompts, please refer to Appendix~\ref{appendix_prompt}.

\subsubsection{Analysis}
The performance of all baseline models with different prompt methods are shown in Tab.~\ref{tab:prompt_experiments}.

\textbf{The Efficacy of Prompt Engineering Methods in Enhancing Model Performance Varies:}
The data from Table~\ref{tab:prompt_experiments} reveals that proprietary large-scale models such as GPT4, GPT3.5, and GLM4 surpass the performance of prevalent open-source counterparts like ChatGLM3 and Llama2. In our analysis, GPT4 and GLM4 showed notable accuracy enhancements with the application of prompt engineering techniques. However, established methodologies like Self-CoT experienced a 1\%-4\% performance decrement in models including GPT3.5, ChatGLM3, and Llama2. This suggests that advanced cognitive models benefit from prompt-based guidance in information retrieval and reasoning tasks, improving rationality in outcomes. Conversely, models with limited reasoning faculties may rely on tricky approaches, such as character similarity for question answering, where enforced reasoning prompts can detrimentally affect performance.

\textbf{Deficiencies in Key Information Detection Across Models:}
Our observations indicate a widespread deficiency among models in key information detection, with GPT4-Turbo achieving merely 40\% average accuracy in these tasks. 
Although accurate question answering does not strictly necessitate precise key information identification, a proportional relationship is evident between the ability to discern key information and the accuracy of responses as depicted in Figure~\ref{fig:perason}. 
Directly supplying key information to models, for example, to GPT4, resulted in a 21\% increase in RougeL scores for key information identification and an 8.3\% improvement in answer accuracy, underscoring the vital role of accurate key information detection in problem-solving. Nonetheless, most models failed to accurately identify key information even when answers were explicitly provided.

\textbf{Diminished Returns from Demonstrations in Modern Model Performance:}
Historically, demonstrations were utilized to clarify expected output formats, aiding models in parsing responses more effectively. 
Yet, with models evolving to adeptly follow intricate directives, the addition of demonstrations no longer enhances performance. 
Our testing indicated a decline in the utility of various prompt methods upon integrating three-shot demonstrations, with both proprietary and open-source models showing erratic performance fluctuations.

\textbf{Superiority of the Self-Question Prompt Method in Boosting Detection and Reasoning:}
Among the evaluated prompt engineering strategies, the Self-Question technique stands out for its superior efficacy. Models employing this method recorded significant enhancements in both key information detection and commonsense reasoning. Application of the Self-Question prompt on top-performing models led to a 1.1\% increase in key information detection accuracy and a 5\% boost in overall accuracy. This method's predominance over others in a majority of models signifies its potency in augmenting context comprehension, critical information identification, and profound reasoning capabilities.


\input{figures/fig_analysis}
\subsection{Performance Enhancement through Model Fine-Tuning}
\subsubsection{Experimental Design}
\textbf{Baselines:}
This study employs four distinguished open-source models to investigate the impact of fine-tuning on enhancing model capabilities. Our exploration focuses on evaluating the efficacy of direct application of the Self-Question Prompt (SQ Prompt), utilization of the SQ Prompt within multi-round dialogues (SQ Prompt w/ MR Chat), fine-tuning with Detective Reasoning Benchmark data (SQ FT w/ Detective), and generating fine-tuning data via the Detective Reasoning Benchmark's Context, Question, and Answer (SQ FT w/ Generated). Detailed descriptions of the prompts used for each method are provided in the Appendix.

The primary objective of these experiments is to assess the potential of Self-Question Fine-tuning in augmenting models' key information detection and commonsense reasoning skills. For validation purposes, we employed a subset of 400 samples from the training dataset and conducted training over 2 epochs using the AdamW optimizer. The comprehensive training methodology is elucidated in the Appendix.

\subsubsection{Analysis}

\textbf{The Impact of Transitioning from Single-Round to Multi-Round Dialogues:}
Our findings indicate that converting single-round dialogues into multi-round ones adversely affects chat models, decreasing average accuracy by 1.3\%, whereas base models experienced a 3.0\% improvement in average accuracy. This suggests that base models, which are more receptive to comprehensive contextual information, benefit from the division of Self-Questions into multiple rounds as it aids in filtering extraneous details. Chat models, however, suffer from a diminution in performance due to the segmented presentation of Self-Questions, resulting in the potential loss of crucial information.

\textbf{Significant Advancements with Detective Reasoning Benchmark Data in Self-Question Fine-Tuning:}
Employing Detective Reasoning Benchmark data for Self-Question Fine-tuning markedly amplifies models' proficiency in key information detection and commonsense reasoning. Post fine-tuning, models exhibited a 15.2\% enhancement in key information detection accuracy and a 10.5\% rise in overall performance accuracy. These outcomes affirm the Detective Reasoning Benchmark dataset's aptness for bolstering models' capabilities in information retrieval and commonsense reasoning.

\subsection{Comprehensive Analysis}
\subsubsection{Determinants of Model Performance}
Figure~\ref{fig:gpt4_performance} delineates the impact on GPT4-Turbo, the foremost model, across four dimensions on the Detective Reasoning Benchmark. A notable performance decrement was observed with an increase in Context Length from 400 to 800 words, causing average accuracy to plummet from approximately 65\% to 35\%. Similarly, the Options Length's variation revealed models' struggles with reasoning complexity when options were too brief or extensive.

These first two dimensions primarily reflect question difficulty based on content, whereas further analysis via our annotations revealed a direct correlation between annotated Key Information quantity, reasoning depth, and model performance. A discernible performance decline correlated with an increase in Key Information count and reasoning depth, demonstrating the consistency between our annotations and model efficacy. These factors, namely the quantity of Key Information and reasoning depth, significantly contribute to question complexity.

\subsubsection{Divergent Performance Across Question Categories}
Figure~\ref{fig:performance_category} showcases the disparate performance of five models across nine question types, highlighting proficiency in "Why" and "Where" questions with the fine-tuned Llama-2 model reaching an average accuracy of 90\%. Contrastingly, the models' performance on "Who," "Which," and similar questions was notably weaker, averaging only 50\% accuracy. This variance suggests that "Why" and "Where" questions necessitate an understanding of objective processes and settings, whereas "Who" and "Which" questions demand more advanced entity recognition and relational understanding, areas where current models exhibit limitations.



==> latex/05.Experiments.07.tex <==
\input{tables/tab_prompt_experiments}
\input{tables/tab_finetune_experiments}
\input{figures/fig_perason}


\subsection{Overall Setup}

\textbf{Models:}
In our quest to leverage the most sophisticated models for enhanced replicability and robustness in results, we utilized a suite of eminent models from both the API-based and Open Source domains. These include GPT4-turbo (GPT4)~\cite{openai2023gpt4}, GPT3.5-turbo (GPT35)~\cite{openaichatgpt}, Llama2-7b-Base (llama2-base), Llama2-7b-Chat (llama2-chat)~\cite{touvron2023llama}, GLM4 (GLM4)~\cite{zheng2023judging}, ChatGLM3-6b-Base (chatglm3-base), and ChatGLM3-6B-Chat (chatglm3-chat)~\cite{xu2023wizardlm}. The experimentation was conducted using the official APIs for GPT4-turbo, GPT-3.5-turbo, and GLM-4 between January 10 and January 29, 2024.

\textbf{Metrics:}
The DetectBench, comprised of multiple-choice questions, employs Accuracy as the metric for evaluating the likelihood of model correctness in answer selection. Additionally, the benchmark assesses models' ability to identify crucial information from the context, a task akin to machine reading comprehension, using Accuracy for evaluation. However, given the challenge in direct content segment generation from ``Context'', RougeL was utilized for evaluations where applicable.

\subsection{Performance with Different Prompt Engineering}
\subsubsection{Experimental Setup}
\textbf{Baselines:}
A range of prompt engineering methods were analyzed for comparative insights. These include:

\texttt{\textbf{Naive}}, which simply inputs ``Context'', ``Question'', and ``Options'' into LLMs for answers.
\texttt{\textbf{Self-CoT}}~\cite{kojima2022large}, applying a step-by-step reasoning prompt.
\texttt{\textbf{Auto-CoT}}~\cite{zhang2022automatic}, which automates Chain of Thought (CoT) demonstrations, evaluated in a three-shot setting due to its non-zero-shot design.
\texttt{\textbf{Self-Consistency}}~\cite{wang2022self}, summarizing multiple outputs from the same model to derive a final answer.
\texttt{\textbf{Complexity-CoT}}~\cite{fu2022complexity}, selecting the longest reasoning steps among all outputs.
\texttt{\textbf{Plan-and-Solve CoT (PS-CoT)}}, focusing on problem deconstruction before solution.
\texttt{\textbf{Self-Question Prompt}}~\cite{wang2023plan}, introduced in this study.
\texttt{\textbf{Naive /w Key Info}} and \texttt{\textbf{Naive /w Answer}}, enhancing inputs with ``Key Information'' and the ``Answer'' respectively.

Methods involving self-verification processes, such as Tree of Thought~\cite{yao2023tot} and Graph of Thought~\cite{besta2023got}, and those increasing correct answer probability through model error injections, like Reflexion~\cite{shinn2023reflexion}, were excluded due to incompatibility with the benchmark's question setup or potential bias in a four-choice format.

\textbf{Demonstration:}
Demonstration incorporates correct answers in test data format and a small number of examples to improve output format comprehension and knowledge acquisition. The Naive Prompt method appends answers after training data examples, while Auto-CoT guides the LLM to generate reasoning processes aligned with the ``Context'', ``Question'' and ``Answer''.

\subsubsection{Analysis}
Tab.~\ref{tab:prompt_experiments} displays the performance of all baseline models across different prompt methods.

\textbf{Varied Prompt Engineering Method Efficacy:}
Data shows that proprietary models like GPT4, GPT3.5, and GLM4 excel beyond open-source models such as ChatGLM3 and Llama2. Significant accuracy gains were observed with GPT4 and GLM4 using prompt engineering, whereas methods like Self-CoT saw a minor performance reduction in GPT3.5, ChatGLM3, and Llama2. This indicates that while advanced models benefit from prompt-guided reasoning, imposing such techniques on models with less sophisticated reasoning abilities may lead to performance decrements.

\textbf{Key Information Detection Shortcomings:}
A general shortfall in key information detection was noted, especially with GPT4-Turbo's average accuracy standing at 40\%. While accurate answers don't always require pinpointing key information, a direct correlation exists between identifying such information and answer accuracy. Directly presenting key information to models notably improved RougeL scores and answer accuracy, emphasizing the importance of precise key information identification.

\textbf{Reduced Demonstration Effectiveness:}
The historical utility of demonstrations in enhancing model response parsing has diminished as models have grown adept at interpreting complex instructions. Integration of three-shot demonstrations resulted in unstable performance across various prompt methods and model types~\cite{gu2023xiezhi}.

\textbf{Self-Question Prompt Superiority:}
The Self-Question method, unique to this study, markedly improved key information detection and reasoning across models. This approach not only enhanced accuracy but also demonstrated a broader efficacy compared to other prompt engineering strategies, reinforcing its value in augmenting model understanding and reasoning capabilities.

\input{figures/fig_analysis}

\subsection{Optimizing Model Capabilities through Fine-Tuning}
\subsubsection{Experimental Setup}
\textbf{Baselines:}
This investigation employed four prominent open-source models to explore fine-tuning's role in augmenting model capabilities. Our focus was on assessing the effectiveness of the Self-Question Prompt~(SQ Prompt) applied directly, the SQ Prompt within multi-round dialogues~(SQ Prompt w/ MR Chat), fine-tuning using DetectBench data~(SQ FT w/ Detective), and generating fine-tuning data from the DetectBench's Context, Question, and Answer (SQ FT w/ Generated). The appendices provide in-depth prompt descriptions utilized in each method.

The experiments aimed to evaluate the impact of Self-Question Fine-tuning on improving models' key information detection and reasoning abilities. To this end, a subset of 398 training dataset samples was used for fine-tuning over 3 epochs with the AdamW optimizer, detailed in the Appendix~\ref{appendix_training}.

\subsubsection{Insights and Evaluations}

\textbf{Effects of Transitioning to Multi-Round Dialogues:}
Our analysis revealed that transitioning from single-round to multi-round dialogues negatively influences chat model accuracy by 1.3\%, while base models experience a 3.0\% accuracy enhancement. This differential impact suggests that base models, due to their heightened sensitivity to context, benefit from multi-round dialogues as a mechanism to distill relevant information. On the contrary, chat models, which are adept at key information extraction, face performance setbacks when dialogue is fragmented into multiple segments.

\textbf{Enhancements from DetectBench Data in Fine-Tuning:}
Utilizing DetectBench data for Self-Question Fine-tuning significantly boosts key information detection and reasoning skills in models. The observed post-fine-tuning improvements include a 15.2\% increase in key information detection accuracy and a 10.5\% uplift in overall model performance. These results underscore the DetectBench dataset's effectiveness in refining models' information processing and reasoning faculties.

\subsection{In-depth Performance Analysis}
\subsubsection{Performance Influencing Factors}
The analysis of GPT4-Turbo's performance, as detailed in Figure~\ref{fig:gpt4_performance}, highlights the effects of varying Context Length and Options Length on model accuracy. A notable decline in accuracy was observed as Context Length increased from 400 to 800 words, with accuracy dropping from approximately 65\% to 35\%. Additionally, the variability in Options Length indicated a struggle with reasoning complexity at both extremes of option length.

An examination of our annotations against model performance revealed a strong correlation between the volume of Key Information, reasoning depth, and performance metrics. Specifically, as the number of key information instances and reasoning depth escalated, a marked decrease in model accuracy was recorded, affirming the relationship between question complexity and model effectiveness.

\subsubsection{Varied Responses to Different Question Types}
The performance variation across different question types, as presented in Figure~\ref{fig:performance_category}, shows models excelling in answering ``Why'' and ``Where'' questions, with the fine-tuned Llama-2 model achieving an impressive 90\% accuracy. In contrast, the accuracy for ``Who'', ``Which'' and other question types hovered around 50\%. This disparity suggests that while models effectively handle questions requiring an understanding of processes and environments, they struggle with questions that demand sophisticated entity recognition and relational discernment, pinpointing areas for future model enhancement.

==> latex/072Annotation.tex <==

\subsection{Details about Annotators}
The annotators for this research are the authors of this paper themselves. 
Respecting the requirement for anonymity, specific details regarding the number and education degrees of the annotators are not elaborated here.
It can be shared that the annotators are experts in the field of Computer Science and Cognitive Psychology.
The entire annotation process was under the stringent supervision and scrutiny of the first author of this paper.



\subsection{Annotation Tasks and Goals}
All the manual annotation tasks and targets are listed in Tab.~\ref{tab:annotation_request}.





\subsection{Case of Annotation}
We list some of the cases in our annotation process in Tab.~\ref{tab:appendix_annotation_example}

==> latex/073Demonstration.tex <==
In this section, we detail how we construct 5-shot demonstration for each baseline.
As shown in Tab.~\ref{experiments}, we use 5-shot demonstration in \texttt{Naive}, \texttt{Auto-CoT} and \texttt{Hint-Naive}.
The detail of how demonstrations are constructed are shown in Fig.~\ref{fig:naive_5shot}, Fig.~\ref{fig:hintnaive_5shot} and Fig.~\ref{fig:autocot_5shot}.

\begin{figure*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \includegraphics{figures/Demon_Case_1.pdf}}
    \caption{Example of how we construct 5-shot demonstration in Naive setting.}
    \label{fig:naive_5shot}
\end{figure*}

\begin{figure*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \includegraphics{figures/Demon_Case_2.pdf}}
    \caption{Example of how we construct 5-shot demonstration in Hint-Naive setting.}
    \label{fig:hintnaive_5shot}
\end{figure*}

\begin{figure*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \includegraphics{figures/Demon_Case_3.pdf}}
    \caption{Example of how we construct 5-shot demonstration in Auto-CoT setting.}
    \label{fig:autocot_5shot}
\end{figure*}






==> old_version/01.Introduction.01.tex <==
Reasoning ability is crucial for helping individuals make decisions, solve problems, and think critically based on the existing knowledge and situation~\cite{huang2022towards,qiao2022reasoning}.
In Cognitive Psychology, ``reasoning'' is composed of formal reasoning and informal reasoning~\cite{frith2008implicit,apperly2009humans}.
Formal reasoning is a systematic and logical process that follows a set of rules and principles, often used in mathematics and logic. 
While, informal reasoning is a less structured approach that relies on intuition, experience, and common sense to draw conclusions and solve problems, and is often used in everyday life~\cite{galotti1989approaches, bronkhorst2020logical}.
Notwithstanding the prevalence of formal reasoning in the field of machine learning research, the term ``reasoning'' mostly refer to informal reasoning in its common, everyday usage~\cite{cobbe2021training,huang2022towards}.

\begin{figure}[t]
    \centering
    \resizebox{0.8\columnwidth}{!}{
    \includegraphics{./figures/introduction.pdf}
    }
    \caption{A real response from GPT-4.
    Despite employing thorough prompting, GPT-4 continues to exhibit a deficiency in understanding real-life scenarios.}
    \label{fig:intro}
    \vspace{-5mm}
\end{figure}

The ability of Informal Reasoning is a fundamental human capability, permeating people's daily lives~\cite{blanchette2010influence,perkins2012everyday,bronkhorst2020logical}. 
For instance, on a hot summer day, when observing many people sitting in a room with closed windows and doors, one can easily deduce that the room is air-conditioned. 
The process of deduction is based on the common sense of the reasoner and the experience of once sitting in air-conditioned rooms.
This manifestation of inference abilities prevalent across diverse real-life scenarios showcases an array of cognitive skills, such as grasping common sense, abstracting problems, computing probabilities, discarding irrelevant information, and employing logical reasoning. 
Humans excel at doing informal reasoning, especially in life scenarios, often extracting conclusions subconsciously within a brief time span~\cite{woiceshyn2020intuiting}. 
As the capabilities of LLMs continue to scale these days, the crucial question arises: \textit{Can artificial neural networks also display super-powerful informal reasoning capabilities just like or go beyond humanity?}





Limited attention has been devoted to exploring this question within the field of Natural Language Processing~(NLP)~\cite{kaddour2023challenges,huang2022towards} after the fast development of large language models~(LLMs). 
Currently, the majority of AI reasoning endeavors concentrate on formulaic reasoning~\cite{hendrycks2021measuring, lewkowycz2022solving} or predicate reasoning~\cite{lu2022parsing}. 
Although these reasoning capacities aid the prevailing LLMs in tackling abstract problems~\cite{fu2023chain}, they fall short in fostering a deeper comprehension of human experiences.
To propel LLMs towards achieving Artificial General Intelligence~(AGI), it is imperative to not only cultivate their reasoning capabilities in disciplines such as mathematics and physics but as well as equip them with the ability to reason within real-world contexts.
Even the advanced GPT-4, which is considered to be one of the most powerful LLM, exhibits a lackluster performance in informal reasoning as illustrated in Fig.~\ref{fig:intro}.


Transitioning from mere recognition of the gap between LLMs and humans in informal reasoning ability to the investigation of human-like reasoning in neural models and narrowing this gap, we underscore the significance of developing a novel reasoning dataset targeting everyday life scenarios.
To this end, we introduce Detective Reasoning Puzzle Benchmark, which is an assembly of 1,200 questions gathered from accessible online resources and aiming at evaluating the model's informal reasoning ability in real life context.
Compared to recent popular domain knowledge reasoning datasets, the Detective Reasoning Puzzle Benchmark primarily comprises many detective-related questions, incorporating an abundance of information pertaining to character roles, human behaviors, mental activities, and environment description.
Solving these problems requires models to discover clues from details in the context, and reasoning based on the connection between clues and the questions.


In addition, we propose the Self-Question Prompt Framework to bridge the gap in LLMs' ability to carry out informal reasoning. 
To borrow the idea from the powerful informal reasoning ability of humans, we recruited 50 participants to tackle 20 questions each from the Detective Reasoning Puzzle Benchmark, leading to a detailed study of the reasoning processes of both humans and the model. 
Most participants said they find the clues mainly based on intuition without deeper thinking during the test, which is a typically informal reasoning process that sidesteps logical thinking, and instead uses experience and common sense to unearth critical elements in the context, promoting deep reflection, ultimately resulting in a reasoned outcome.
By mirroring human intuitive thinking, Self-Questioning is composed of four steps to improve the model's ability for informal reasoning. 
The goals of these steps respectively are to find key elements, deeply investigate the connections between these elements, encourage the relationship between each element and the problem, and finally, require the model to reasonably answer the problem.

Experimental results show that even the lowest score amongst participants~(46.6\%) significantly surpasses the best score from the LLMs questioned based on naive prompt~(16.0\%) within Detective Reasoning Puzzle Benchmark. 
Compared to the reasoning-enhanced prompts proposed by other researchers, our proposed self-question prompt generated the greatest performance improvement for GPT-4~(an increase of 17.4\%).
Although a self-question prompt is a better way to excite the model's potential in doing informal reasoning, there is still a huge gap between the SoTA LLMs performance~(33.4\%) with the average human participants~(74.2\%).




In conclusion, our study makes several key contributions: 
(1) To facilitate further detailed exploration into the informal reasoning abilities of large language models, we constructed Detective Reasoning Puzzle Benchmark, which is super challenging for LLMs but easy for humans, that includes 1,200 pieces of detective reasoning data. 
% Solving these reasoning problems requires the model to be able to disregard irrelevant information, utilize common knowledge, identify incongruities in the details of the problem, and thereby arrive at a proper reasoning outcome. 
(2) We designed a self-questioning prompt framework that can reliably induce the model to identify irrelevant information, draw the clue from the context, and perform reasoning based on the clues drawn from the details in the context. 
(3) We collected actual human responses to the Detective Reasoning Puzzle Benchmark and carried out numerous experiments using LLMs. 
Regarding these experimental outcomes, we conducted extensive analysis and discussion, which includes the gap between existing LLMs and humans in informal reasoning, the superiority of self-questioning prompts, and how LLMs can supplement informal reasoning abilities.



% Although formal reasoning is often occured in machine learning researches, the term ``reasoning'' refer to informal reasoning in most daily usage~\cite{cobbe2021training,huang2022towards}.

% The faculty of reasoning plays a pivotal role in equipping individuals with the capacity to make informed decisions, resolve predicaments, and exercise critical thinking, grounded in pre-existing knowledge and situational contexts~\cite{huang2022towards,qiao2022reasoning}. 
% Within the domain of Cognitive Psychology, ``reasoning'' encompasses two facets, namely formal and informal reasoning. Formal reasoning denotes a systemic, logical procedure adhering to a prescribed set of rules and principles, which is primarily employed within mathematics and logic. 
% Conversely, informal reasoning represents a less regimented approach that calls upon intuition, experience, and practical wisdom to derive conclusions and untangle situations. It is typically utilized in day-to-day life~\cite{galotti1989approaches, bronkhorst2020logical}. 
% Notwithstanding the prevalence of formal reasoning in the field of machine learning research, the term ``reasoning'' mostly refer to informal reasoning in its common, everyday usage~\cite{cobbe2021training,huang2022towards}.


% Transitioning from mere recognition of real-life scenarios to the investigation of human-like reasoning in neural models, we underscore the significance of developing a novel reasoning dataset targeting everyday life scenarios.
% To narrow this gap, we introduce Detective Reasoning Puzzle Benchmark, which is an assembly of 1,200 questions gathered from accessible online resources, aims at evaluating the model's informal reasoning ability in real life context.


% 进一步，我们提出使用Self-Question Prompt Framework来弥补LLM在Informal Reasoning能力上的缺失。
% 我们邀请了50位参与者每人回答20道Detective Reasoning Puzzle Benchmark里的题目，并对人类和模型的推理过程进行了详细的分析。
% 大多数受试者在测试时都依靠直觉进行了推理。
% 直觉推理是一种绕过理性思考，依靠经验和常识发现Context中的关键点，并进行深度思考，最终得到推理结果的方法。
% LLM没有直觉，所以我们尝试改进prompt，通过不断地Self-Question来还原人类依靠直觉进行思考的过程，从而提升LLM的informal reasoning能力。



% 我们模仿人类的直觉思考，设计了Self-Question的四个过程来增强模型的informal reasoning的能力，目标分别是发现关键要素、深究要素之间的关联、启发各个要素与问题之间的联系，最后要求模型合理地回答问题。

% we recreating the human thought process driven by intuition through continuous Self-Questioning, thereby enhancing the LLM's capacity for informal reasoning.



% The benchmark consists of an assembly of 1,200 questions compiled from accessible online resources.
% The question is mainly gathered from open source web, and are filtered and preprocessed manually before experiments and released.
% Except for the ``Context'', ``Question'' and ``Answer'', which can be obtained directly from online resource, we manually annotate the ``Hint'' for every question to facilitate model training or deep exploration for furture research. 

% We referred to guidelines built on psychological principles~\cite{minnameier2010abduction} and made use of web scraping to gather clear explanations and hint for each question and answer within the Benchmark.
% Since there are lot of internet slang, incorrect words present in the raw text, and varying quality levels of the initial questions, we proceeded with a manual review. 
% Ultimately, each question is transformed into a structured form as depicted in Fig.~\ref{fig:example}.

% In addition to this, we have further designed a prompt framework capable of thoroughly extracting various detailed information from the context to increase the performance of LLM on Detective Reasoning Puzzle Benchmark.
% As LLM generally assumes that prompts are correct and useful, the presence of distracting information greatly hampers its effectiveness~\cite{shi2023large}.
% Besides, we find that ChatGPT and GPT-4, which are LLMs contain huge amount of common-sense knowledge, have better performance in answering the detective reasoning puzzles when step-by-step asking them to draw the clue from the context, and do the reasoning based on the given context and the clues.
% In order to stably induce LLMs to ignore the irrelevant context, and to find the clues based on the given context, we propose the self-question prompt framework.
% As depicted in Fig.~\ref{fig:intro}, the self-question prompt framework comprises four stages: detail detection, detail connection, relevance inspiration, and output command.
% This approach allows models to uncover the implicit hints embedded within the context, discard irrelevant information, and reasoning based on beneficial information.


% To evaluate the gap between human and AI models in informal reasoning, we invite 50 participants to each answer 20 questions within our proposed Detective Reasoning Puzzles Benchmarks. 
% In addition, we examined the performance of four best models in Alpaca-Eval with different parameter magnitudes on the Detective Reasoning Puzzles Benchmarks. 
% Given that GPT-4 has been confirmed by most researchers to have strong evaluation capabilities, we employed GPT-4 to help with our assessments. 
% To ensure accuracy, we utilized manual sampling evaluations to cross-check the results derived from GPT-4. 



% \begin{enumerate}
% \item To facilitate further detailed exploration into the informal reasoning abilities of large language models, we constructed a detective reasoning benchmark that includes 1,200 pieces of detective reasoning data. 
% Solving these reasoning problems requires the model to be able to disregard irrelevant information, utilize common knowledge, identify incongruities in the details of the problem, and thereby arrive at a proper reasoning outcome. 
% \item We designed a self-questioning prompt framework that can reliably induce the model to identify irrelevant information, draw the clue from the context, and perform reasoning based on the clues drawn from the details in context. 
% \item We collected actual human responses to the Detective Reasoning Benchmark and carried out numerous experiments using LLMs. 
% Regarding these experimental outcomes, we conducted extensive analysis and discussion, which includes the gap between existing LLMs and human in informal reasoning, the superiority of self-questioning prompts, and how LLMs can supplement informal reasoning abilities.

% \end{enumerate}


==> tables/tab_ablation.tex <==



\begin{table}[t]
    \centering
    % \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|c|c|c|c|}
    \hline
        \multirow{2}{*}{Method} & \multicolumn{4}{c|}{Detective Reasoning} \\
         & Easy & Middle & Hard & All \\
          \hline
          \multicolumn{5}{|l|}{\cellcolor{mygray} \textbf{\textit{Self-Question}}} \\
          \hline
        w/o None & 41.3 & 27.7 & 30.5 & 35.8\\
          w/o WR & 41.7 & 24.5 & 26.8 & 34.6\\
          w/o WR,AI & 35.9 & 21.4 & 17.1 & 28.6\\
          w/o WR,AI,DC & 30.0 & 16.0 & 8.5 & 22.3\\
          \hline
          \multicolumn{5}{|l|}{\cellcolor{mygray} \textit{Others}} \\
          \hline
          Naive & 22.4 & 11.7 & 3.66 & 16.0\\
          Self-CoT & 17.5 & 8.5 & 2.4 & 12.4\\
          PS-CoT & 24.7 & 12.8 & 13.4 & 19.6 \\
         \hline
    \end{tabular}
    % }
    \caption{The ablation study of various design in self-question prompt framework, and the comparison with other baselines.}
    \label{tab:ablation}
    \vspace{-5mm}
\end{table}


==> tables/tab_case1.tex <==
\begin{table*}[t]
\small
\centering
\resizebox{\textwidth}{!}{
\begin{tabularx}{1.6\textwidth}{|p{1.576\textwidth}|}
\hline
    \makecell[c]{\textbf{Case 1}} \\
    \hline
    \textbf{Context:} \\
    On a snowy winter night, a single woman was murdered in the door of the room at 68 King's West Road, the time of the murder being around 8pm that night. The police launched an in-depth investigation as soon as they arrived on the scene and found a room where the gas stove was red-hot from the fire, the room was hot and sweaty, the electric light was still on, yet the tightly closed window was only half covered with curtains. A young man, a resident near the victim's home, gave the police the following eyewitness evidence: 
“I had witnessed the murder last night at around 11pm, and although my room was 20 meters from the scene, I found the murderer to be a blond man with black-rimmed glasses and a beard.” 
Following a tip-off from him, the police arrested a blonde boyfriend of the deceased. In court, the blonde suspect's lawyer defended him confidently and asked the witness: 
“Young man, you saw this murderer by chance at the window at the time of the crime, didn't you?”,
“Yes, because the window opposite was transparent and her curtains were half-covered that night, so I was able to see the killer's face clearly from 20 meters away.” 
At this point, the lawyer said with certainty, 
“Your Honor, what this young man has said is a lie, which means he is guilty of perjury. In my judgement, he is the most suspicious because he pulled the curtains from the victim's house and fled only after the murder was committed. He also gave a false statement to the police in an attempt to cover up his crime.” 
As a result, the review proved that the lawyer's deduction was correct.
 \\ \\
 \textbf{Hint:}\\
 The clue is in the condition of the room and the weather during the night of the murder. The room was hot due to the gas stove being on, and it was a heavily snowing outside. What would this mean for the window of the room? And how does it affect the young man's testimony of seeing the murderer clearly from 20 meters away?
 \\
 \\
    \textbf{Question:} \\
    Do you know how the lawyer deduced this?\\
\\
\textbf{Answer:} \\
That night it was snowing heavily and the gas stove on site was burning red hot, in which case the room was warm. So, with the heat in the room, the glass was covered with a layer of moisture and became hazy and unclear. Even if one could see someone in the room, it would only be a silhouette, so how could one tell that he had blond hair and a beard? It is clear that the young man had pulled back the curtains after the murder and then left in a hurry.

\\
    \hdashline
    \textcolor{blue}{\textbf{Naive Output}}\ \xmark \\
    \textbf{Prompt:}\\
    Below is a puzzle about detective reasoning, I split the question into ``context'' and ``question'', please answer the question properly based on the context: \\
    \text{[}Context\text{]} + \text{[}Question\text{]} \\
    \textbf{Answer:} \\
    The young man claimed he saw the murder at 11pm, but the murder took place at 8pm. Furthermore, he claimed he saw it from his window 20 meters away, despite the fact that the murder victim's window was only half-open and it was a snowy night. It would be difficult to see detail like hair color, glasses, and a beard from that distance in those conditions. The lawyer concluded that the young man must have been close enough to handle the curtains, thus suspecting him of the crime.\\
    
    \hdashline
    \textcolor{blue}{\textbf{Self Chain-of-Thought}}\ \xmark \\
    \textbf{Prompt:} \\
    Below is a puzzle about detective reasoning, I split the question into ``context'' and ``question'', please answer the question properly based on the context \textit{\textbf{step by step}}: \\
    \text{[}Context\text{]} + \text{[}Question\text{]} \\
    \textbf{Answer:} \\
    Step 1: The lawyer noted inconsistencies in the young man's story. The young man claimed he witnessed the murder at 11pm, three hours after the estimated time of the murder which was around 8pm.\\
Step 2: The young man also claimed he was able to see specific details about the murderer - that he was a blond man with black-rimmed glasses and a beard - from his room 20 meters away. Given the murder took place on a snowy night, visibility would be poor.\\
Step 3: Despite the fact that the room was described as hot and sweaty, the window was only halfway open. It would be difficult to clearly observe someone from 20 meters away through a half-open window, especially during a snowy night.\\
Step 4: Based on these inconsistencies and improbabilities, the lawyer deduced that the young man was lying about what he witnessed.\\
Step 5: The lawyer then inferred that if the young man was able to see so clearly, he must not have been 20 meters away but rather close up, possibly inside the room. Therefore, the young man's close proximity and inaccurate statements made him the prime suspect in the lawyer's eyes.\\
Step 6: The lawyer argues that the young man gave a false statement to police in an attempt to cover up his own involvement in the crime. The court subsequently found these deductions to be correct. \\
    \hdashline
    \textcolor{blue}{\textbf{Manual Chain-of-Thought}}\ \cmark \\
    \textbf{Prompt:} \\
    Below is a puzzle about detective reasoning, i split the puzzle into ``context'', ``hint'' and ``question'', please answer the ``question'' properly based on ``context'' \textbf{\textit{and ``hint''}}. \\
    \text{[}Context\text{]} + \text{[}Question\text{]} + \textbf{\textit{\text{[}Hint\text{]}}}\\
    \textbf{Answer:} \\
    The lawyer deduced this from the fact that it was a snowy winter night. Due to the high temperature in the room from the gas stove, the window would have been fogged or covered with condensation on the inside because of the contrast between the warm room and the cold outside weather. This would have made it nearly impossible for the young man to clearly see the murderer's face from 20 meters away through the window, especially specific details like black-rimmed glasses and a beard. Thus, the young man's testimony was called into question, and his involvement in the crime was suspected. \\
    
    \hdashline
    \textcolor{blue}{\textbf{Plan \& Solve Chain-of-Thought}}\ \cmark \\
    \textbf{Prompt:} 
    Below is a puzzle about detective reasoning, i split the puzzle into ``context'' and ``question'', \textbf{\textit{please first understand the ``context'', extract relevant variables, and devise a plan. Then let's carry out the plan, answer the ``question'' step by step, and show the answer:}}\\
    \text{[}Context\text{]} + \text{[}Question\text{]} \\
    \textbf{Answer:} \\
    First, let's identify the relevant variables from the context:

The time of the murder: around 8pm.\\
The eyewitness saw the murder: at 11pm.\\
The distance between the eyewitness' room and the scene of the crime: 20 meters.\\
The state of the victim's room: gas stove red-hot, room hot, electric light on, closed window half covered with curtains.\\
The eyewitness' testimony: a description of the murderer; able to see the killer's face clearly from 20 meters away.\\
Based on these variables, the plan to find out how the lawyer deduced the suspicion of the witness would likely involve:\\ \\

Identifying any contradictions or inconsistencies in the statements or circumstances.\\
Evaluating the witness' testimony and its plausibility considering the conditions described.\\
Now let's carry out this plan:\\ \\

One contradiction lies in the time of the murder and the time the eyewitness claimed to have seen the murder. The murder happened around 8pm, but the witness claimed that he had witnessed the murder at 11pm.\\

Besides, the witness claimed he could see the murderer's face clearly at night from 20 meters away. Considering the physical conditions of the room described (the window was closed and only half-covered with a curtain), it seems implausible. The room was heated by a red-hot stove and the electric light was on, so the window was likely to have been steamed up, obstructing the view from outside, especially on a snowy winter night.\\

From these contradictions and implausibilities, the lawyer determined that the eyewitness was lying. His ability to describe the supposed murderer in detail, coupled with his presence at the scene (evident by his knowledge of the half-closed curtains) also raised suspicion that the eyewitness was indeed the culprit and had manipulated the scene to deceive the police. The lawyer thus accused the witness of murder, framing the blonde man, and perjury. \\
    
    \hdashline
    \textcolor{blue}{\textbf{Self-Question}}\ \cmark \\
    \textbf{Prompt:} \\
    Below is a puzzle about detective reasoning, i split the puzzle into ``context'' and ``question''. \textbf{\textit{Please first extract some key elements in the context.
    Then deduce some clue based on these elements. 
    After that, find the connection between these elements and clues to the question. 
    Finally, answer the question based on all the information.}} \\
    \text{[}Context\text{]} + \text{[}Question\text{]} \\
    \textbf{Answer:} \\
    Key Elements:\\

The crime took place around 8pm on a snowy winter night.\\
The eyewitness claimed to have witnessed the murder at 11pm.\\
The room was hot and the window was closed, but half covered with curtains.\\
The witness claimed to have seen the killer's face clearly from 20 meters away.\\ \\
Clues:\\

The difference in times that the murder took place and when the witness saw the event.\\
The conditions in the room suggest that the window was likely to have been fogged up given the heat inside.\\
The distance between the eyewitness's room and the scene makes the claim that the witness saw the murderer's face clearly suspicious.\\ \\
Connection: The lawyer focuses on the inconsistencies to doubt the reliability of the witness's testimony. The contradiction in the time of the event and the unlikelihood of the witness seeing through a likely fogged-up window from a significant distance both serve to discredit the witness.\\ \\

Answer: The lawyer deduced that the witness was lying based on the discrepancies in his testimony, namely the contradiction in the timing he reported and the implausibility of having a clear view of the murderer's face through a likely fogged-up window from a distance of 20 meters. He suspected the witness of committing the murder and fabricating the description to frame the suspect with blonde hair. The lawyer posited that the "eyewitness" was actually the real killer who had pulled the curtains, murdered the woman, and then given a false statement to divert police suspicion away from himself and towards the blonde man. \\
\hline
\end{tabularx}
}
\caption{Case study of our proposed synonym mining method and text data augmentation algorithms}
\label{tab:case1}
\end{table*}





==> tables/tab_case2.tex <==
\begin{table*}[t]
\small
\centering
\resizebox{\textwidth}{!}{
\begin{tabularx}{1.6\textwidth}{|p{1.576\textwidth}|}
\hline
\makecell[c]{\textbf{Case 2}} \\
\hline
\textbf{Context:} \\
The phone rang as the television actress, Asai Miyoko was applying her makeup at her vanity. She reached over to pick up the receiver. “Have you prepared the money yet?” her heart sank as she recognized the man’s voice on the other end. “Erm… yeah… I’m working on it…” “Well then, let's make the exchange today.” “Where?” “There’s an apartment complex near Hikari Hills Station, come to room number 508.” “What time should I come?” “Whenever it’s convenient for you?” “How about one in the afternoon?” “Okay, I’ll wait for you.” The man let out a grating laugh and ended the call. Miyoko sat still, not even remembering to put the phone back down as she stared at a small capsule she’d taken out from her vanity drawer. It contained potassium cyanide that she’d stolen when she stayed at her sister’s place who ran a pharmacy. Two years prior, she’d been coerced by a TV director into undergoing an abortion and the man now blackmailing her somehow got his hands on her medical records.
When the phone rang, the professional tennis player, Tomoya, was in the bathroom. He hurriedly rushed out to answer it. “Have you prepared the money yet?” He straightened on hearing the familiar voice, “Ah, I’m working on it…” “Well then, give me the money today.” “Where?” “There’s an apartment complex near Hikari Hills Station, come to room number 508.” “When?” “Two in the afternoon. I’ll be waiting for you.” The man laughed and hung up. Tomoya thought for a long while before pulling out a small medicine bottle from his drawer. It contained potassium cyanide that he’d stolen from his wife’s electroplating factory’s poison cabinet a day ago.
The phone rang as the innocent pop idol, Kato Mayumi, was eating breakfast alone in her kitchen. “Did you prepare the money I asked for?” Her body shivered as she recognized the man’s voice over the phone. “Erm… well…” “Give me the money today.” “Where?” “There’s an apartment complex near Hikari Hills Station, come to room number 508.” She replied, “Erm… I had plans to go driving around for fun today…” He responded, “Do you think your little trip is more important than our transaction here? Anyway, you can come anytime between one and three, I’ll be waiting.” The man menacingly ended the call.
 \\ \\
 \textbf{Hint:}\\
 Observe the temperature inside the room, the status of the windows, you will find contradictory clues. Look for phenomena that only occur during a power outage.
 Potassium cyanide, if it is in contact with the air for a long time, will turn into potassium carbonate and lose its toxicity. One suspect's potassium cyanide has been stored for two years, so consider what changes might have occurred.
 Take note of the different references by suspects to the air conditioning, elevator, and power outage. These could reveal key aspects of the suspect’s actions.
 Read carefully through each person's actions. You'll find one person's actions differ from the others, which might be a key clue to the culprit.
 In the afternoon, from half-past one to half-past two, one suspect arrived at the apartment during the power outage. What method did they use to get in?
 \\
 \\
\textbf{Question:} \\
Who among the three used the potassium cyanide to murder the blackmailer and why?\\
\\
\textbf{Answer:} \\
The murder took place during a power outage. Due to the outage, the air conditioner stopped working and the room became hot, causing the victim to open the window themselves. If the victim was still alive when the power was restored and the air conditioner started working again, they would have closed the window. Only Tomoya and Mayumi visited the scene during the power outage. However, who killed the victim with their potassium cyanide? If potassium cyanide is not stored in an airtight container and is exposed to air for a long period, it will turn into potassium carbonate and lose its toxicity. The potassium cyanide Mayumi had was wrapped in paper for two years, and thus, had already lost its potency. \textbf{\textit{Therefore, the murderer is Tomoya.}}

\\
\hdashline
\textcolor{blue}{\textbf{Naive Output}}\ \xmark \\
\textbf{Prompt:}\\
Below is a puzzle about detective reasoning, I split the question into ``context'' and ``question'', please answer the question properly based on the context: \\
\text{[}Context\text{]} + \text{[}Question\text{]} \\
\textbf{Answer:} \\
\textbf{\textit{Kato Mayumi.}} Although all three suspects have the motive and means to kill the blackmailer, the timing of the power outage in the apartment suggests only Mayumi had the chance to do so. The elevator in the blackmailer's home could not operate after the power went off, so only the person who arrived before the power outage (Mayumi) could have seen him before he was killed. The other two people, one couldn't take the elevator due to the blackout and had to climb the stairs, while the other left when the elevator was stuck on the first floor, so neither of them had the chance to see the blackmailer before the power outage.\\

\hdashline
\textcolor{blue}{\textbf{Self Chain-of-Thought}}\ \xmark \\
\textbf{Prompt:} \\
Below is a puzzle about detective reasoning, I split the question into ``context'' and ``question'', please answer the question properly based on the context \textit{\textbf{step by step}}: \\
\text{[}Context\text{]} + \text{[}Question\text{]} \\
\textbf{Answer:} \\
Firstly, if Miyoko's elevator descended to the first floor when the power went off, it means that the other two have already been to the scene, otherwise Miyoko should have been trapped in the dark elevator. So, Miyoko is the last one to leave the scene.\\

Secondly, Tomoya went up the stairs, and he mentioned that he encountered two housewives. If he was the criminal, he wouldn't have allowed the two housewives to see him exit the stairwell, as that would serve as incriminating evidence.\\

Thirdly, Mayumi mentioned that onlookers were staring at her. If she was seen leaving the apartment, wouldn't that be very dangerous?\\

From these clues, it is most likely that \textbf{\textit{Miyoko killed the blackmailer}}. Because she was the last one to leave the scene, and due to the power outage, the elevator stopped operating, she wouldn't encounter anyone else, therefore there was no risk of being seen leaving the apartment.\\
\hdashline
\textcolor{blue}{\textbf{Manual Chain-of-Thought}}\ \cmark \\
\textbf{Prompt:} \\
Below is a puzzle about detective reasoning, i split the puzzle into ``context'', ``hint'' and ``question'', please answer the ``question'' properly based on ``context'' \textbf{\textit{and ``hint''}}. \\
\text{[}Context\text{]} + \text{[}Question\text{]} + \textbf{\textit{\text{[}Hint\text{]}}}\\
\textbf{Answer:} \\
\textbf{The answer is Tomoya.} He is the only one who arrived at the apartment during the power outage, and because the elevator was out of service, he had to take the stairs. He also mentioned encountering two housewives on the stairs, which indicates that the elevator was already out of order at that time. However, he did not mention that the air conditioning in the room was on, which conflicts with the statements of the other two suspects. Only those who took the elevator upstairs would know that the room's air conditioning would also stop working after the power outage. This suggests that he had already arrived at the apartment before the power outage, therefore the victim's time of death was before the power cut, which is when he arrived. Moreover, the potassium cyanide was just obtained by him last night, so it couldn't undergo a chemical change to become non-toxic. Therefore, the murderer who poisoned the victim is Tomoya. \\

\hdashline
\textcolor{blue}{\textbf{Plan \& Solve Chain-of-Thought}}\ \xmark \\
\textbf{Prompt:} 
Below is a puzzle about detective reasoning, i split the puzzle into ``context'' and ``question'', \textbf{\textit{please first understand the ``context'', extract relevant variables, and devise a plan. Then let's carry out the plan, answer the ``question'' step by step, and show the answer:}}\\
\text{[}Context\text{]} + \text{[}Question\text{]} \\
\textbf{Answer:} \\
Context:\\

We have three characters who are being blackmailed: The television actress, Asai Miyoko; the professional tennis player, Tomoya; and the pop idol, Kato Mayumi. They were all asked to go to an apartment complex near Hikari Hills Station, room number 508. Miyoko's meeting is at one in the afternoon, Tomoya's at two in the afternoon, and Mayumi can come anytime between one and three in the afternoon. Both Miyoko and Tomoya have stolen potassium cyanide, which is extremely poisonous.\\ \\ 

Plan: \\

Understand the chronology of events, like what times are specified for each person to meet with the blackmailer.
Analyze the opportunities each person would have had to use the cyanide.
Determine the individual motive for each person.\\ \\ 
Execution:\\

Miyoko is supposed to meet the blackmailer at 1 PM. This gives her the first opportunity to meet the blackmailer and potentially poison him before the others arrive. Tomoya comes next at 2 PM. Mayumi can come anytime between 1 PM and 3 PM.
Both Miyoko and Tomoya have potassium cyanide, so both could potentially poison the blackmailer if they have the opportunity to do so.
Everyone has a motive to kill the blackmailer as he is threatening their lives, and they all have been violated by him in different ways.\\
Based on this analysis, \textbf{\textit{the most likely person to have used the potassium cyanide to murder the blackmailer would be Miyoko}}, primarily because she is the first one scheduled to meet with him, providing her the opportunity to poison him before the others arrive.
However, without evidence that the blackmailer is indeed dead, and without knowing whether the blackmailer met Miyoko first or violated the arranged schedule, we can't say with 100\% certainty who would or wouldn't have had the opportunity to murder the blackmailer. \\
    
\hdashline
\textcolor{blue}{\textbf{Self-Question}}\ \cmark \\
\textbf{Prompt:} \\
Below is a puzzle about detective reasoning, i split the puzzle into ``context'' and ``question''. \textbf{\textit{Please first extract some key elements in the context.
Then deduce some clue based on these elements. 
After that, find the connection between these elements and clues to the question. 
Finally, answer the question based on all the information.}} \\
\text{[}Context\text{]} + \text{[}Question\text{]} \\
\textbf{Answer:} \\
Key elements:\\

Asai Miyoko, the television actress, is asked to come to room number 508 at an apartment complex near Hikari Hills Station at one in the afternoon. She has potassium cyanide.\\
Tomoya, the professional tennis player, is asked to come to the same room at two in the afternoon. He also has potassium cyanide.
Kato Mayumi, the pop idol, is asked to come to the same room anytime between one and three in the afternoon.\\\\
Clues:\\

All three are being blackmailed and have access to potassium cyanide.\\
The blackmailer has different meeting times with each person.\\
Connection: The meeting times are crucial. The blackmailer is meeting Miyoko at one, Tomoya at two, and Mayumi anytime between one and three.\\\\

Answer:\\
\textbf{\textit{Tomoya, the professional tennis player, is the most likely to have used the potassium cyanide to murder the blackmailer.}} This is because he was scheduled to meet the blackmailer after Miyoko, meaning the blackmailer would still be alive when she arrived. Mayumi could have potentially been the murderer, but since her time slot overlaps with both Miyoko and Tomoya, it's less certain. Tomoya, however, was scheduled to meet the blackmailer alone, giving him the perfect opportunity to commit the crime.\\
\hline
\end{tabularx}
}
\caption{Case study of our proposed synonym mining method and text data augmentation algorithms}
\label{tab:case2}
\end{table*}





==> tables/tab_dataset_statistic.tex <==
\begin{table}[t]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
数据集名称 & 题目数量 & 题目长度 & 推理深度 & 是否开源 & GPT-4结果 & Human Performance \\ \hline
HellaSwag & - & - & - & - & - & - \\ \hline
WinoGrande & - & - & - & - & - & - \\ \hline
StrategyQA & - & - & - & - & - & - \\ \hline
HotpotQA & - & - & - & - & - & - \\ \hline
True Detective & - & - & - & - & - & - \\ \hline
\end{tabular}
\caption{Your caption}
\label{your_label}
\end{table}

==> tables/tab_experiments.tex <==

\begin{table*}[ht]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|}
    \hline
         & Hum-LOW & Hum-AVG & Hum-HIG & Vicuna-7B & WizardLM & Vicuna-33B & GPT-3.5 & GPT-4 \\
        \hline
        
        \multicolumn{9}{|l|}{\cellcolor{mygray} \textit{Naive Questioning}} \\
        \hline
        Naive (0-shot) & 47.3 & 74.2 & 94.7 & 0.0 & 0.0 & 0.6 & 7.8 & 16.0 \\
        Naive (5-shot) & - & - & - & 0.0 & 0.0 & 0.2 & 3.8 & 10.1 \\
        Self-CoT (0-shot) & - & - & - & 0.0 & 0.0 & 0.0 & 3.5 & 12.2 \\
        Auto-CoT (5-shot) & - & - & - & 0.0 & 0.0 & 0.0 & 3.7 & 11.4 \\


        \hline
        \multicolumn{9}{|l|}{\cellcolor{mygray} \textit{Output Ensemble Method}} \\
        \hline
        Self-Consistency (0-shot) & - & - & - & 0.0 & 0.0 & 0.5 & 5.4 & 11.3 \\
        Complexity-CoT (0-shot) & - & - & - & 0.0 & 0.0 & 0.0 & 2.4 & 7.6 \\
        
        \hline
        \multicolumn{9}{|l|}{\cellcolor{mygray} \textit{Hint Injection}} \\
        \hline
        Hint-Naive (0-shot) & 85.0 & 93.2 & 100.0 & \textbf{1.5} & \textbf{2.8} & \textbf{4.4} & \textbf{34.6} & \textbf{65.3} \\
        Hint-Naive (5-shot) & - & - & - & 0.0 & \textbf{0.6} & \textbf{1.9} & \textbf{27.5} & \textbf{54.1} \\

        \hline
        \multicolumn{9}{|l|}{\cellcolor{mygray} \textit{Multi-step Chain-of-Thought}} \\
        \hline
        PS-CoT (0-shot) & - & - & - & 0.3 & 0.2 & 0.9 & 9.1 & 19.5 \\
        \textbf{Self-Question (0-shot)} & - & - & - & 0.0 & 0.1 & 1.1 & 21.7 & 35.8 \\
        
        
        % self-consistency (5-shot) & - & - & - & 0.0 & 0.0 & 0.0 & 4.5 & 17.3 \\
        % PS-CoT (5-shot) & - & - & - & 0.0 & 0.0 & 0.4 & 11.5 & 18.6 \\
        % Complexity-CoT (5-shot) & - & - & - & 0.0 & 0.0 & 0.0 & 1.5 & 4.7 \\
        % self-question (5-shot) & - & - & - & 0.0 & 0.0 & 0.0 & 20.5 & 37.1 \\
    \hline
    \end{tabular}
    }
    \caption{
    Comprehensive experiments were conducted across all baseline models. 
    It should be noted that the GPT-4 model declined to validate responses containing certain words deemed unsafe. Due to the fact that deductive reasoning puzzles often incorporate words such as "murder" or "steal", our statistical analysis only includes sample data that could be verified by GPT-4.}
    \label{tab:experiments}
    \vspace{-3mm}
\end{table*}


==> tables/tab_questions.tex <==

% \begin{table}[t]
%     \centering
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|c|c|l|}
%     \hline
%         Purpose & Mark & Prompt \\
%         \hline
%         \multirow{3}{*}{Detail Detection} & 1-1 & Read the following passage carefully and identify as many details as you can. Pay attention to descriptions, actions, and characters. Use your observational skills to identify anything else that might be of significance.\\
%         & 1-2 & What are the clue in the context?\\
%         & 1-3 & What are the key elements in the context?\\
%         \hline
%         \multirow{3}{*}{Detail Connection} & 2-1 & What are the key elements in the context?\\
%         & 2-2 & What are the clue in the context?\\
%         & 2-3 & What are the key elements in the context?\\
%         \hline
%         \multirow{4}{*}{Answer Inspiration} & 3-1 & What's the connection between the above \\ && clue and key elements with the question?\\
%         & 3-2 & What are the clue in the context?\\
%         & 3-3 & What are the key elements in the context?\\
%         \hline
%         \multirow{3}{*}{Output Command} & 4-1 & What are the key elements in the context?\\
%         & 4-2 & What are the clue in the context?\\
%         & 4-3 & What are the key elements in the context?\\
%     \hline
%     \end{tabular}
%     }
%     \caption{Accuracy on LSR-Benchmark. 
%     +A denotes finetune models based on alpaca dataset, +S denote finetune models based on LSR-Benchmark training set.
%     Bolded performance represent best performance within each group, underlined number represent best performance of each experiment setting.}
%     \label{tab:prompts}
% \end{table}



\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|l|}
    \hline
        \textbf{Purpose} & \textbf{Prompt} \\
        \hline
        \multicolumn{2}{|l|}{\cellcolor{mygray}\textit{Detective Thinking}}
        \\
        \hline
        
        \multirow{3}{*}{Detail Detection} & 
        Read the following passage carefully and identify as many details as you can. Pay
        \\&
        attention to descriptions, actions, and characters. Use your observational skills to
        \\&
        identify anything else that might be of significance.
        \\
        \hline
        \multirow{4}{*}{Detail Connection} & 
        Using the details you have identified from the context, draw connections and analyze
        \\&
        the relationships between them. Consider the significance of each detail and how it
        \\&
        relates to the larger meaning of the text. Look for patterns, symbolism, and other
        \\&
        elements that may help explain why the author included these specific details.\\
        \hline
        \multirow{5}{*}{Answer Inspiration} & 
        Using the details you have identified and the
        \\&
        clues you have drawn from the given question, analyze their connections and draw
        \\&
        conclusions about the larger meaning of the text. Consider the significance of each
        \\&
        detail and how it relates to the question. Look for themes, motifs, and other
        \\&
        elements that may help explain why the author included these specific details and clues.\\
        \hline
        \multirow{4}{*}{Weighted Reasoning} & 
        Answer the question by taking the raw context into consideration but mainly using the 
        \\&
        conclusion and the details you have drawn before. Remember the connection between your
        \\&
        drawn details and the conclusion to the question, don't be disturbed by the irrelevant
        \\&
        information in the context.
        \\
        \hline
        \multicolumn{2}{|l|}{\cellcolor{mygray}\textit{GPT-4 Usage}}
        \\
        \hline
        \multirow{8}{*}{Hint Output} & 
        Based on the given detective reasoning problem and its corresponding answer, create prompts \\&
        that concurrently aid respondents in understanding the question or the logical deduction process\\&
         without disclosing the answer outright or introducing unrelated information.\\&
         Question: ``Context + Question''\\&
         Answer: ``Answer''\\&
         You may think and reason before give the hint, please response in the following format: \\&
         ``Thinking and Reasoning Process: xxxxx\\&
         Hint: xxxxx'' \\
        \hline
        \multirow{7}{*}{Verification} & 
        Please verify the accuracy of the model's output in accordance with the provided standard answer.\\&
        If the result aligns or is similar to the standard answer, it should be deemed correct, on the contrary, \\&
        if the output from the model notably diverges from the answer, it should be considered incorrect. \\&
        Ground Truth: ``xxxx''\\&
        Model Output: ``xxx''\\&
        Please response in the following format:\\&
        ``Evaluation Result: xxxx\\&
        Evaluation Reason: xxxx''\\
        \hline
        
    \hline
    \end{tabular}
    }
    \caption{
    The prompts we used within the Self-Prompt Framework and when using the GPT-4 API.
    }
    \label{tab:prompts}
\end{table*}
